Serving Time: Real-Time, Safe Motion Planning and Control for Manipulation of Unsecured Objects

A key challenge to ensuring the rapid transition of robotic systems from the industrial sector to more ubiquitous applications is the development of algorithms that can guarantee safe operation while in close proximity to humans. Motion planning and control methods, for instance, must be able to certify safety while operating in real-time in arbitrary environments and in the presence of model uncertainty. This paper proposes Wrench Analysis for Inertial Transport using Reachability (WAITR), a certifiably safe motion planning and control framework for serial link manipulators that manipulate unsecured objects in arbitrary environments. WAITR uses reachability analysis to construct over-approximations of the contact wrench applied to unsecured objects, which captures uncertainty in the manipulator dynamics, the object dynamics, and contact parameters such as the coefficient of friction. An optimization problem formulation is presented that can be solved in real-time to generate provably-safe motions for manipulating the unsecured objects. This paper illustrates that WAITR outperforms state of the art methods in a variety of simulation experiments and demonstrates its performance in the real-world.

==> Algorithms/pzfk.tex <==
%~~~~~~~~~~~~ Compose FK
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]

% \State{\bf parfor} $i \in \Nt$ %// parallel for each time step

\State{\bf for} $j = 1:\nq+1$ %// for each joint \hspace{0.2in}

    \State\hspace{0.2in} $\pz{p_0}(\pzqi) \leftarrow \zeros$ %// initialize frame location 

    \State$\hspace{0.2in} \pz{R_0}(\pzqi) \leftarrow I_{3 \times 3}$ %// initialize frame orientation
    
    \State\hspace{0.2in}$\pz{R_{j}^{j-1}}(\pzqji), \pz{\nom{p\jssmu}} \leftarrow \pz{\homtrans_{j}^{j-1}}(\pzqji)$ as in \eqref{eq:homogeneous_transform}
    
    \State\hspace{0.2in}$\pz{p_j}(\pzqi) \leftarrow \pz{p_{j-1}}(\pzqi) \oplus \pz{R_{j-1}}(\pzqi) \pz{p_{j}^{j-1}}$
        
    \State\hspace{0.2in}$ \pz{R_j}(\pzqi) \leftarrow  \pz{R_{j-1}}(\pzqi)  \pz{R_{j}^{j-1}}(\pzqji)$ 
    
    \State\hspace{0.2in}$\pz{\FK_j}(\pzqi) \leftarrow \{ \pz{R_j}(\pzqi) ,  \pz{p_j}(\pzqi) \}$ 
     
    %  \State\hspace{0.4in}{\bf for} $l = 1:j$

    %     \State\hspace{0.6in}$\pzi{R}, \pzi{\nom{p}} \leftarrow \texttt{pzTransMat}(\pzi{q_j})$ 
    
    %     \State\hspace{0.6in}$\pzi{\pj} \leftarrow \pzi{\pj} \oplus \pzi{\Rj} \odot \pzi{p_{l}^{l-1}}$
        
    %     \State\hspace{0.6in}$\pzi{\Rj} \leftarrow \pzi{\Rj} \odot  \pz{R\lssmu}$ 

    % \State\hspace{0.4in}{\bf end for}
    
    % \State\hspace{0.4in}$\pz{\FK_j} \leftarrow \{ \pz{\Rj} ,  \pz{\pj} \}$ 
  
    
\State{\bf end for} %\hspace{0.2in}

% \State{\bf end parfor}

\end{algorithmic}
\caption{\small $\{\pzi{\FK_j}\,:\, j \in \Ne,\ i \in \Nt \} = \texttt{PZFK}(\{ \pzi{q_j} \,:\, j \in \Ne,\ i \in \Nt \})$}
\label{alg:compose_fk}
\end{algorithm}




% \State\hspace{0in}{\bf for} $j = 1:\nq$ %// for each joint

%     % \State\hspace{0.2in}$\pz{R_{j}^{j-1}}(\pzqji), \pz{\nom{p\jssmu}} \leftarrow \texttt{pzTransMat}(\pzi{q_j})$ 
    
    
    
% \State\hspace{0in}{\bf end for}

% % \State{\bf end parfor}

% \end{algorithmic}
% \caption{\small $\{\pz{\FK_j}(\pzqi)\,:\, j \in \Nq \} = \texttt{PZFK}(\pzqi)$}
% \label{alg:compose_fk}
% \end{algorithm}

==> Algorithms/pzfo.tex <==
%~~~~~~~~~~~~ Compose FK
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]

% \State{\bf parfor} $i \in \Nt$ %// parallel for each time step

\State{\bf for} $j = 1:\nq+1$ %// for each joint \hspace{0.2in}
    \State\hspace{0.2in}$\pzi{p_j} \leftarrow \pz{\mathbf{0}}$ %// initialize frame location 
        
    \State\hspace{0.2in}$\pzi{\R_j} \leftarrow \pz{I_{3 \times 3}}$ %// initialize frame orientation
    
     \State\hspace{0.2in}{\bf for} $l = 1:j$

        \State\hspace{0.4in}$\pzi{R\lssmu}, \pzi{\nom{p\lssmu}} \leftarrow \texttt{pzTransMat}(\pzi{q_j})$ 
    
        \State\hspace{0.4in}$\pzi{p_j} \leftarrow \pzi{p_j} \oplus \pzi{R_j} \odot \pzi{p_{l}^{l-1}}$
        
        \State\hspace{0.4in}$\pzi{R_j} \leftarrow \pzi{R_j} \odot  \pzi{R\lssmu}$ 

    \State\hspace{0.2in}{\bf end for}
    
    \State\hspace{0.2in}$\pzi{\FO_j} \leftarrow \pzi{p_j} \oplus  \pzi{R_j} \odot \pzi{L_j}$ 
  
    
\State{\bf end for} % \hspace{0.2in}

% \State{\bf end parfor}

\end{algorithmic}
\caption{\small $\{\pzi{\FO_j}\,:\, j \in \Ne,\ i \in \Nt \} = \texttt{PZFO}(\{ \pzi{q_j} \,:\, j \in \Ne,\ i \in \Nt \})$}
\label{alg:compose_fo}
\end{algorithm}

==> Algorithms/pzrnea2.tex <==
% \begin{algorithm}[t]
% \small
% \jon{fix long lines , double check $p_j^{j-1}$, fix $\nq$}
% \begin{algorithmic}[1]
% \State Compute $\pzqdai$ and $\pzqddai$ using \eqref{eq:pz_mod_err}
% \State Initialize base acceleration $a_0^0$.
% \State{\bf parfor} $i = 1:\nt$ // parallel for each time step

% \State\hspace{0.2in}Compute $\pzi{\dot{q}_a}$ and $\pzi{\ddot{q}_a}$ using \eqref{eq:modified_ref}.
% \State\hspace{0.2in}{\bf for} $j = 1:\nq$ %// for each joint
    
%     \State\hspace{0.4in}$\pz{R\jssmu}, \pz{\nom{p\jssmu}} \leftarrow \texttt{pzTransMat}(\pzqji)$   \Ram{this hasn't been defined.}
    
%     \State\hspace{0.4in} $\pz{R\jssm} \gets \texttt{pzTranspose}(\pz{R\jssmu})$
    
% \State\hspace{0.2in}{\bf end for}

% \State\hspace{0.2in}{\bf for} $j = 1:\nq$ %// for each joint (start of forward recursion)

%     \State\hspace{0.4in} $\pzi{\omega\jss} \gets \pzi{R\jssm} \bigodot \pzi{\omega\jssmm} \bigoplus \pzi{\qdj}\zj$
    
%     \State\hspace{0.4in} $\pz{\omega\jssa} \gets \pz{R\jssm} \bigodot \pz{\omega\jssmma} \bigoplus \pz{\qajdot}\zj$
    
%     \State\hspace{0.4in} $\pz{\dot{\omega}\jss} \gets \pz{R\jssm} \bigodot \pz{\dot{\omega}\jssmm} \bigoplus ((\pz{R\jssm} \bigodot \pz{\omega\jssmma}) \bigotimes \newline \hspace*{7em}  \bigotimes  (\pz{\qdj} \zj)) \bigoplus \pz{\ddot{q}_{a,j}}\zj$
    
%     % \State\hspace{0.4in} $\pz{a\jss} \gets (\pz{R\jssm} \bigodot \pz{a\jssmm}) \bigoplus (\pz{\dot{\omega}\jss} \bigotimes \pz{p\jssmj}) \bigoplus (\pz{\omega\jss} \bigotimes (\pz{\omega\jssa} \times \pz{p\jssmj}))$
    
%         \State\hspace{0.4in} $\pz{a\jss} \gets (\pz{R\jssm} \bigodot \pz{a\jssmm}) \bigoplus (\pz{\dot{\omega}\jss} \bigotimes \pz{p\jssmu}) \bigoplus  \newline \hspace*{7em}  \bigoplus (\pz{\omega\jss} \bigotimes (\pz{\omega\jssa} \times \pz{p\jssmu}))$
    
    
%     \State\hspace{0.4in} $\pz{a\jssc} \gets \pz{a\jss} \bigoplus (\pz{\dot{\omega}\jss} \bigotimes \pz{c\jss}) \bigoplus  \newline \hspace*{7em}  \bigoplus  (\pz{\omega\jss} \bigotimes (\pz{\omega\jssa} \bigotimes \pz{c\jss})) $
    
%     \State\hspace{0.4in} $\pz{F\jss} \gets \pz{m_i} \bigodot \pz{a\jssc}$
    
%     \State\hspace{0.4in} $\pz{N\jss} \gets \pz{I\jss} \bigodot \pz{\dot{\omega}\jss} \bigoplus (\pz{\omega\jssa}  \bigotimes (\pz{I\jss} \bigodot \pz{\omega\jss})) $

% \State\hspace{0.2in}{\bf end for}

% \State\hspace{0.2in}Initialize $\pz{f^{\nq+1}_{\nq+1}}, \pz{n^{\nq+1}_{\nq+1}}, \pz{R^{\nq}_{\nq+1}}$ \Ram{more details}

% \State\hspace{0.2in}{\bf for} $j = \nq:-1:1$ %// for each joint (start of backward recursion)

% \State\hspace{0.4in} $\pz{f\jss} \gets (\pz{R\jssp} \bigodot \pz{f^{j+1}_{j+1}}) \bigoplus \pz{F\jss} $

% \State\hspace{0.4in} $\pz{n\jss} \gets (\pz{R\jssp} \bigodot \pz{n^{j+1}_{j+1}}) \bigoplus (\pz{c\jss} \bigotimes \pz{F\jss}) \bigoplus  \newline \hspace*{7em}  \bigoplus  (\pz{p\jssmj} \bigotimes (\pz{R\jssp} \bigodot \pz{f^{j+1}_{j+1}})) \bigoplus \pz{N\jss} $ 

% \State\hspace{0.4in} $\pz{\ujt} \gets \pz{n\jss} \bigodot z_j$

% \State\hspace{0.2in}{\bf end for}

% \State{\bf end parfor}
% \end{algorithmic}
% \caption{\small $\{\pz{\ujt}\,:\, j \in \Nq,\ i \in \Nt\} = \texttt{PZRNEA}(\pz{\qA}, \pzgreek{\Delta})$}
% \label{alg:PZRNEA}
% \end{algorithm}

% \texttt{PZRNEA}(\{ \pzqji, \pzqdji, \pzqdaji, \pzqddaji \,:\, j \in N_q,\ i \in N_t \}


\begin{algorithm}[t]
\small
\begin{algorithmic}[1]
\State Compute $\pzqdai$ and $\pzqddai$ using \eqref{eq:pz_mod_traj}
\State Initialize base acceleration $a_0^0$.
% \State{\bf parfor} $i = 1:\nt$ // parallel for each time step

% \State\hspace{0.2in}Compute $\pzi{\dot{q}_a}$ and $\pzi{\ddot{q}_a}$ using \eqref{eq:modified_ref}.
\State\hspace{0in}{\bf for} $j = 1:\nq$ %// for each joint
    
    \State\hspace{0.2in}$\pz{R\jssmu}, \pz{\nom{p\jssmu}} \leftarrow \texttt{pzTransMat}(\pzqji)$   \Ram{this hasn't been defined.}
    
    \State\hspace{0.2in} $\pz{R\jssm} \gets \texttt{pzTranspose}(\pz{R\jssmu})$
    
\State\hspace{0in}{\bf end for}

\State\hspace{0in}{\bf for} $j = 1:\nq$ %// for each joint (start of forward recursion)

    \State\hspace{0.2in} $\pz{\omega\jss} \gets \pz{R\jssm}  \pz{\omega\jssmm} \bigoplus \pz{\qdj}\hat{z}_j$
    
    \State\hspace{0.2in} $\pz{\omega\jssa} \gets \pz{R\jssm}  \pz{\omega\jssmma} \bigoplus \pz{\qajdot}\hat{z}_j$
    
    \State\hspace{0.2in} $\pz{\dot{\omega}\jss} \gets \pz{R\jssm}  \pz{\dot{\omega}\jssmm} \bigoplus ((\pz{R\jssm}  \pz{\omega\jssmma}) \bigotimes (\pz{\qdj} \hat{z}_j)) \bigoplus \pz{\ddot{q}_{a,j}}\hat{z}_j$
    
    % \State\hspace{0.2in} $\pz{a\jss} \gets (\pz{R\jssm}  \pz{a\jssmm}) \bigoplus (\pz{\dot{\omega}\jss} \bigotimes \pz{p\jssmj}) \bigoplus (\pz{\omega\jss} \bigotimes (\pz{\omega\jssa} \times \pz{p\jssmj}))$
    
        \State\hspace{0.2in} $\pz{a\jss} \gets (\pz{R\jssm}  \pz{a\jssmm}) \bigoplus (\pz{\dot{\omega}\jss} \bigotimes \pz{p\jssmu}) \bigoplus (\pz{\omega\jss} \bigotimes (\pz{\omega\jssa} \times \pz{p\jssmu}))$
    
    
    \State\hspace{0.2in} $\pz{a\jssc} \gets \pz{a\jss} \bigoplus (\pz{\dot{\omega}\jss} \bigotimes \pz{c\jss}) \bigoplus (\pz{\omega\jss} \bigotimes (\pz{\omega\jssa} \bigotimes \pz{c\jss})) $
    
    \State\hspace{0.2in} $\pz{F\jss} \gets \pz{m_i}  \pz{a\jssc}$
    
    \State\hspace{0.2in} $\pz{N\jss} \gets \pz{I\jss}  \pz{\dot{\omega}\jss} \bigoplus (\pz{\omega\jssa}  \bigotimes (\pz{I\jss}  \pz{\omega\jss})) $

\State\hspace{0in}{\bf end for}

\State\hspace{0in}Initialize $\pz{f^{\nq+1}_{\nq+1}}, \pz{n^{\nq+1}_{\nq+1}}, \pz{R^{\nq}_{\nq+1}}$ \Ram{more details}

\State\hspace{0in}{\bf for} $j = \nq:-1:1$ %// for each joint (start of backward recursion)

\State\hspace{0.2in} $\pz{f\jss} \gets (\pz{R\jssp}  \pz{f^{j+1}_{j+1}}) \bigoplus \pz{F\jss} $

\State\hspace{0.2in} $\pz{n\jss} \gets (\pz{R\jssp}  \pz{n^{j+1}_{j+1}}) \bigoplus (\pz{c\jss} \bigotimes \pz{F\jss}) \bigoplus  \newline \hspace*{7em}  \bigoplus  (\pz{p\jssmj} \bigotimes (\pz{R\jssp}  \pz{f^{j+1}_{j+1}})) \bigoplus \pz{N\jss} $ 

\State\hspace{0.2in} $\pz{u}_j(\pzqAi, \intparams) \gets \hat{z}_j^\top \pz{n\jss}$

\State\hspace{0in}{\bf end for}

% \State{\bf end parfor}
\end{algorithmic}
\caption{\small \phantom{stupid stupid stupid stupid stupid stupid stupid} $\{ \pz{u}_j(\pzqAi, \intparams) \,:\, j \in \Nq\} = \texttt{PZRNEA}(\pzqAi, \intparams , a_0^0)$}
\label{alg:PZRNEA}
\end{algorithm}


==> Algorithms/rnea.tex <==
\begin{algorithm}[t]
\jon{define makeHomTrans, double check $p_j^{j-1}$}
\small
\begin{algorithmic}[1]
\State{\bf parfor} $t \in T$ // parallel for each time step

\State\hspace{0.2in}{\bf for} $j = 1:\nq$ // for each joint
    
    \State\hspace{0.4in} $\nom{R\jssmu}, p\jssmu \gets \texttt{TransMat}(\nom{\qj})$ 
    
    \State\hspace{0.4in} $\nom{R\jssm} \gets \texttt{transpose}(\nom{R\jssmu})$
    
\State\hspace{0.2in}{\bf end for}

\State\hspace{0.2in}{\bf for} $j = 1:\nq$ // for each joint (start of forward recursion)

    \State\hspace{0.4in} $\nom{\omega\jss} \gets \nom{R\jssm} \bigodot \nom{\omega\jssmm} \bigoplus \nom{\qdj}\xi$
    
    \State\hspace{0.4in} $\nom{\omega\jssa} \gets \nom{R\jssm} \bigodot \nom{\omega\jssmma} \bigoplus \nom{\qajdot}\xi$
    
    \State\hspace{0.4in} $\nom{\dot{\omega}\jss} \gets \nom{R\jssm} \bigodot \nom{\dot{\omega}\jssmm} \bigoplus ((\nom{R\jssm} \bigodot \nom{\dot{\omega}\jssmm}) \bigotimes (\nom{\qdj} \xi)) \bigoplus \nom{\qddj}\xi$
    
    \State\hspace{0.4in} $\nom{a\jss} \gets (\nom{R\jssm} \bigodot \nom{a\jssmm}) \bigoplus (\nom{\dot{\omega}\jss} \bigotimes \nom{p\jssmj}) \bigoplus (\nom{\omega\jss} \bigotimes (\nom{\omega\jssa} \times \nom{p\jssmj}))$
    
    \State\hspace{0.4in} $\nom{a\jssc} \gets \nom{a\jss} \bigoplus (\nom{\dot{\omega}\jss} \bigotimes \nom{c\jss}) \bigoplus (\nom{\omega\jss} \bigotimes (\nom{\omega\jssa} \bigotimes \nom{c\jss})) $
    
    \State\hspace{0.4in} $\nom{F\jss} \gets \nom{m_i} \bigodot \nom{a\jssc}$
    
    \State\hspace{0.4in} $\nom{N\jss} \gets \nom{I\jss} \bigodot \nom{\dot{\omega}\jss} \bigoplus (\nom{\omega\jssa}  \bigotimes (\nom{I\jss} \bigodot \nom{\omega\jss})) $

\State\hspace{0.2in}{\bf end for}

\State\hspace{0.2in}Initialize $\nom{f^{\nq+1}_{\nq+1}}, \nom{n^{\nq+1}_{\nq+1}}, \nom{R^{\nq}_{\nq+1}}$

\State\hspace{0.2in}{\bf for} $j = \nq:-1:1$ // for each joint (start of backward recursion)

\State\hspace{0.4in} $\nom{f\jss} \gets (\nom{R\jssp} \bigodot \nom{f^{j+1}_{j+1}}) \bigoplus \nom{F\jss} $

\State\hspace{0.4in} $\nom{n\jss} \gets (\nom{R\jssp} \bigodot \nom{n^{j+1}_{j+1}}) \bigoplus (\nom{c\jss} \bigotimes \nom{F\jss}) \bigoplus (\nom{p\jssmj} \bigotimes (\nom{R\jssp} \bigodot \nom{f^{j+1}_{j+1}})) \bigoplus \nom{N\jss} $ 
\State\hspace{0.4in} $\nom{\ujt} \gets z_j^\top \nom{n\jss} $

\State\hspace{0.2in}{\bf end for}

\State{\bf end parfor}
\end{algorithmic}
\caption{\small $\{\nom{\ujt}\,:\, j \in \Nq,\ t\in T\} = \texttt{RNEA}(\nom{\q},\nom{\qd}, \nom{\qadot}, \nom{\qdd}, \nom{\Delta})$ }
\label{alg:RNEA}
\end{algorithm}

==> Sections/00_outline.tex <==
\section*{Outline}
\begin{outline}[enumerate]

\1 Introduction

    \2 Background and Motivation
    
        \3 Introduce the waiter motion problem as a non-prehensile manipulation task which requires persistently feasible trajectories that are robust to uncertainty. \Parker{Start with something higher-level. Maybe discuss prehensile motion generally, then more specifically the waiter problem.}
        
        \3 The use of reachability analysis enables construction of overapproximations of the forces (accelerations) applied to the object(s) being manipulated which can be used to ensure persistent feasibility. 
        
        \3 This work describes the extension of the reachability-based approaches in (RTD Paper) and (U-ARMTD Paper) to include constraints on the forces applied by the end effector, which enables a novel method of addressing the waiter motion problem. \Parker{Can you also say it is  applicable to non-prehensile motion more broadly, with the waiter problem as an example?}
        
        \3 Figure: general overview figure of robot arm moving a tray and cup through a trajectory
        
        \begin{figure}
            \centering
            \includegraphics[width=0.9\columnwidth]{Figures/ARMTD_Force_Generic_Diagram_v1.jpg}
            \caption{Caption}
            \label{fig:GenericDiagram}
        \end{figure}
        
    \2 Related Work
    
        \3 There is a body of literature focusing on this task, which developed time-optimal motions along a predefined trajectory. Review what constraints they enforce, how they are enforced and whether they can be persistently feasible. \Ram{this work needs to be much better organized. Like what are the properties for algorithms we care about and can we arrange the related work according to the relevant criteria in some way}
        \Zac{I can continue looking and reading. I think the properties we care about are persistent feasibility and how their algorithms discretize, what constraints they are enforcing, and performance.}
        \Parker{Is there a more general non-prehensile review paper you could cite, like \cite{ruggiero2018nonprehensile}?}
        
            \4 Waiter Motion Papers: Around 5 papers so far that I can cite here, they focus on time-optimal paths of predetermined trajectories and only worry about constraints ensuring loosely placed object doesn’t move. Some have only friction constraints. Doesn’t seem like any are real time. One incorporates uncertainty and using learning based approach to tighten bounds iteratively. 
            
            \4 GOMP Papers and other Trajectory planning under constraints based on grasping papers. GOMP papers focus on generating time-optimal trajectories under end-effector acceleration constraints. Need to take a closer look at how they discretize and enforce safety between time steps. GOMP-FIT acceleration constraint doesn’t work in every scenario? They also explicitly mentioned at ICRA that their method doesn’t account for wrench on grasped object. GOMP-ST uses learning to form an acceleration constraint to prevent delamination of a suction cup gripper. Use trajopt to generate waypoints.
            
        \3 Method of modeling objects. We use a RNEA while treating the object(s) as part of the robot. What do other people do?
        
    \2 Contributions and Overview of Proposed Method
    
        \3 Extension of ARMTD framework to include constraints on wrench applied by end-effector which ensure a loosely placed object has no motion relative to the supporting surface. \Parker{Maybe rephrase this? It doesn't sound as good as saying you introduce a method for solving the waiter problem in a recursively feasible manner while accounting for uncertainty. The paper so far seems to be focusing on the waiter problem, so your contribution should be framed in terms of this problem as well.}
        
        \3 Simulation results of method with loosely placed object(s) \Parker{Both this and the next point are not contributions so much as proving that your first contribution actually works.}
        
        \3 Hardware demonstration of method working?
        
\1  \Ram{we need a preliminary section where you define all relevant notation. }

\input{Sections/Symbols}

\subsection{Notation}
\Parker{Include things here like inner product, matrix notation, vectors as column vectors, bounds, set notation, etc. You may also be able to introduce some symbols such as the generalized coordinates.}
        
\1 Modeling of Contact Interactions


    \2 Figure: diagram of cup and tray with the relevant wrench and dimensions indicated along with a reference frame.
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\columnwidth]{Figures/ARMTD_Force_Contact_Diagram_v1.jpg}
        \caption{Caption}
        \label{fig:my_label}
    \end{figure}
    
    \2 Describe the assumptions about the robot properties and dynamics. Things like inertia and the trajectories and forward occupancy.
    
    \begin{assum}
   The robot operates in a three dimensional workspace, which we denote $W \subset \R^3$.
    The robot arm is composed of only revolute joints, where the $j$\ts{th} joint actuates the robot's $j$\ts{th} link.
    \Ram{this sentence should live outside of the assumption box because it isn't an assumption its an observation.}Note that joints with multiple degrees of freedom may be represented in this framework using links with zero length.
    The robot's $j$\ts{th} joint has position and velocity limits given by $\qj \in [\qlim^-, \qlim^+]$ and $\qdj \in [\dqlim^-, \dqlim^+]$ for all $t \in T$, respectively.
    The robot is fully actuated, where the robot's input $u: T \to \R^{\nq}$ \Parker{what are the inputs, torques? If so maybe the symbol for torques?} has limits that are given by $u(t) \in [\ulim^-, \ulim^+]$ for all $t \in T$.
    The robot is gripping a tray and can maintain force closure throughout its motion. 
    On the tray is object and the tray's coefficient of static friction is $\mu_s$. 
    \end{assum}
    
    \2 Describe the task and the constraints that we are seeking to enforce. We wish to prevent relative motion of the object and tray, which can occur when the object separates \Parker{Unsure what separates means, maybe define the types of motion the object can take in specific terms?}, slides or tips over. 
    
    \2 Optimization Problem Solved During Each Planning Iteration 
    
        \3 Continuous time optimization problem formulation from write up \Parker{Maybe make constraints (5)-(8) words or general functions rather than equations, since you introduce none of the notation for them at this point. Additionally, you should move this up to point C., state this is the problem you are solving to compute inputs u(t) which are used to generate trajectories q(t). Then jump into the properties these trajectories need to satisfy.}
        
        \begin{align}
            \label{eq:optcost}
            &\underset{u}{\min} &&\texttt{cost}(u, q_{goal}) \\
            \label{eq:optpos}
            &s.t. && \qj \in [\qlim^-, \qlim^+]  &\forall t \in T, j \in \Nq \\
            \label{eq:optvel}
            &&& \qdj \in [\dqlim^-, \dqlim^+]  &\forall t \in T, j \in \Nq \\
            \label{eq:opttorque}
            &&& \ujt \in [\ulim^-, \ulim^+]  &\forall t \in T, j \in \Nq \\
            % \label{eq:optposcon}
            % &&& \pjt \in [p_j^-, p_j^+]  &\forall t \in T, j \in \Nq \\
            % \label{eq:optorncon1}
            % &&& \hat{z}_{d,j}^{T} \hat{z}_{j}(t) \geq z_{d,j}^-  &\forall t \in T, j \in \Nq \\
            % \label{eq:optorncon2}
            % &&& \hat{x}_{d,j}^{T} \hat{x}_{j}(t) \geq x_{d, j}^-  &\forall t \in T, j \in \Nq \\
            \label{eq:optcolcon}
            &&& \FO_j(q(t)) \bigcap \obsset = \emptyset  &\forall t \in T, j \in \Nq \\
            \label{eq:optsepcon}
            &&& -1*\FNorm \le 0 &\forall t \in T, j \in \Nq \\
            \label{eq:optslipcon}
            &&& |\FTan| - \mu_{s}|\FNorm| \le 0 &\forall t \in T, j \in \Nq \\
            \label{eq:opttipcon}
            &&& ||\ZMP|| - \objrad \le 0 &\forall t \in T, j \in \Nq
        \end{align}
        
        \noindent where $r$ is the radius of the contact patch (assumed to be a circular contact patch)
    
    \2 
    
    \begin{defn}
    A trajectory \q is safe \Ram{is safe the right word?} if it satisfies the following conditions for all time
    \begin{enumerate}
        \item the normal force $\FNorm$ is always positive in the end-effector frame.
        \item the magnitude of the tangential force $\FTan$ does not exceed the magnitude of the normal force $\FNorm$ multiplied by the coefficient of static friction $\mu_s$ \Parker{maybe be more explicit here that the forces are in the end-effector frame}. \Zac{I think where I end up introducing $\FTan$ and $\FNorm$ first, I will specify this, will also be clear in figure hopefully}
        \item the Zero Moment Point (\ZMP) does not leave the convex hull of the contact area.
    \end{enumerate}
    \end{defn}
    
    \2 Describe what modeling choices are made to capture the interaction forces between a loosely placed object and a tray the robot is manipulating. This is where I want to introduce that we are using RNEA to calculate the interaction wrench. We treat the interaction as 6 joints with zero length to achieve 6-DOF motion and use RNEA to calculate the forces and moments applied to those joints.
    
    \2 \Ram{may want to explain why solving this problem is difficult}
    
    \2 Difficulties with solving this problem arise due trying to ensuring persistent feasibility, which may not be possible with other methods, or when dealing with uncertainty in parameters like friction or inertia properties of the object being manipulated.
    
    
    \2 Explain that the goal is to use polynomial zonotope representations to overapproximate the wrench and therefore the constraints, while also dealing with uncertainty in variables like the mass, dimensions, inertia and coefficient of friction. 

\1 Trajectory Design

    
    \2 \Parker{Add why this is needed. You could simply solve for your q(t) at each discrete time step, but just because the constraints are satisfied at each point doesnt mean they are satisfied between points. Therefore you use RTD which parameterizes trajectories...} \Zac{probably talk about this later when describing how they are overapproximated using PZs} Describe the space of trajectories that are optimized over at run-time to safely move the robot between configurations.
    
    \2 Describe the important components of a desired trajectory, such as a trajectory parameter $k \in K$ which uniquely determines its corresponding trajectory, a braking maneuver which ensures that the system can safely come to a stop, and that the reference position, velocity and acceleration trajectories are continuous. 
        
        \3 Definition of a desired trajectory:
    
        \begin{defn}
        \label{def:traj_param}
        For each $k \in K$, a \emph{desired trajectory} is a function $q_d(\cdot; k) : T \to \Q$ that satisfies the following properties:
        
        \begin{enumerate}
        
        \item The trajectory starts at a specified initial condition $(\initq, \initdq, \initddq)$, so that $q_d(0; k) = \initq$, $\dot{q}_d(0; k) = \initdq$, and $\ddot{q}_d(0; k) = \initddq$.
        
        \item $\dot{q}_d(\tfin; k) = 0$ and $\ddot{q}_d(\tfin; k) = 0$ (i.e., each trajectory brakes to a stop, and at the final time has zero velocity and acceleration).
        
        \item $\ddot{q}_d(\cdot; k)$ is Lipschitz continuous and bounded.
        
        \end{enumerate}
        \end{defn}
        
    
\1 Controller Design

    \2 This section describes the passivity-based controller and how the TRO paper develops ultimate bounds on tracking performance.

    \2 Theoretical Overview
    
        \3 Describe the nominal controller and how it does not guarantee perfect tracking since error can arise due to mismatches between the nominal and true parameters of the system.
        
        \3 Useful inclusions from the T-RO paper:
        
            \4 Nominal controller:
            \begin{equation}\label{eq:nominal_controller}
            \nominal,
            \end{equation}
            
            \4 Modified reference velocity and acceleration trajectories:
            \begin{align}\label{eq:modified_ref} % modified error
            \qakdot &= \qdeskdot + K_r \err, \Hquad          \err = \qdesk - \q \\
            \qakddot &= \qdeskddot + K_r \errdot,            \Hquad \errdot = \qdeskdot - \qd.
            \end{align}

            \4 Total control input:
            \begin{equation}\label{eq:controller}
            \controller,
            \end{equation}
        
        \3 Short paragraph about how the T-RO U-ARMTD paper developed a robust controller and it is used in this paper as well. The main results are that given uncertainty in the inertial properties of the robot, the tracking error is uniformly and ultimately bounded. \Parker{Does this extend to uncertainty in the properties of the object placed on the tray?}
        
        \3 Useful inclusions from the T-RO paper:
        
            \4 \begin{defn}\label{def:worst_case_disturbance}
            Let $\mathbb{I}\mathbb{R}^{n_q}$ be the set of all real-valued interval vectors.  
            The \emph{measure of worst case disturbance} is the function $\rho: \mathbb{I}\mathbb{R}^{n_q} \xrightarrow{} \mathbb{R}^{n_q}$ which is defined as
            \begin{equation}
                \rho([\wdistinterval]) = \max(|\underline{\wdistinterval}|, |\overline{\wdistinterval}|)\label{eq:worst_case_disturbance},
            \end{equation}
            where the max$(\cdot)$ operator is applied element-wise over the interval vector.
            \end{defn}
            
            \4 
            \begin{prop}\label{thm:eigenvalue_bound}
            Let $\intparams$ be an interval of inertial parameters.
            % and let $[\bM] = [\bM(\cdot,\underline{\trueparams}), \bM(\cdot,\overline{\trueparams})]$ be the interval of corresponding inertia matrices. 
            Define $\lambdamin(\bM(\q,\trueparams))$ and $\lambdamax(\bM(\q,\trueparams))$ to be the minimum and maximum eigenvalues of $\bM(\q,\trueparams)$, respectively.
            % Let $\sigma_{m}(\trueparams)$ and $\sigma_{M}(\trueparams)$ be uniform bounds on the eigenvalues of $\bM(\cdot, \trueparams)$ \cite{Ghorbel1998uniform}.
            There exist ultimate bounds $\sigma_m$ and $\sigma_M$ on the eigenvalues of the mass matrix so that
            \begin{align}
                \sigm &\leq \lambdamin(\Mq)\\
                \sigM &\geq \lambdamax(\Mq)
            \end{align}
            holds for all $\q \in Q$ and $\trueparams \in \intparams$ \cite{Ghorbel1998uniform}.
            % Let $\sigma_{m}(\trueparams)$ and $\sigma_{M}(\trueparams)$ be uniform bounds on the eigenvalues of $\bM(\q, \trueparams)$ for all $\q \in Q$ \cite{Ghorbel1998uniform}.
            % Then for all $\trueparams \in \intparams$ and $\q \in Q$ we have
            % \begin{align}
            %     \sigma_{m}(\underline{\trueparams}) &\leq \lambdamin(\Mq)\\
            %     \sigma_{M}(\overline{\trueparams}) &\geq \lambdamax(\Mq).
            % \end{align}
            \end{prop}
            
            \4
            \begin{thm}
            \label{thm:robust_controller}
                % \pat{Robust input gives ultimate bound $\norm{\robr} \leq \ultbound \, \forall t > t_1$. Need to rearrange so these terms are introduced before the proof}
                Let $\roblevel > 0$ be a user-specified maximum value of the candidate Lyapunov function
                \begin{equation}
                    \label{eq:lyap_r}
                    \roblyap = \frac{1}{2}\robr^\top \Mq \robr.
                \end{equation}
                and, define 
                \begin{equation}
                    \label{eq:CBF_defn}
                    \robh = -\roblyap + \roblevel.
                \end{equation}
                Next, let 
                \begin{equation}
                    \label{eq:CBF_lower_bound}
                    \robhmin \coloneqq \inf_{\trueparams^* \in \intparams}\left(-\frac{1}{2}\robr^\top M(q, \trueparams^*) \robr \right) + \roblevel,
                \end{equation}
                and therefore $\robhmin \leq \robh$ for all $\q \in Q$ and $\robr \in \R^{n_q}$.
                \shrey{It seems bits of the proof have leaked into this theorem statement}
                For brevity, we define $\normwmax = ||\rho([\wdistinterval])||$.
                Finally, let $\robKinf:\R \to \R$ be some extended class $\mathcal{K}_\infty$ function (i.e., $\robKinf: \R \to \R$ is strictly increasing with $\robKinf(0) = 0$ and is defined on the entire real line $\R = (-\infty, \infty)$.
                
                Then, the robust input
            \begin{equation}
                \label{eq:robust_input}
                \robv = -\robcoeff \frac{\robr}{\norm{\robr}}
            \end{equation}
            with
            \begin{equation}
                \label{eq:robust_coeff}
                \robcoeff = \max\left(0, \frac{-\robKinf(\robhmin)}{\norm{\robr}} + \normwmax\right)
            \end{equation}
            ensures the modified tracking error trajectories $\robrnot$ are uniformly ultimately bounded:
            \begin{equation}
                \norm{\robr} \leq \ultbound \qquad \forall t \geq 0
            \end{equation}
            when tracking reference trajectories that satisfy Def. \ref{def:traj_param}.
            
            \end{thm}
            
            \4
            % as a corollary, the tracking error is uniformly bounded
            \begin{cor}\label{cor:tracking_error}
            If $\robrnot$ is ultimately bounded, then the complete controller \eqref{eq:controller} with robust input \eqref{eq:robust_input} reaches any desired tracking performance provided a large enough gain matrix $K_r$.
            In particular, letting
            \begin{align}
                \pbound &\coloneqq \frac{1}{K_r}\ultbound \label{eq:ultimate_bound_position}\\
                \vbound &\coloneqq 2\ultbound,\label{eq:ultimate_bound_velocity}
            \end{align}
            \pat{@jon might need your help proving these...}
            we have that $|\errj| \leq \pbound$ and $|\errjdot| \leq \vbound$ for all time.
            \end{cor}
        
    \2 Numerical Implementation
    
        \3 Describe the numerical implementation of RNEA and IRNEA which are used to compute the robust input to the controller, as well as the contact forces for the waiter motion constraints.
    
\1 Planning Algorithm Theory
    
    \2 Overview paragraph: Explain how planning is performed in receding horizon fashion and that each trajectory is certifiably safe. Real time planning is achieved through planning for the next iteration while the current iteration is executing, and we make use of a braking maneuver to ensure safety \Parker{if a new plan cannot be computed in time. Thus, this method is recursively feasible}. 

    \2 Outline the execution of a single planning iteration, including if braking occurs. Go over all the components of the optimization problem solved during the planning iteration. \Zac{move last sentence closer to opt prob?}
        

    \2 Describe our approach: Generating polynomial zonotope overapproximations of the trajectory and all of the constraints enables fast optimization that also ensures safety.  Highlight the other benefits of this method.
    
    \2 Trajectory Overapproximation
    
        \3 Overview is to describe how a trajectory is overapproximated. 
        
        \3 First, describe how a planning time interval is overapproximated. 
        
        \begin{equation}
                \label{eq:time_pz}
                \pzi{T} = \frac{(i-1) + i}{2}\timestep + \frac{1}{2} \timestep \tvar
        \end{equation}  
        with indeterminate $\tvar \in \iv{-1, 1}$.
        
        \3 Give definition of trajectory parameter and how the space of trajectory parameters relates to the desired trajectories.
        
        \begin{defn}
        \label{def:pz_Kj}
        We represent the interval $\Kj$ as a poynomial zonotope $\pz{\Kj} = \kjvar$ where $\kjvar \in \iv{-1, 1}$ is an indeterminate.
        Any particular choice of $k_j$ is trivially related to the corresponding subset $k_j = \texttt{slice}(\pz{\Kj}, \kjvar, k_j)$.
        Letting $\kvar = (x_{k_1}, x_{k_2}, ..., x_{k_{\nq}})^\top$ we introduce the shorter notation $\pz{\ \cdot \ ; k} = \texttt{slice}(\pz{\ \cdot \ }, \kvar, k)$, which allows us to obtain subsets of polynomial zonotopes corresponding to a choice of $k$ by slicing the corresponding $\kvar$ indeterminates.
        \end{defn}
        
        
        
        \3 Describe construction of overapproximation of desired trajectory and how the overapproximated trajectory ensures that the continuous time trajectory lies within.  
        
        \3 \begin{lem}
        Overapproximative polynomial zonotope representations of the desired trajectory $\qdeskj$ can be formed by using $\pzi{T}$ and $\pz{\Kj}$ in the arguments of the functions. 
        The resulting polynomial zonotope $\pzqdesji$ satisfies
        \begin{equation}
            \qdeskj \in \pzi{\qdesk} \quad \forall t \in \pzi{T}, \kj \in \pz{\Kj}
        \end{equation}
        Overapproximative polynomial zonotope representations are similarly constructed for $\pzqddesji$ and $\pzqdddesji$.
        \end{lem}
        
        
        \3 Describe how slicing a polynomial zonotope representing the trajectory parameters can be used to recover the trajectory it parameterized.
        
        \3 \Zac{slice algorithm is given in ARMTD paper. add small section about it in a preliminaries maybe?}
        
        Given an indeterminate $\pzv_s$ and a value $\sigma \in [-1, 1]$, slicing yields a subset of $\pz{P}$ by plugging $\sigma$ into the specified element $\pzv_s$:
        \begin{equation}
            \texttt{slice}(\pz{P}, \pzv_s, \sigma) \subset \pz{P} = \{ z \in \pz{P} \, \mid \, z = \sum_{i=0}^{\pzn} \pzgi \pzv ^{\pzei}, \, \pzv_s = \sigma \}.
        \end{equation}
        
    \2 Reachable Set Construction
    
        \3 Describe how the overapproximated joint trajectories are used in the computation of arm kinematics and dynamics.
        
        \3 Forward Kinematics Reachable Set
            
            \4 describe how the polynomial zonotope overapproximation of the joint trajectories is used to calculate the polynomial zonotope overapproximation of the forward kinematics of the robot.
            
            \4 give regular FK to motivate need for sine and cosine overapproximations?
            
            \4 \Zac{theorem that sin and cos of pzs are also overapproximative. Taylor expansion and overapproximate the remainder?}
        
            \4 \begin{thm}
            The sine and cosine of a polynomial zonotope can be overapproximated by computing a Taylor expansion series with an overapproximated Lagrange Remainder.
            \end{thm}
        
            \4 polynomial zonotope forward kinematics for the $j^{th}$ frame at the $i^{th}$ timestep:
            \begin{equation}\label{eq:pzfk_j}
                \pzi{\FK_j} = 
                \begin{bmatrix} \pzi{R_j} & \pzi{p_j}\\
                \mathbf{0}  & 1 \\
                \end{bmatrix},
            \end{equation}
            where
            \begin{equation}
                \pzi{R_j} = \prod_{l=1}^{j} \pzi{R_{l}^{l-1}}
            \end{equation}
            and
            \begin{equation}
                \pzi{p_j} = \sum_{l=1}^{j} \pzi{R_l} \pzi{p_{l}^{l-1}}.
            \end{equation}
            

            
            \4 
            \begin{thm}
            \label{thm:FK_overapprox}
            Given that $sin(\pz{q_i})$ and $cos(\pz{q_i})$ are overapproximative, then $\pz{\FK}$ is an overapproximation of the forward kinematics of the robot, i.e. $\FK_{j,i} \in \pzji{\FK} \quad \forall \pzi{T}$.
            \end{thm}
            
        \3 Forward Occupancy Reachable Set
        
            \4 The forward occupancy is overapproximated using the overapproximated forward kinematics. This is used to ensure the robot does not collide with obstacles in the environment.
            
            \4 \Zac{need to add how $\pz{L_j}$ is constructed. is this just using the CORA toolbox?}
            
            \4 
            \begin{align}\label{eq:pz_forward_occupancy_j}
                 \pzi{\FO_j} = \pzi{p_j} \oplus \pzi{R_j} \odot \pz{L_j}.
            \end{align}
            
            
            \4 
            \begin{thm}
            Given that $\pzi{p_j}$, $\pzi{R_j}$ and $\pz{L_j}$ are overapproximations, then $\FO_{j,i} \in \pzi{\FO_j} \quad \forall t \in \pzi{T}$.
            \end{thm}

        \3 Input Reachable Set
        
            \4 Describe the construction of an overapproximation of the input. (This comes from the T-RO paper)
            
            \4 The nominal control input is overapproximated 
            
            \begin{equation}
                \label{eq:pz_nominal_input}
                \pzi{\tau} = \bM(\pzi{q}, \nomparams) \pzi{\ddot{q}_a} + \bC(\pzi{q}, \pzi{\dot{q}},\nomparams) \pzi{\dot{q}_a} + \bG(\pzi{q}, \nomparams).
            \end{equation}
            
            \4 Theorem that $\norm{\robv}$ is bounded:
            
            \begin{thm}
            The norm of the robust input $\norm{\robv}$ at the $i$\ts{th} timestep is bounded by
            \begin{equation}
                \label{eq:pz_robust_input_bound}
               \norm{\robv} \leq \frac{-\robKinf(\texttt{inf} \pzi{h})}{\ultbound} + \norm{\rho(\pzi{w})}
            \end{equation}
            for all $(q, \robr) \in \robH$, where $\pzi{h}$ and $\pzi{w}$ are polynomial zonotope versions of the CBF $h$ and disturbance $\wdist$ respectively.
            \end{thm}
            
            \4 Final result is that the robust input $\pzi{u}$ is overapproximated: 
            \begin{equation}
            \label{eq:pz_input}
                \pzi{u} = \pzi{\tau} - \pzi{v}.
            \end{equation}
            
            \4 \begin{thm}
            Given that $\pzi{\tau}$ and $\pzi{v}$ are overapproximations, the control input $\pzi{u}$ is overapproximated.
            \end{thm}
            
        \3 End Effector Wrench Reachable Set
        
            \4 Describe the construction of an overapproximation of the end effector wrench. This is done through using PZ-RNEA and the overapproximated joint trajectories. (Likely need a theorem/proof stating that this method does result in an overapproximated wrench?)
            
            \4 \begin{thm}
            Given $\pz{\q}$, $\pz{\qd}$, $\pz{\qadot}$, $\pz{\qdd}$, and $\pz{\Delta}$ are overapproximative, then algorithm \ref{alg:PZRNEA} results in an overapproximation of the wrench $[\pz{f\jss},  \pz{n\jss}]^{T}$ exerted on joint $j$.
            \end{thm}
            
            \Zac{Note: need to update PZ-RNEA algorithm with the wrench output}
            
            
    \2 Constraint Generation
    
        \3 Describe how the constraints are written using the reachable sets. 
        
            \4 Separation constraint is the Fz related component of the contact wrench. \Zac{need to add notation for specifying axial component of force}.
            
            \4 Friction constraint is rewritten to involve only summation and multiplication operations.
            
            \4 Tipping constraint is rewritten to involve only summation and multiplication operations.
        
        
        \3 \begin{thm}
        Given $[\pz{f\jss},\pz{n\jss}]^{T}$, the constraints (will reference eqn numbers when added) are overapproximative.
        \end{thm}

    
    \2 Trajectory Optimization
    
        \3 Polynomial zonotope formulation of the optimization problem
        
        \begin{align}
            \label{eq:optcost}
            &\underset{k}{min} &&\texttt{cost}(k, q_{goal}) \\
            \label{eq:pz_optpos}
            &&& \pzqjki \subseteq [\qlim^-, \qlim^+] \qquad &\forall i, j \\
            \label{eq:pz_optvel}
            &&& \pzqdjki \subseteq [\dqlim^-, \dqlim^+] \qquad &\forall i, j \\
            \label{eq:pz_opttorque}
            &&& \pzujki \subseteq [\ulim^-, \ulim^+] \qquad &\forall i, j \\
            \label{eq:pz_optposcon}
            % &&& \pzki{p_j} \subseteq [p_j^-, p_j^+] \qquad &\forall i, j \\
            % \label{eq:pz_optorncon1}
            % &&& \pzi{\hat{z}_{j}; k} \odot \pzi{\hat{z}_{d,j}}  \geq z_{d, j}^- \qquad &\forall i, j \\
            % \label{eq:pz_optorncon2}
            % &&& \pzk{\hat{x}_{j}} \odot \pz{\hat{x}_{d,j}}  \geq x_{d, j}^- \qquad &\forall i, j \\
            \label{eq:pz_optcolcon}
            &&& \pzki{\FO_j} \bigcap \obsset = \emptyset \qquad &\forall i, j \\
            \label{eq:pz_optsepcon}
            &&& -1*\pzki{\FNorm} \le 0 &\forall i, j \\
            \label{eq:pz_optslipcon}
            % &&& \pzki{\FTan}*\pzki{\FTan} - {\mu_{s}}^2*\pzki{\FNorm}*\pzki{\FNorm} &\forall i, j \\
            &&& |\pzki{\FTan}| - {\mu_{s}}|\pzki{\FNorm}| \le 0 &\forall i, j \\
            \label{eq:pz_opttipcon}
            &&& |\pzki{\ZMP}| - r \le 0 &\forall i, j
            % \pzki{\MG}  \surfnorm - \pzki{\FG} \cdot \surfnorm * \objrad \le 0
        \end{align}
        \noindent where $i \in \Nt$ and $j \in \Nq$ and $r$ is the radius of the contact patch (assumed to be a circular contact patch). 
        
        
        \begin{thm}
        Any feasible solution to \ref{pz_optpos} parameterizes a trajectory that is collision free, satisfies input torque limits, and results in no relative motion between a loosely placed object and the end-effector of the robot over the time horizon $\pzi{T}$.
        \end{thm}

        
\1 Planning Algorithm Implementation

    \2 Trajectory Creation
        
        \3 Describe what trajectories are being used (currently constant acceleration), how they are parameterized and what their polynomial zonotope representations look like. 
    
    \2 FK, FO, and PZRNEA Algorithm Implementation
    
        \3 PZRNEA Algorithm:
        
        \input{Algorithms/pzfk}
        
        \input{Algorithms/pzfo}
        
        % \begin{align}
        %   &\pzi{u} = \texttt{PZRNEA}(\pzi{q}, \pzi{\dot{q}}, \pzi{\dot{q}_a}, \pzi{\ddot{q}_a}, \pz{\Delta}) \\
        %   &+ \pzi{-\robcoeff \frac{\robr}{\norm{\robr}}} \\
        %   &\jon{\text{how to express robust input?}} \\
        %   &\jon{\text{fix \texttt{PZRNEA} input}}
        % \end{align}
        \input{Algorithms/pzrnea}
    
    \2 Constraint Implementation
    
        \3 Collision Avoidance
        
            \4 Describe the collision constraint. The FO does not intersect any obstacle.
        
        \3 Torque Limits
        
        \3 End effector wrench constraints
        
            \4 Separation constraint: require that the normal force is greater than zero, i.e. the object does not separate from the tray.
            
            \4 Friction cone constraint: fundamental friction law is satisfied so no sliding occurs.
            
            \4 ZMP constraint: The ZMP point remains in the contact patch so no tipping occurs.
            
    \2 \Ram{you need to describe the gradients of the cost function and the constraints}
    
    \2 We analytically compute the gradients of the cost function and the constraints. Polynomial differentiation enables computing the gradients of the constraints. 

\1 Experiments 

    \2 One Object Simulation
        
        \3 Ran 100 trials with random initial/goal configurations. Expected results are:
            
            \4 ARMTD-Force
                \5 no failures
                \5 some safe stops
                \5 computation time: on the order of minutes for a single trajectory and 30 seconds for a single planning iteration.
            
            \4 GPOPS
                \5 might have failures
                \5 not sure how to do safe stops
                \5 computation time: on the order of hours to days for a single trajectory and hours for a single planning iteration.
                
    \2 Table of Simulation Results
    
    \begin{table}[]
        \centering
        \begin{tabular}{c|c c c}
             Optimization Method & Goals Reached & Crashes & Safe Stops \\
             \hline
             ARMTD-Force & 89 & 0 & 11 \\ 
             GPOPS & 50 & 50 & 0
        \end{tabular}
        \caption{Results for 100 random scenarios for two optimization methods, ARMTD-Force and GPOPS.}
        \label{tab:my_label}
    \end{table}
                
\1 Conclusion
    



\end{outline}

==> Sections/03_models_backup.tex <==
\section{Arm, Contact Wrench, and Environment} % Modeling of Contact Interactions
\label{sec:modeling}

The goal of this work is to plan safe trajectories for a serial manipulator which is manipulating a serving tray that is holding objects of uncertain weight and size. 
This section introduces a model of the manipulator and contact and concludes by describing the environment in which the robot is moving. 

\subsection{Extended Arm Model}

Given an $\nq$-dimensional serial robotic manipulator with configuration space $Q$ and a compact time interval $T \subset \R$ we define a trajectory for the configuration as $q: T \to Q \subset \R^{\nq}$. 
The velocity of this configuration trajectory is $\dot{q}: T \to \R^{\nq}$.
We make the following assumptions about the structure of the robot model:
\begin{assum}[Workspace and Configuration Space]
The robot operates in a three dimensional workspace, which we denote $W \subset \R^3$.
The robot is composed of only revolute joints, where the $j$\ts{th} joint actuates the robot's $j$\ts{th} link.
The robot's $j$\ts{th} joint has position and velocity limits given by $\qj \in [\qlim^-, \qlim^+]$ and $\qdj \in [\dqlim^-, \dqlim^+]$ for all $t \in T$, respectively.
During online operation, the robot has encoders that allow it to measure its joint positions and velocities.
Finally, the robot is fully actuated, where the robot's input $u: T \to \R^{\nq}$ has limits that are given by $u_j(t) \in [\ulim^-, \ulim^+]$ for all $t \in T$ and $j \in \{1,\ldots,\nq\}$. 
\end{assum}
\noindent Note that we make the one-joint-per-link assumption with no loss of generality because joints with multiple degrees of freedom (e.g., spherical joints) may be represented in this framework using links with zero length.
In addition, this work can be extended to robots with prismatic joints by straightforward extensions to the RNEA algorithms presented in \cite{michaux2023}.
Finally, let $\Nq = \{1,\ldots,\nq\}$.

\subsubsection{Tray and Object Model}

 \begin{figure}
        \centering
        \includegraphics[width=0.9\columnwidth]{Figures/RSS_2022_Figure_2_v2.pdf}
        \caption{Free Body Diagram of a manipulated object with the applied forces and moments. $\COMproj{}$ is the projection of the COM onto the contact plane.}
        \label{fig:contactdiagram}
    \end{figure}
    
    As illustrated in Fig. \ref{fig:contactdiagram}, the full system considered in this paper is comprised of a robotic manipulator that grasps a flat surfaced tray with an object resting on it.
    The normal to the tray is denoted by the unit vector $\eenorm \in \R^3$.
    We make the following assumptions about the full system:
    \begin{assum}
        \label{assum:contact}
        The manipulator is able to maintain force closure on the tray for all time.
        The object that is placed on the tray starts at rest (i.e., with zero velocity and acceleration relative to the tray) and the point representing the normal projection of the COM of the object onto the tray is denoted by $\COMproj{} \in W$.
        The object has a circular contact area with the tray that has radius $\objrad{}$.
        % The tray and object volumes are overapproximated as unions of convex polytopes \Ram{do we need notation for these objects? Also is it just sufficient to treat them with the link volume as we do in forward occupancy calculation or do we need to state the assumption here?}.
        % and therefore the tray can be treated as an additional link, where the corresponding joint is located between the grasp points of the manipulator. %\Zac{probably need to illustrate this, cite the paper that Rodriguez paper does which does this?}
        % When the object is not moving relative to its supporting surface, it can also be treated as an additional link, where the corresponding joint is located at point $\COMproj{}$, as shown in Figure \ref{fig:contactdiagram}. % this joint location is important for the ZMP constraint
        % The homogeneous transformation between the additional joint reference frames and the $\nq^{th}$ joint reference frame are known.
        % need to make sure that the part of the environment section gets incorporated where it is cited that convex objects can always be overapproximated by unions of convex polytopes. 
        % Furthermore, the true inertial parameters of the tray, $\Delta_{q+1}$, and the object, $\Delta_{q+2}$ lie in the known intervals $[\Delta_{q+1}]$ and $[\Delta_{q+2}]$, respectively. % with some nominal interval known as well.
    \end{assum}
    \noindent Based on this assumption, the tray can be treated as an additional joint in the kinematic chain of the manipulator. 
    In particular, this $(\nq+1)^{\text{th}}$ joint is located at the grasp point of the manipulator with the tray and can be treated as a fixed joint. 
    Note that the approach described in this paper could be generalized to ensure that a force closure condition was satisfied throughout the motion, but in the interest of simplicity, we have left out that extension. 
    One can similarly generalize the types of contact patch.
    If the object moves with respect to the tray during motion, we say that the object is \emph{slipping}.
    \Ram{do we want to call it something other than slipping because it could be tipping or other motion.}
    
    This paper's goal is to devise a strategy to avoid slipping.
    As we describe in Sec. \ref{sec:}, our approach first performs optimization to identify a trajectory parameter that can be tracked by the robot without slipping.
    Then, as we describe in Sec. \ref{sec:}, we track the trajectory by applying a robust passivity-based controller. 
    To do this, we treat joint $\nq+2$ as a fixed joint.
    As we describe in Sec. \ref{subsec:contact_constraint}, one can formulate constraints that ensure that the contact wrench applied to joint $\nq+2$ does not induce slipping, which ensures that the fixed joint model for joint $\nq+2$ is satisfied.  
    Throughout the remainder of the paper, we refer to this manipulator, tray, and object system as the \emph{extended arm}, and append the trajectory of the configuration to include these two additional joints, {\textit i.e.}, $Q \subset \R^{\nq+2}$ so $q:T \to Q$ and $\dot{q}:T \to \R^{\nq+2}$.
    We also let $\Ne = \{1,\ldots,\nq+2\}$.
    Because of the importance of joint $\nq + 2$, we sometimes use the subscript $\contact$ when referring to it, {\textit e.g.}, $q_\contact(t)$ refers to component $\nq+2$ of $\q$, which represents joint $\nq+2$'s trajectory at time $t$.
    % As a result, we need (1) a model that can be utilized within the optimization problem to predict the forces and torques that are generated on the object by the manipulator and tray while tracking a particular trajectory; and (2) a model to synthesize the robust passivity-based control input that tracks the computed trajectory and keeps the object at rest relative to the tray while the tray is moved.
    
    % To accomplish this objective, we use a pair of models that are identical for the first $\nq+1$ joints, but differ at joint $\nq+2$ as described next.
    % \begin{rem} 
    % \label{rem:model_lastjoint}
    % To synthesize the robust passivity based-control, we model joint $\nq+2$ as a fixed joint. 
    % The kinematics and dynamics of this model, which we refer to as the \defemph{control model}, are described in the remainder of this section.
    % To ensure that this fixed joint assumption is satisfied, in the optimization problem, we build a model that predicts the wrenches generated at $\COMproj{}$ by the motion of the manipulator and tray. 
    % The dynamics of this model, which we refer to as the \defemph{optimization model}, is described in Sec. \ref{sec:}.
    % \end{rem}
    

\subsubsection{Extended Arm Kinematics}

Next, we introduce the extended arm's kinematics.
Suppose there exists a fixed inertial reference frame, which we call the \defemph{world} frame.
In addition suppose there exists a \defemph{base} frame, which we denote the $0$\ts{th} frame, that indicates the origin of the robot's kinematic chain.
We assume that the $j$\ts{th} reference frame $\{\hat{x}_j, \hat{y}_j, \hat{z}_j\}$ is attached to the robot's $j$\ts{th} revolute joint, and that $\hat{z}_j = [0, 0, 1]\trans$ corresponds to the $j$\ts{th} joint's axis of rotation for $j \in \Nq$.
The reference frames for joints $\nq+1$ and $\nq+2$ have their x-axis aligned with joint $\nq$.
The z-axis of the reference frame for joint $\nq+1$ is aligned with joint $\nq$, and the z-axis of the reference frame for joint $\nq+2$ is aligned with the normal of the tray surface.

Then for a configuration at a particular time, $\q$, the position and orientation of frame $j$ with respect to frame $j-1$ can be expressed using homogeneous transformations \cite[Ch. 2]{spong2005textbook}:
\begin{equation}
\label{eq:homogeneous_transform}
    T_{j}^{j-1}(\qj) = 
    \begin{bmatrix} R\jssmu (\qj) & p\jssmu \\
    \zeros  & 1 \\
    \end{bmatrix},
\end{equation}
where $R\jssmu (\qj)$ is a configuration-dependent rotation matrix and $p\jssmu$ is the fixed translation vector from frame $j-1$ to frame $j$.
We use this superscript and subscript convention for all quantities moving forward. 
Finally, note that for fixed joints $T_j^{j-1}$ is fixed.

With these definitions, we can express the forward kinematics of the extended arm.
Let $\FK_j: Q \to \R^{4 \times 4}$ map the robot's configuration to the position and orientation of the $j$\ts{th} joint in the world frame:
\begin{equation}\label{eq:fk_j}
    \FK_j(\q) = 
    \prod_{l=1}^{j} T_{l}^{l-1}(q_l(t)) = 
    \begin{bmatrix} R_j(\q) & p_j(\q) \\
    \zeros  & 1 \\
    \end{bmatrix},
\end{equation}
% \pat{per Zac: should the $\qj$ in the product be $q_l$ instead? also, should the matrix have a $R_{j}$ and $p_{j}$} \jon{fixed}
where 
\begin{equation}
    R_j(\q) \coloneqq R_j^{0}(\q) = \prod_{l=1}^{j}R_{l}^{l-1}(\ql)
\end{equation}
and 
\begin{equation}
    p_j(\q) = \sum_{l=1}^{j} R_{l}(\q) p_{l}^{l-1}.
\end{equation}

\subsubsection{Extended Arm Occupancy}

An arm's kinematics can be used to describe the volume occupied by the arm in the workspace. 
Let $L_j \subset \R^3$ denote an overapproximation to the volume occupied by the $j$\ts{th} link with respect to the $j$\ts{th} reference frame. 
Then the map $\FO_j: Q \to \pow{W}$ gives the forward occupancy of link $j$:
\begin{align}\label{eq:forward_occupancy_j}
     \FO_j(\q) &= p_j(\q) \oplus R_j(\q) L_j,
\end{align}
where the first expression gives the position of joint $j$ and the second gives the rotated volume of link $j$.
The function $\FO: Q \to \pow{W}$ then gives the volume occupied by the entire arm in the workspace:
\begin{align}\label{eq:forward_occupancy}
    \FO(\q) = \bigcup_{j = 1}^{\nq+2} \FO_j(\q) \subset W. 
\end{align}

\subsubsection{Extended Arm Dynamics}
We assume the robot is composed of $\Nq$ rigid links with inertial parameters given by the vector
\begin{equation}\label{eq:true_intertial_parameters}
    \Delta = (m_1, \ldots, m_{\nq+2}, c_{x,1}, \ldots, c_{z,{\nq+2}}, I_{xx,1}, \ldots, I_{zz,{\nq+2}})\trans
\end{equation}
where $m_j$, $c_j =(c_{x,j}, c_{y,j}, c_{z,j})\trans$, and $(I_{xx,j}, \ldots, I_{zz,j})\trans$  represent the mass, center of mass, and inertia tensor of the $j$\ts{th} link, respectively. 
The dynamics are represented by the standard manipulator equations \cite{spong2005textbook}:
\begin{equation}\label{eq:manipulator_equation}
    % \roboteqn    
    \bM(\q, \Delta) \qdd +
    \bC(\q, \qd, \Delta) \qd +
    \bG(\q, \Delta) = u(t)
\end{equation}
where $\Mq \in \R^{\nq+2 \times \nq+2}$ is the positive definite inertia matrix, $\Cqd$ is the Coriolis matrix, $\Gqd$ is the gravity vector, and $u(t)$ is the input torque all at time $t$.
Note, for simplicity, we do not explicitly model friction, but it can be incorporated in $\bG(\q, \Delta)$ \cite{giusti2017efficient,giusti2021interval}.

We make the following assumptions about the robot's inertial parameters:
\begin{assum}[Inertial Parameter Bounds]
\label{assum:arm_model}
The model structure (i.e., number of joints, sizes of links, etc.) of the robot is known, but its true inertial parameters $\trueparams$ are unknown. 
The uncertainty in each inertial parameter is known and given by the interval vector
\begin{equation}
    \intparams = \left(\iv{m_1}, \ldots, \iv{m_{\nq+2}}, \iv{c_{x,1}}, \ldots, \iv{c_{z,{\nq+2}}}, \iv{I_{xx,1}}, \ldots \iv{I_{zz,\nq+2}}\right)\trans
\end{equation}
% where polynomial zonotopes $\pz{m_j} \subset \R$, $\pz{c_j} \subset \R^3$, and $\pz{I_j}\subset \R^{3 \times 3}$ represent the uncertainties in the mass, center of mass, and inertia tensor of the $j$\ts{th} link, respectively.
where $[m_j] \subset \mathbb{IR}$, $[c_j] \subset \mathbb{IR}^3$, and $[I_j]\subset \mathbb{IR}^{3 \times 3}$ represent the uncertainties in the mass, center of mass, and inertia tensor of the $j$\ts{th} link, respectively.
% An interval overapproximation $\pzparams \subseteq \intparams$ is given by
% \begin{equation}
    % [\Delta] = \left([m_1], \cdots, [m_{\nq}], [c_{x,1}], \cdots, [c_{z,{\nq}}], [I_{xx,1}], \cdots [I_{zz,\nq}]\right)\trans
% \end{equation}
% where $[m_j] = [\setop{inf}(\pz{m_j}), \setop{sup}(\pz{m_j})]$, $[c_j] = [\setop{inf}(\pz{c_j}), \setop{sup}(\pz{c_j})]$, and $[I_j] = [\setop{inf}(\pz{I_j}), \setop{sup}(\pz{I_j})]$.
% where $[m_j] = [\setop{inf}(\pz{m_j}), \setop{sup}(\pz{m_j})] \subset \mathbb{IR}$, $[c_j] = [\setop{inf}(\pz{c_j}), \setop{sup}(\pz{c_j})] \subset \mathbb{IR}^3$, and $[I_j] = [\setop{inf}(\pz{I_j}), \setop{sup}(\pz{I_j})] \subset \mathbb{IR}^{3 \times 3}$.
% where $[m_j] \subset \mathbb{IR}$, $[c_j] \subset \mathbb{IR}^3$, and $[I_j]\subset \mathbb{IR}^{3 \times 3}$ represent the uncertainties in the mass, center of mass, and inertia tensor of the $j$\ts{th} link, respectively.
The true parameters lie in this interval, i.e., $\trueparams \in \intparams$.
Any inertia tensor drawn from $[I_j]$ must be positive semidefinite.
In addition, if we let $[\Delta]_j$ denote the $j$\ts{th} component of $[\Delta]$, then $\texttt{inf}([\Delta]_j ) > -\infty$  and $\texttt{sup}([\Delta]_j) < \infty$ for all $j$.
% In addition, if we let $\pzgreek{\Delta}_\pz{j}$ denote the $j$\ts{th} component of $\pzparams$, then $\setop{inf}(\pzgreek{\Delta}_\pz{j}) > -\infty$  and $\setop{sup}(\pzgreek{\Delta}_\pz{j}) < \infty$ for all $j$.
Finally, there exists a nominal vector of inertial parameters $\nomparams \in \intparams$ that serves as an estimate of the true parameters of the system.
\end{assum}
\noindent Note, we do not assume that $\Delta_0$ is equal to the true parameters of the system or even a good estimate to the true parameters. 


\subsection{Contact Wrench Model for Joint $\nq+2$}
\label{subsec:contact_constraint}

To ensure that the object does not slip, we need a model that predicts wrenches applied on the object during motion.
As we describe below, the wrenches applied to the object are a function of robots configuration trajectory and its velocity and acceleration.
To simplify, notation we define the \emph{total trajectory}, $\qT$, as:
\begin{equation}
\label{eq:total_traj}
\qT(t) = \begin{bmatrix} \q^{\top} & \qd^{\top} & \qdd^{\top} \end{bmatrix}^{\top},
\end{equation}
at time $t$,
The motion of the object relative to the supporting surface is determined by the wrenches applied to it.
Because there are no external wrenches applied to the system, the object at time $t$ is manipulated only by the following contact wrench \Ram{this fact is missing a citation} 
% \begin{equation}
% \cwrench(\q,\qd,\qdd) = 
% \begin{bmatrix} 
% \cxforce(\q,\qd,\qdd) \\ \cyforce(\q,\qd,\qdd) \\ \czforce(\q,\qd,\qdd) \\ \cxmoment(\q,\qd,\qdd) \\ \cymoment(\q,\qd,\qdd) \\ \czmoment(\q,\qd,\qdd) \end{bmatrix},
% \end{equation}
\begin{equation}
\cwrench(\qT(t)) = 
\begin{bmatrix} 
\cforce(\qT(t)) \\ \cmoment(\qT(t)) \end{bmatrix},
\end{equation}
where $\cforce(\qT(t)) \in \R^3$ and $\cmoment(\qT(t)) \in \R^3$ and the gravito-inertial wrench 
\begin{equation}
\gravinertwrench{\contact}(\qT(t)) =
\begin{bmatrix}
\FGravInert{}(\qT(t)) \\  \MGravInert{}(\qT(t))
\end{bmatrix},
\end{equation}
where both of these wrenches are described in the frame associated with joint $\contact$.
\Ram{it would be helpful to tell us what space these things belong to. Like is it in $\R^6$}
For convenience, we denote the first, second, and third components of $\cforce(\qT(t))$ by $\cxforce(\qT(t)),$ $\cyforce(\qT(t)),$ and $\czforce(\qT(t)),$ respectively.
The contact wrench is applied by the manipulator through the supporting surface, and is located at point $\COMproj{}$.
The gravito-inertial wrench acts on the center of mass of the object being manipulated.
By constraining the contact wrench, the motion of the object can be constrained in all six degrees of freedom, resulting in no slipping.
As is described in Appendix \ref{app:nea}, one can apply a a variant of the Recursive Newton Euler Algorithm to compute this contact wrench.
% Due to the location of the contact joint, \eqref{eq:joint_force}-\eqref{eq:joint_torque} calculates the contact wrench $\cwrench(t)$ applied by the manipulator and tray to the object, and it is expressed in the contact frame.

We next describe how to constrain the contact wrench to restrict relative motion of the object.
% Describe the constraints that need to be enforced to achieve the task
\subsubsection{Separation Constraint}
    
The first degree of freedom to constrain is translation in the $\hat{z}_{\contact}$ direction, shown in Fig. \ref{fig:contactdiagram}.
Translation into the tray is prevented by a reaction force from the tray, which is assumed to be a rigid body.
The first constraint on the contract wrench prevents translation away from the tray surface.
A violation of this constraint means that the two bodies separate from one another, resulting in no normal force between the two bodies. 
 %Therefore the normal force is equal to the component of the contact force along the z-axis.
Thus this separation constraint can be written as
\begin{equation}
    \label{eq:sep_constraint}
    -\czforce(\qT(t)) \leq 0,
\end{equation}
where $\czforce(\qT(t))$ is the vertical force component of the contact wrench and is expressed in the contact frame, thus it corresponds to the normal force.
Satisfaction of this constraint means that a normal force exists, and therefore the object is not translating vertically relative to the tray.

\subsubsection{Linear Slipping Constraint}
    
The next two degrees of freedom, translation in the $\hat{x}_{\contact}$ and $\hat{y}_{\contact}$ directions, can be constrained using the static Coulomb friction law.
To represent this require, define the \emph{linear slip} function as: 
\begin{equation}
\slip(\qT(t)) := \lvert \cforcetan(\qT(t)) \rvert - \CoefFric \lvert \czforce(\qT(t)) \rvert,
\end{equation}
where $\CoefFric$ is the coefficient of static friction and $\cforcetan(\qT(t))$ is the force component of the contact wrench that is tangential to the supporting surface and is expressed in the contact frame.
If
\begin{equation}
    \label{eq:slip_constraint}
   \slip(\qT(t)) \leq 0,
\end{equation}
then the static friction between the object and the tray prevents the object from linearly slipping. 
Note that we do not consider rotational friction or uncertainty in the coefficient of static friction for simplicity, but extending the formulation to include such a constraint or uncertainty is a straightforward extension. 
        
    % \subsection{Rotational Slipping Constraint}
    
    %     \Zac{need to be wary about uniform vs nonuniform pressure distribution on contact area. could relate to the ZMP? look at center of pressure which is related but may not be the same}
    %     A rotational friction law is used to constrain rotation about $\hat{z}_{\contact}$.
    %     To derive the constraint, we first make the following assumptions:
    %     \begin{assum}
    %         \label{assum:rotational_friction}
    %         The object has a circular contact patch with radius $\objrad$ with a uniform normal pressure distribution and a uniform static coefficient of friction.
    %     \end{assum}
    %     Dividing the contact area into differential elements with area $dA$, then the maximum differential frictional moment is given by
    %     \begin{equation}
    %         \label{eq:diff_friction_moment}
    %         d\czmomentmax = \CoefFric p \objrad dA
    %     \end{equation}
    %     where $p$ is the normal pressure acting on the differential element. 
    %     Through integrating Eq. \eqref{eq:diff_friction_moment} over the contact area, the maximum frictional moment can be obtained:
    %     \begin{equation}
    %         \label{eq:integral_friction_moment}
    %         \begin{split}
    %         \czmomentmax & = \int_A d\czmomentmax \\
    %         & = \int_A \CoefFric p \objrad dA \\
    %         & = \CoefFric \frac{\czforce}{\pi \objrad^2} \int_{0}^{r_{o}} 2 \pi \objrad^2 dr \\
    %         & = \frac{2}{3} \CoefFric \objrad \czforce{}
    %         \end{split}
    %     \end{equation}
        
    %     The rotational friction constraint can be written as
    %     \begin{equation}
    %         \label{eq:rot_slip_constraint}
    %         \lvert \czmoment{} \rvert \leq \frac{2}{3} \CoefFric \objrad \lvert \czforce \rvert
    %     \end{equation}
    %     % depends on the contact area geometry.
        
    %     \Zac{need to add another subplot to the experimental figure for this}
    
\subsubsection{Tipping Constraint}
    
Finally, we must constrain the last two degrees of freedom, which are rotation about $\hat{x}_{\contact}$ and $\hat{y}_{\contact}$.
Motion about these axes corresponds to the object tipping over. 
To prevent this, we use a Zero Moment Point (ZMP) constraint, which requires that the ZMP point exists inside the convex hull of the contact area of the object \cite{VUKOBRATOVIC2012}.
This ensures that the normal component of the contact force can apply a sufficient counteracting moment to balance the gravito-inertial wrench of the object.
        % mention that the wrench is transmitted only through the friction and normal force, which correspond to f_x,f_y,f_z and n_z? so only these components are used to write constraints. 
First, the vector from $\COMproj{}$ to the ZMP point is \Ram{cite something.}:
\begin{equation}
    \label{eq:ZMPpoint}
    \frac{\eenorm{} \times \MGravInertProj{}(\qT(t))}{\eenorm{} \cdot \FGravInertProj{}(\qT(t))},
\end{equation}
where 
% $\COMproj{}$ is the point representing the normal projection of the COM of the object onto the supporting surface, $\ZMPpoint{}(\qT(t))$ is the location of the ZMP point, 
$\MGravInertProj{}(\qT(t))$ is the gravito-inertial moment acting on the object about $\COMproj{}$, and $\FGravInertProj{}(\qT(t))$ is the gravito-inertial force acting on $\COMproj{}$. 
        % also assuming no other external wrench acting on object so only gravito-inertial wrench needs to be balanced by the supporting surface wrench
        % Need to make sure that the gravito-inertial force and moment are labelled properly. Maybe cite another paper as well? 
        
Next, there are only two wrenches acting on the object, the wrench applied by the manipulator and the gravito-inertial wrench of the object. 
For there to be no relative motion, these two wrenches must balance each other. 
Therefore $\MGravInertProj{}(\qT(t)) = -\cmoment(\qT(t))$ and $\FGravInertProj{}(\qT(t)) = -\cforce(\qT(t))$.
Substituting these terms in \eqref{eq:ZMPpoint} yields
\begin{equation}
    \label{eq:ZMPpointContact}
    \ZMPvec{}(\qT(t)) = \frac{\eenorm{} \times \cmoment(\qT(t))}{\eenorm{} \cdot \cforce(\qT(t))}.
\end{equation}
        % since the negative signs can be factored out and canceled. 
        % \Zac{should probably change the name of $\ZMPvec{}$}
Note that the contact frame is located at $\COMproj{}$, so \eqref{eq:ZMPpointContact} gives the position of the ZMP point with respect to the origin of the contact frame.
Using the description of the contact path as in Ass. \ref{assum:contact}, the ZMP constraint can be written as:
\begin{equation}
    \label{eq:tip_constraint}
    \lVert \ZMPvec{}(\qT(t)) \rVert \leq \objrad.
\end{equation}
\Ram{what norm are you using? Is it the two norm?}
If this constraint is satisfied, then the ZMP point stays inside the circular contact area and the object does not tilt \Ram{what does tilt mean?} relative to the tray.
Using these constraints and by applying \Ram{reference a theorem or something}, one can ensure that slipping does not occur:
\begin{lem}
    \label{lem:constraint_satisfaction}
    If the object starts at rest and \eqref{eq:sep_constraint}-\eqref{eq:tip_constraint} are satisfied by a trajectory $\qT(t)$ for all $t \in T$, then the object will not slip for $t \in T$.
\end{lem}
        
        % \Zac{should redo the ZMP constraint to be like the obstacle avoidance constraint. represent the contact area using a halfspace representation and then check if the ZMP point is inside the halfspace area. would be something like A*slice(ZMPt;k)/slice(ZMPb;k)-b<0 I think.}

\subsection{Environment}
\label{subsec:environment}

% \shrey{figure suggestion: there should be an environment with obstacles figure in the numerical examples section, so it would be helpful to point to that here and be like ``for an example, look later in the text at Fig. whatever''}

Next, we describe obstacles and the start and goal configurations of the robot.
% The robot's origin is assumed to coincide with the environment's origin without loss of generality.

\subsubsection{Obstacles}
We begin by defining and making a few assumptions about obstacles:
% We denote the set of obstacles as a set $O \subset W$.
% We make the following assumptions about obstacles:
\begin{assum}[Obstacles]
\label{assum:obstacles}
The transformation between the world frame of the workspace and the base frame of the robot is assumed to be known, and obstacles are expressed in the base frame of the robot.
At any time, the number of obstacles $\nObs \in \N$ in the scene is finite ($\nObs < \infty$).
Let $\obsset$ be the set of all obstacles $\{ O_1, O_2, \ldots, O_{\nObs} \}$.
% \pat{$\obsset$ is a set here, but we use it like it's the union of obstacles when writing the trajopt}
Each obstacle is convex, bounded, and static with respect to time.
% The robot has access to a conservative estimate of the size and location of each obstacle (this work is concerned with planning and control, not perception).
The arm has access to a zonotope overapproximation of each obstacle's volume in workspace.
\end{assum}
\noindent We say that the arm is \defemph{in collision} with an obstacle if $\FO_j(\q) \cap O_i \neq \emptyset$ for any $j \in \Ne$ or $i \in \{1,\ldots,\nObs\}$. 
Note that this work is concerned with planning and control around obstacles without slipping, not perception of obstacles.
A convex, bounded object can always be overapproximated as a zonotope \cite{guibas2003zonotopes}.
In addition, if one is given a non-convex bounded obstacle, then one can outerapproximate that obstacle by computing its convex hull. 
Dynamic obstacles may also be considered within the \MethodName{} framework by introducing a more general notion of safety \cite[Definition 11]{vaskov2019towards}, but we omit this case in this paper to ease exposition.
Next, note that we have assumed for convenience that the robot is able to sense all obstacles workspace. 
However, in practice, one could assume that the robot has a finite sensing horizon in which it is able to sense obstacles. 
In this instance, one could extend the results regarding the collision free behavior of \MethodName{} by applying Theorem 39 in \cite{kousik2020bridging}.
Finally, if a portion of the scene is occluded then one can treat that portion of the scene as an obstacle.

\subsubsection{Start and Goal Configurations}
Next, we describe the start and goal configurations of the robot.
\begin{defn}[Start and Goal Configurations]
\label{def:start_and_goal_config}
The robot begins from rest from the known starting configuration $\qstart$.
It has zero initial velocity and zero initial acceleration.
\MethodName{} attempts to find and execute a sequence of safe trajectories from $\qstart$ to a user-specified goal configuration, $\qgoal$.
\end{defn}
\noindent We note that an end-effector goal position in workspace may be specified instead of the configuration $\qgoal$ if desired.
We omit this case for simplicity, as it only affects the user-specified cost function in Sec. \ref{sec:planning_formulation}.



==> Sections/04_planningtheory.tex <==
\section{Proposed Method Overview}
\label{sec:planning_formulation}


This section provides a high-level overview of \MethodName{}. 
In particular, this section summarizes how limits are placed on planning time (Section \ref{subsec:timing}), how \MethodName{} represents trajectories (Section \ref{subsec:parameterization}), and describes an optimization problem that could ensure $\relativeMotion$ free behavior (Section \ref{subsec:theoretical_optprob}). 
Section \ref{sec:formulation} describes how to formulate this optimization problem in a tractable manner. 

\subsection{Timing}
\label{subsec:timing}

Recall that \MethodName{} performs planning in a receding horizon fashion.
We assume without loss of generality that the control input and trajectory of a planning iteration begin at time $t=0$ and end at a fixed time $\tfin$.
To ensure persistent real-time operation, we require that \MethodName{} identifies a new trajectory parameter within a fixed planning time of $t\plan$ seconds, where $t\plan < \tfin$.
Thus \MethodName{} has limited planning time and must select a new trajectory parameter before completing its tracking of the previously identified desired trajectory.
If no new trajectory parameter is found in time, \MethodName{} defaults to a braking maneuver that brings the robot to a stop at time $t = \tfin$.
As is described in Sec. \ref{subsec:parameterization}, we require each desired trajectory to contain such a maneuver, which is verified as safe in the previous planning iteration.

\subsection{Trajectory Parameterization}
\label{subsec:parameterization}

In each planning iteration, \MethodName{} chooses a desired trajectory to be followed by the arm. 
These trajectories are chosen from a pre-specified continuum of trajectories, with each uniquely determined by a \textit{trajectory parameter} $k \in K$.
The set $K \subset \R^{n_k}$, $n_k \in \N$, is compact and represents a user-designed continuum of trajectories. 
In general, $K$ can be designed to include trajectories designed for a wide variety of tasks and robot morphologies \cite{holmes2020armtd, kousik2020bridging, kousik2019_quad_RTD}, as long as each trajectory satisfies the following properties.
\begin{defn}[Trajectory Parameters]
\label{def:traj_param}
For each $k \in K$, a \emph{desired trajectory} is an analytic function $q_d(\,\cdot\,; k) : T \to Q$ that satisfies the following properties:
\begin{outline}[enumerate]
\1 The trajectory starts at a specified initial condition $(\initq, \initdq, \initddq)$, so that $q_d(0; k) = \initq$, $\dot{q}_d(0; k) = \initdq$, and $\ddot{q}_d(0; k) = \initddq$.
\1 $\dot{q}_d(\tfin; k) = 0$ and $\ddot{q}_d(\tfin; k) = 0$ (i.e., each trajectory brakes to a stop, and at the final time has zero velocity and acceleration).
\1 $\ddot{q}_d(\,\cdot\,; k)$ is Lipschitz continuous and bounded.
% \1 For $j = \nq+1$, $q_{d,j}(t,k) = 0$  for all $t \in T$.
% \pat{Again I vote to remove this last part!} 
% \Zac{depends on how the dynamics equation is updated? \eqref{eq:manipulator_equation} is currently $\R^{\nq}$ but RNEA is $\R^{\nq+1}$?}
\end{outline}
\end{defn}
\noindent The first property allows for desired trajectories to be generated online.
In particular, recall that \MethodName{} performs real-time receding horizon planning by executing a desired trajectory computed at a previous planning iteration while constructing a new desired trajectory for the subsequent time interval. 
The first property allows desired trajectories that are generated by \MethodName{} to begin from the appropriate future initial condition of the robot.
The second property ensures that a fail safe braking maneuver is always available.
The third property ensures that desired position, velocity, and acceleration trajectories for the tracking controller are sufficiently continuous.
% The fourth property requires that the desired trajectory is $0$ for the fixed joint of the extended arm corresponding to the tray-object interface. 
Once a particular trajectory parameter is computed, \MethodName{} tracks the identified desired trajectory by applying a feedback control input described in Section \ref{sec:controller}. 

% This control input is a function of the interval inertial parameters $[\Delta]$, and the state of the robot; however, it cannot be a function of the true inertial parameters because these are not assumed known. 
% Applying this control input to the arm using \eqref{eq:manipulator_equation} generates an associated trajectory of the arm. 
% Note that this position and velocity trajectory is a function of the true inertial parameters of the robot. 
% We denote the position and velocity trajectories at time $t \in T$ under trajectory $k \in K$ and under the true inertia model parameters $\Delta \in \intparams$ by $q(t;k,\Delta)$ and $\dot{q}(t;k,\Delta)$, respectively.
% We similarly denote the total trajectory by $\qT(t;k,\Delta)$. 
% To simplify notation, in this section, we denote the feedback control input at time $t \in T$ under trajectory $k \in K$ by $u(t;k)$ 
% {\it Note that after this section, the control input is allowed to be a function of the interval inertial parameters, $\intparams$, the state of the system, and the trajectory parameter.}

\subsection{Online Trajectory Optimization}  
\label{subsec:theoretical_optprob}

Using this parameterization and the constraints described in Sec. \ref{subsec:contact_constraint}, a solution resulting in safe manipulation of unsecured objects can be computed using:
\begin{align}
    \label{eq:optcost}
    &\underset{k \in K}{\min} &&\texttt{cost}(k) \\
    % \label{eq:optpos}
    % &&&  q_j(t; k, \Delta) \in [\qlim^-, \qlim^+]  &&\forall t \in T, \Delta \in [\Delta], j \in \Nq \\
    % \label{eq:optvel}
    % &&& \dot{q}_j(t; k, \Delta) \in [\dqlim^-, \dqlim^+]  &&\forall t \in T,  \Delta \in [\Delta], j \in \Nq \\
    % \label{eq:opttorque}
    % &&&  u_j(t;k) \in [\ulim^-, \ulim^+]  &&\forall t \in T,  \Delta \in [\Delta], j \in \Nq \\
    % \label{eq:optcolcon}
    % &&& \FO_j(q(t; k,\Delta)) \bigcap \obsset = \emptyset  &&\forall t \in T,  \Delta \in [\Delta], j \in \Ne \\
    \label{eq:optsepcon}
    &&&  \sep(\qT(t;k, \Delta)) \leq 0 &&\forall t \in T,  \Delta \in [\Delta] \\
    \label{eq:optslipcon}
    &&& \slip(\qT(t;k,\Delta)) \leq 0 &&\forall t \in T,  \Delta \in [\Delta]  \\
    \label{eq:opttipcon}
    %&&& ||\ZMPvec{}((\qT(t;k, \Delta))|| \le \objrad &&\forall t \in T,  \Delta \in [\Delta].
    &&& \tip(\qT(t;k,\Delta)) \le 0 &&\forall t \in T,  \Delta \in [\Delta].
\end{align}
In this optimization problem, the cost function, \eqref{eq:optcost} specifies a user-defined objective, such as bringing the robot close to some desired goal while
% Each of the constraints guarantee the safety of any feasible trajectory parameter, as we describe next.
% We define an optimal trajectory in the following way.
% First, the trajectory must be executable by the robot.
% This means the trajectory must not violate the robot's joint position \eqref{eq:optpos}, velocity \eqref{eq:optvel}, or input \eqref{eq:opttorque} limits.
% These constraints must be satisfied for each joint over the entire planning horizon despite model uncertainty.
% Although we have suppressed the dependence, we stress that {\it the control input in the remainder of the paper is also function of the state of the robot arm, which is a function of the (unknown) true inertial parameters}.
\eqref{eq:optsepcon}-\eqref{eq:opttipcon} ensure that the object on the tray does not experience $\relativeMotion$.

Implementing a real-time optimization algorithm to solve this problem is challenging for several reasons.
First, the dynamics of the robot are nonlinear and constructing an explicit solution to them is intractable. 
% Second, the constraints to ensure collision free and $\relativeMotion$ free behavior are non-convex. 
Second, the constraints must be satisfied for all time $t$ in an uncountable set $T$.
% Note, as we discuss in Section \ref{sec:experimental}, one could incorporate obstacle avoidance, input, and joint limit constraints into this optimization problem. 
% These would only further compound the difficulties associated with solving the optimization problem above.
The next section proposes a method to generate tight overapproximations to the trajectories and constraints that are differentiable and enable the application of fast optimization techniques.

==> Sections/Symbols.tex <==
\subsection{List of Symbols}

\begin{itemize}

    \item $a_0$: coefficient (for zonotopes it can be the center)
    
    \item $\pzei$: polyzonotope exponents
    
%    \item $\robgain$: robust input "gain"

    \item $\beta_i$: zonotope indeterminants
    
    \item $c$: zonotope center
    
    \item $_c$: subscript c denotes the contact joint meaning $j=\nq+2$
    
    \item $c_{x_j}$: x-coordinate of COM of j-th link (same for y and z) % this seems to overload c somewhat
    
    \item $C$: Matrix zonotope center
    
    \item $C(q, \Delta)$: Coriolis matrix

    \item $\Delta$: vector of inertial parameters
    
    \item $\Delta_0$: vector of nominal inertial parameters
    
    \item $[\Delta]$: vector of interval inertial parameters
    
    % \item $\pz{\Delta}$: vector of PZ inertial parameters
    
    \item $e$: vector of joint position errors
    
    \item $\dot{e}$: vector of joint velocity errors
    
    \item $\pbound$: ultimate position bound for single joint
    
    \item $\vbound$: ultimate velocity bound for single joint
    
    \item $\pboundvec$: vector of ultimate position bounds
    
    \item $\vboundvec$: vector of ultimate velocity bounds
    
    \item $\text{f}_j^i$: Force at joint $j$ expressed in frame $i$. Note: frame notation dropped if frame is the joint frame, i.e. the indices would be the same.
    
    \item $\cforce$: force at contact joint in contact frame
    
    \item $\cforcenormal$: normal component of contact force
    
    \item $\cforcetan$: tangential component of contact force
    
    \item $\genwrench{j}$: wrench at joint $j$ expressed in frame $j$
    
    \item $\cwrench$: contact wrench applied to loose object by manipulator, corresponds to wrench at joint $j=\nq_{+2}$
    
    \item $F_i^j$: Force at COM of link $i$ expressed in frame $j$
    
    \item $\FGravInert$: Gravito-Inertial forces acting on loose object
    
    \item $\FK_i(q)$: forward kinematics of link $i$
    
    \item $\FO_i(q)$: forward occupancy of link $i$
    
    \item $\robcoeff$: robust input coefficient
    
    \item $g_i$: $i^{th}$ zonotope generator
    
    \item $\pzgi$: $i^{th}$ PZ coefficient (aka generator) % currently the same as the zonotope generator
    
    \item $G_i$:  $i^{th}$ generator matrix of Matrix zonotope 
    
    \item $G(q, \Delta)$: gravity vector
    
    \item $\kscale$: scale for $k$ interval
    
    \item $\robh$: control barrier function
    
    \item $\robH$: forward invariant set associated with $\robh$
    
    \item $i$: time index
    
    \item $I_i^j$: link i inertia tensor wrt frame j
    
    \item $j$: joint index
    
%   \item $\mathcal{J}_i$: joint reachable set
%   \item $J_i(t)$: offline overapproximation of joint reachable set

    \item $k$: trajectory parameter
    
    \item $K$: space of trajectory parameters
    
    \item $K_r$: gain matrix % not sure
    
    \item $\kappa_P$: robust controller gain
    
    \item $L_j$: volume of link j
    
%   \item $\lambda_j$: indeterminants

    \item $\lambda_{min}$: smallest eigenvalue
    
    \item $\lambda_{max}$: largest eigenvalue
    
    \item $m_i$: mass of link i
    
    \item $M$: matrix zonotope
    
%   \item$\Mit$: matrix zonotope as a function of time

    \item $M$: positive definite inertia matrix \Zac{overloads the capital M}
    
    \item $n$: reaction torque at the joint
    
    \item $N$: torque at the COM of a body
    
    \item $\MGravInert$: Gravito-Inertial Moments acting on loose object
    
    \item $\pz{M}$: poly zonotope Mass matrix
    
    \item $\pz{M(\pz{\q})}$: pz mass matriz as a function of pz state.
    
    \item $M(\q, \Delta)$ true mass matrix at $\q$
    
    \item $n$: generic constant
    
    \item $\eenorm{}$: supporting surface normal
    
    \item $\cmoment$: moment at the contact joint expressed in contact frame. subscript denotes a component. 
    
    \item $\nq$: number of joints
    
    \item $\nt$ number of time steps
    
%   \item $n_{n_q}^{n_q}$: moment

    \item $\nObs$: number of obstacles
    
    \item $N_i^j$: moment of body $i$ expressed in $j^{th}$ frame
    
    \item $O_j$: Obstacle $j$ where $j$ is a generic index
    
    \item $\obsset$: set of all obstacles
    
    \item $\mathbb{N}$: natural numbers
    
    \item $\pzn$: number of PZ generators
    
    \item $p_1$: generic point inside poly zonotope
    
    \item $p_2$: generic point inside poly zonotope
    
    \item $p_i$: position of frame $i$ relative to frame $0$
    
    \item $p_{i-1,i}^j$: position of frame i wrt frame i-1 expressed in frame j \jon{i think this is not needed}
    
    \item $\COMproj$: projection of the COM of loose object onto the supporting surface
    
    \item $\pz{P_1}$: generic polynomial zonotope
    
    \item $\pz{P_2}$: generic polynomial zonotope
    

%   \item $[\Phi]$: interval disturbance
%   \item $\varphi_P$: robust controller gain

    \item $q$: vector of joint positions
    
    \item $\qd$: vector of joint velocities
    
    \item $\qdd$: vector of joint accelerations
    
    \item $\initq$: estimate of initial position
    
    \item $\initdq$: estimate of initial velocity
    
    \item $\qdes$: desired joint positions
    
    \item $\qdesdot$: desired joint velocities
    
    \item $\qdesddot$: desired joint accelerations
    
    \item $\qadot$: modified velocity trajectory
    
    \item $\qaddot$: modified acceleration trajectory
    
    \item $\pzqji$: poly zonotope representation of $q$ at $i$\ts{th} time step
    
    \item $\pzqdji$: poly zonotope representation of $\qd$ at $i$\ts{th} time step
    
    \item $Q$: configuration space
    
    \item $\robr$: modified error
    
    \item $\objrad$: radius of contact area of object
    
    \item $R_{i-1}^i$: orientation of frame $i-1$ \textit{wrt} frame $i$
    
    \item $R_i(q)$: orientation of frame $i$ \textit{wrt} frame $0$
    
    \item $\pz{R_{i-1}^i}$: poly zonotope representation of orientation of frame $i-1$ \textit{wrt} frame i
    
    \item $\mathbb{R}^n$: n-dimensional set of real numbers
    
%   \item $\rho$: worst-case disturbance

%   \item $S_i(t)$: sliced reachable set

    \item $\sigma$: coefficient to be sliced/evaluated
    
    \item $\sigma_m$: uniform bound (lower)
    
    \item $\sigma_M$: uniform bound (upper)
    
    \item $t$: time
    
    \item $T$: compact time interval
    
    \item $T_{j}^{j-1}(\qj)$: homogeneous transformation from joint j-1 to joint j
    
    \item $\tau$: nominal control input
    
    \item $u$: control input
    
    \item $\CoefFric$: coefficient of static friction between the loose object and the supporting surface
    
%   \item $U_i(t)$: overapproximation of input reachable set
    
    \item $\robv$: robust control input
    
    \item $\dot{v}_i^j$: acceleration of frame $i$ expressed in frame $j$
    
    \item $\dot{v}_{COM,i}^j$: acceleration of the COM of link i expressed in frame j
    
    \item $\roblyap$: Lyapunov function
    
    \item $\roblevel$: Lyapunov function threshold
    
%   \item $V_i(t)$: zonotope representation of link i volume

    \item $w$: disturbance due to inertial uncertainty
    
    \item $\normwmax$ norm of max disturbance
    
    \item $W$: workspace
    
    \item $\omega_i^j$: frame i angular velocity wrt frame j
    
    \item $\dot{\omega}_i^j$: frame i angular acceleration wrt frame j
    
    \item $\pzv$: indeterminant for polynomial zonotope
    
    \item $\hat{x}_j$: unit vector of $j^{th}$ joint reference frame in the positive x direction
    
    \item $\hat{y}_j$: unit vector of $j^{th}$ joint reference frame in the positive y direction
    
    \item $\hat{z}_j$: unit vector of $j^{th}$ joint reference frame in the positive z direction
    
    \item $\ZMPpoint$: point that is the location of the ZMP
    
    \item $Z$: generic zonotope
    
    \item $Z_1$: generic zonotope
    
    \item $Z_2$: generic zonotope

% what notation will I need to add
% coefficient of friction mew
    \item $\mu_{s}$: coefficient of static friction
% radius of contact patch of loose object 
    \item $\objrad$: radius of the contact patch of the loosely placed object (assuming symmetrical contact patch)
% PZ inner approximation of contact patch of loose object
    
% height of loose object
    %\item $\heightobj$: height of the COM of the loosely placed object
% point indicating projection of COM of loose object onto the contact plane
% ZMP
    \item \ZMPpoint: the Zero Moment Point of the loosely placed object
% components of a generic force expressed in a certain frame
\end{itemize}

==> Sections/abstract.tex <==
\begin{abstract}
    In order to transition robotic manipulators from their current highly structured environments to operating in close proximity to humans and in environments where uncertainty is prevalent, certifiably safe motion planning and control methods are needed. The waiter motion problem is an illustrative task where current methods have yet to make the transition. We propose \MethodName{}, a certifiably safe motion planning and control framework and apply it to the waiter motion problem. This framework contains a mid-level receding horizon trajectory planner and a low-level robust controller which enable a robotic manipulator to safely operate in the presence of obstacles and uncertainty. In simulation, \MethodName{} outperforms a similar framework.
\end{abstract}

==> Sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

==> Sections/controller_design.tex <==
\section{Controller Design}
\label{sec:control_des}

This section summarizes the development of a robust passivity-based controller, which was introduced in previous work \cite{}. 
% Motivate need for robust controller
When there is uncertainty in the inertial parameters of the manipulator system, including the extended kinematic chain, the dynamics of the manipulator become uncertain. 
The controller conservatively compensates for this uncertainty and provides a bound on the worst-case tracking error.
This bound is critical for ensuring persistent feasibility while operating in a receding horizon fashion, as it enables us to account for the worst-case tracking performance when executing any desired trajectory.
In Sec. \ref{sec:plan_alg_theory}, constraints for obstacle avoidance, manipulator limits, and manipulation force constraints are developed using the bound.
This results in guaranteed constraint satisfaction when tracking a $\textit{feasible}$ desired reference trajectory, despite error in tracking the desired trajectory.
For the remainder of this section, we have dropped the dependence on $k$ in the trajectories for convenience.

In order to formulate the controller, we first define a \emph{total feedback trajectory}, $\qA$, at time $t$ consisting of the robot trajectory and the desired trajectory.
It is defined as:
\begin{equation} \label{eq:total_feedback_traj}
\qA(t) = \begin{bmatrix} q(t) & \dot{q}(t) & \ddot{q}(t) & q_d(t) & \dot{q}_d(t) & \ddot{q}_d(t) \end{bmatrix}.
\end{equation}
Using $\qA(t)$, we define a \emph{modified reference velocity trajectory}, $\dot{q}_a$, and \emph{modified reference acceleration trajectory}, $\ddot{q}_a$ as:
\begin{equation}\label{eq:modified_ref} % modified error
\begin{split}
    \dot{q}_a(t) &= \dot{q}_d(t) + K_r \err(t), \quad \err(t) = q_d(t) - q(t) \\
    \ddot{q}_a(t) &= \ddot{q}_d(t) + K_r \errdot(t), \quad \errdot(t) = \dot{q}_d(t) - \dot{q}(t)
    \end{split}
\end{equation}
where the gain matrix $K_r$ is a diagonal positive definite matrix.
% While these trajectories depend on the trajectory parameter $k \in K$, we have dropped this dependence for convenience in the remainder of the discussion.

For a given desired reference trajectory, the robust passivity-based control input at time $t \in T$ is $u(\qA(t), \Delta_0, [\Delta]) \in \R^\nq$, which is composed of a passivity-based nominal input $\tau(\qA(t), \Delta_0) \in \R^\nq$ and a robust input $\robv(\qA(t),\Delta_0, [\Delta]) \in \R^\nq$:
\begin{equation}
    \label{eq:controller}
	\controller
\end{equation}
This controller decomposition is similar to that proposed in \cite{giusti2016bound} and \cite{giusti2017efficient}.
The term $\robv(\qA(t),\Delta_0, [\Delta])$ compensates for the worst-case disturbances due to a mismatch between the nominal inertial parameters $\nomparams$ and the true inertial parameters $\Delta$.

The next subsection details the construction of the nominal input $\tau(t;k)$, and the following subsection details the construction of the robust input $\robvk$. 
% For brevity, we drop the notation for dependence on $t$ and $k$, i.e. $u$, meaning it is implied unless otherwise stated.

% could collapse these subsections?
\subsection{Nominal Input}

    The nominal control input is formed using the nominal model of the manipulator with the nominal inertial parameters $\nomparams$ described in Assumption \ref{assum:arm_model}, and is given by
    \begin{equation}
    	\label{eq:nominal_controller}
        \nominal
    \end{equation}
    where $\qatkdot$ and $\qatkddot$ are the modified reference velocity and acceleration defined above.

\subsection{Robust Input}

    The torques resulting from inertial parameter mismatch are treated as a disturbance $w$ given by
    \begin{equation}
        \label{eq:disturbance_equation}
        \begin{split}
        \wdist(\qA(t), &\Delta_0, \Delta) =  (\bM(q(t),\trueparams) -\bM(q(t),\nomparams)) \ddot{q}_a(t) + \\
         &+ (\bC(q(t), \dot{q}(t), \trueparams) - \bC(\q(t), \dot{q}(t), \nomparams))\dot{q}_a + \\ &+ \bG(q(t),\trueparams) - \bG(q(t),\nomparams).
         \end{split}
    \end{equation}
    In practice, the true disturbance $w$ is unknown, but can be bounded by
    \begin{equation}
        \label{eq:disturbance_vector}
        \wdist(\qA(t), \Delta_0, \Delta) \in \iv{\wdistinterval(\qA(t), \Delta_0, [\Delta])},
    \end{equation}
    where $\iv{\wdistinterval(\qA(t), \Delta_0, [\Delta])}$ is computed by plugging $\intparams$ into \eqref{eq:disturbance_equation} in place of $\trueparams$ and using interval arithmetic.
    % don't have alg IRNEA in this paper yet to reference here...
    
\subsection{Controller}

    This subsection details the construction of the controller using the nominal and robust inputs.
    First, we define a function for determining the measure of the worst case disturbance
    \begin{defn}
        \label{def:worst_case_disturbance}
        Let $\texttt{inf}([\wdistinterval(\qA(t),\Delta_0, [\Delta])]) =\underline{\wdistinterval}$ and $\texttt{sup}( [\wdistinterval(\qA(t),\Delta_0,[\Delta])]) = \overline{\wdistinterval}$.
        The \emph{measure of the worst case disturbance} is the function $\rho: \mathbb{I}\mathbb{R}^{n_q} \xrightarrow{} \mathbb{R}^{n_q}$ given by
        \begin{equation}
            \label{eq:worst_case_disturbance}
            \rho([\wdistinterval(\qA(t),\Delta_0,[\Delta])]) = \max(|\underline{\wdist}|, |\overline{\wdist}|)
        \end{equation}
        where the $\max$ operator is applied element-wise over the interval vector argument.
    \end{defn}
    Using this function, it can be shown that the worst-case disturbance bounds the absolute value of the disturbance $\abs{\wdist(\qA(t),\Delta_0,\Delta)}$.
    
    % \begin{lem}\label{lem:disturbance_bound}
    %     For all $t \in T$, $k \in K$ and $\trueparams \in \intparams$
    %     \begin{equation}
    %         \normwmax \geq \norm{\wdist}.    
    %     \end{equation}
    %     where $\normwmax = \norm{\rho(\wdistinterval)}$.
    % \end{lem}
    \begin{lem}\label{lem:disturbance_bound}
    For all $\qA(t) \in \mathbb{R}^{6\nq}$ and $\trueparams \in \intparams$
        \begin{equation}
            \rho([\wdistinterval(\qA(t), \Delta_0,[\Delta])] \geq \abs{\wdist(\qA(t), \Delta_0, \Delta)},
        \end{equation}
        where the inequality is appied element-wise.
    \end{lem}
    \begin{proof}
        Throughout the proof, we suppress the dependence on $\qA(t)$, $\Delta$, and $\Delta_0$ for convenience.
        From Eq. \eqref{eq:disturbance_vector}, the true disturbance $\wdist$ is contained in the interval $[\wdist]$. 
        Therefore, $\abs{w} \in [0, \max(|\underline{\wdistinterval}|, |\overline{\wdistinterval}|)]$. 
        Next from Def. \ref{def:worst_case_disturbance}, $\rho([\wdistinterval]) = \max(|\underline{\wdistinterval}|, |\overline{\wdistinterval}|)]$, and so $\rho([\wdistinterval]) \geq |w| \; \forall w \in \iv{w}$.
        % Next, from Def. \ref{def:worst_case_disturbance}
        % \begin{equation}
        %     \rho(\wdistinterval) \geq |\wdist|, \quad \forall \wdist \in \wdistinterval
        % \end{equation}
        % Because $\norm{\wdist} = \norm{(\abs{\wdist})}$, we have $\norm{{\rho(\wdistinterval)}} \geq \norm{\wdist}$.
    \end{proof}
    
    Plugging \eqref{eq:controller} into \eqref{eq:manipulator_equation}, and substituting in \eqref{eq:disturbance_equation}, one obtains 
    \begin{equation}
        \label{eq:modified_manipulator_equation}
        \begin{split}
            \robv(\qA(t), \Delta_0, [\Delta]) + \wdist(\qA(t), \Delta_0,\Delta) = \bM(q(t),\trueparams)\robrdot(t) + \\ + \bC(q(t), \dot{q}(t), \trueparams)\robr(t)
        \end{split}
    \end{equation}
    where
    \begin{align}
        \robr(t) &= \errdot(t) + K_r \err(t) \label{eq:modified_error}\\
        \robrdot(t) &= \errddot(t) + K_r \errdot(t).
    \end{align}
    
    In order to ensure persistent feasibility, we need to obtain a uniform bound on the modified tracking error $r: T \to \R^{\nq}$.
    First, we make the following assumption about the mass matrix $\bM(\qt,\trueparams)$:
    \begin{assum}\label{ass:eigenvalue_bound}
        Let $\lambdamin(\bM(\qt,\trueparams))$ and $\lambdamax(\bM(\qt, \trueparams))$ be the minimum and maximum eigenvalues of $\bM(\qt,\trueparams)$.
        There exists a uniform bounds $\sigma_m > 0$ and $\sigma_M > 0$ on these eigenvalues so that
        \begin{align}
            0 & < \sigm \leq \lambdamin(\bM(\qt,\trueparams)) \\
            0 & < \lambdamax(\bM(q,\trueparams)) \leq \sigM
        \end{align}
        holds for all $\qt \in Q$ and $\trueparams \in \intparams$. 
    \end{assum}
    This assumption is verified numerically during experiments.
    The following theorem, whose proof can be found in \cite{} \Zac{cite ARMOUR}, describes the construction of the robust input $\robv$ in order to achieve a uniformly bounded tracking error for $\robr$.
    \begin{thm}
        \label{thm:robust_controller}
        Suppose Assumption \ref{ass:eigenvalue_bound} is satisfied.
        Let $\roblevel > 0$ be a user-specified maximum value of the candidate Lyapunov function
        \begin{equation}
            \label{eq:lyap_r}
            \roblyap = \tfrac{1}{2}\robr(t)^\top \bM(q(t),\trueparams) \robr(t)
        \end{equation}
        and define 
        % \begin{equation}
        %     \label{eq:CBF_defn}
        %     \robh = -\roblyap + \roblevel.
        % \end{equation}
        % Next, let 
        \begin{equation}
            \label{eq:CBF_lower_bound}
            \begin{split}
                \robhmin \leq \inf_{\trueparams^* \in \intparams} -V(\qA(t),\Delta^*) + \roblevel
            \end{split}
        \end{equation}
         for all $\qA(t)$. Let $\robKinf:\R \to \R$ be some extended class $\mathcal{K}_\infty$ function (i.e., $\robKinf: \R \to \R$ is strictly increasing with $\robKinf(0) = 0$).
         Finally, suppose that $e(0) = \dot{e}(0) = 0$. %$r(0) \leq \ultbound$.
        
        Then, if the robust input is set equal to
        \begin{equation}
            \label{eq:robust_input}
            \robv(\qA(t), \Delta_0, [\Delta] ) = \begin{cases} 
            -\robcoeff(\qA(t),\Delta_0, [\Delta]) \frac{\robr(t)}{\norm{\robr(t)}} & \norm{\robr(t)} \neq 0 \\ 
            \phantom{-} 0 & \norm{\robr(t)} = 0 
            \end{cases} 
        \end{equation}
        with
        % \begin{equation}
        %     \label{eq:robust_coeff}
        %     \begin{split}
        %     \robcoeff(\qA(t),\Delta_0,[\Delta]) = \max\Big(0, \frac{-\robKinf(\robhmin)}{\norm{\robr(t)}} +  \\ \phantom{ \robcoeff(\qA(t),\Delta_0,[\Delta]) =}  + \norm{\wmax(\qA(t),\Delta_0,[\Delta])}\Big),
        %     \end{split}
        % \end{equation}
        \begin{equation}
            \label{eq:robust_coeff}
            \begin{split}
            \robcoeff(\qA(t),\Delta_0,[\Delta]) = \max\Big(0, \frac{-\robKinf(\robhmin)}{\norm{\robr(t)}} +  \\ \phantom{ \robcoeff(\qA(t),\Delta_0,[\Delta]) =}  + \frac{\abs{r(t)}^\top\wmax(\qA(t),\Delta_0,[\Delta])}{\norm{r(t)}}\Big),
            \end{split}
        \end{equation}
        and letting
        \begin{equation}
            \label{eq:ultimate_bound_defn}
            \epsilon \coloneqq \ultbound,
        \end{equation}
        then the modified tracking error trajectories $r: T \to \R^{\nq}$ are uniformly bounded by
        \begin{equation}
            \label{eq:ultimate_bound}
            \norm{\robr(t)} \leq \epsilon \qquad \forall t \in T
        \end{equation} when tracking reference trajectories that satisfy Def. \ref{def:traj_param}.
        \end{thm}
        
        
        
    %     Then, if the robust input is set equal to
    %     \begin{equation}
    %         \label{eq:robust_input}
    %         \robvk = \begin{cases} 
    %         -\robcoeff \frac{\robr}{\norm{\robr}} & \norm{\robr} \neq 0 \\ 
    %         \phantom{-} 0 & \norm{\robr} = 0 
    %         \end{cases} 
    %     \end{equation}
    %     with
    %     \begin{equation}
    %         \label{eq:robust_coeff}
    %         \robcoeff = \max\left(0, \frac{-\robKinf(\robhmin)}{\norm{\robr}} + \normwmax\right)
    %     \end{equation}
    %     then the modified tracking error trajectories $r: T \to \R^{\nq}$ are uniformly bounded by
    %     \begin{equation}
    %         \label{eq:ultimate_bound}
    %         \norm{\robr} \leq \ultbound \qquad \forall t \geq 0
    %     \end{equation}
    %     when tracking reference trajectories that satisfy Def. \ref{def:traj_param}.
    % \end{thm}
    
    Through Theorem \ref{thm:robust_controller}, the robust input $\robv$ can be constructed such that the tracking error trajectories $\robrnot: T \to \R^{\nq}$ are uniformly bounded. 
    This bound can be used to provide bounds on the position error and velocity error of the manipulator system, which we utilize for planning desired trajectories in Sec. \ref{sec:plan_alg_theory}.
    Importantly, this uniform bound applies for all $T$.
    
    \begin{cor}
        \label{cor:tracking_error}
        Suppose Assumption \ref{ass:eigenvalue_bound} is satisfied and $e(0) = \dot{e}(0) = 0$. 
        If $\robrnot: T \to \R^{\nq}$ is uniformly bounded as in \eqref{eq:ultimate_bound}, then the controller \eqref{eq:controller} with robust input \eqref{eq:robust_input} reaches any desired tracking performance provided a large enough gain matrix $K_r$.
        In particular, letting
        \begin{align}
            \pboundj &\coloneqq \frac{\epsilon}{K_{r, j}} \quad \regtext{and}\label{eq:ultimate_bound_position}\\
            \vbound &\coloneqq 2\epsilon\label{eq:ultimate_bound_velocity},
        \end{align}
        where $\epsilon$ as in \eqref{eq:ultimate_bound_defn} and $K_{r, j}$ is the $j$\ts{th} element of the diagonal gain matrix $K_r$, we have that $|\errj(t)| \leq \pboundj$ and $|\errjdot(t)| \leq \vbound$ for all $t \in T$.
    \end{cor}
    \noindent Theoretically, the tracking error bounds can be designed to be arbitrarily small, but they are practically limited by the physical capabilities of the manipulator.
    Attempting to enforce very small bounds would result in large torques being required, causing control input saturation.
    In Sec. \ref{sec:plan_alg_theory}, we explain how we overapproximate the torques required to track a given desired trajectory including all possible tracking error.
    Sec. \ref{sec:plan_alg_imp} details how these overapproximations are used to write constraints on the control input in order to prevent control input saturation.
    
% eq 48 and 49
% plug in interval inertial parameters for true or nominal inertial parameters?
% def 10
% lemma 11
% prop 12
% thm 14

% cor 15 important, req eq 60, 44, 58

% maybe just state that a uniform bound is developed which enables any desired tracking performance to be reached.

% also does this controller work for the trajectories that I am using? pretty sure it does




%%%%%%%%%%%%%%%%%%%%%%% Outline for Quick Reference %%%%%%%%%%%%%%%%%%%%%%%

%    \2 This section describes the passivity-based controller and how the TRO paper develops ultimate bounds on tracking performance.
%
%    \2 Theoretical Overview
%    
%        \3 Describe the nominal controller and how it does not guarantee perfect tracking since error can arise due to mismatches between the nominal and true parameters of the system.
%        
%        \3 Useful inclusions from the T-RO paper:
%        
%            \4 Nominal controller:
%            \begin{equation}\label{eq:nominal_controller}
%            \nominal,
%            \end{equation}
%            
%            \4 Modified reference velocity and acceleration trajectories:
%            \begin{align}\label{eq:modified_ref} % modified error
%            \qakdot &= \qdeskdot + K_r \err, \Hquad          \err = \qdesk - \q \\
%            \qakddot &= \qdeskddot + K_r \errdot,            \Hquad \errdot = \qdeskdot - \qd.
%            \end{align}
%
%            \4 Total control input:
%            \begin{equation}\label{eq:controller}
%            \controller,
%            \end{equation}
%        
%        \3 Short paragraph about how the T-RO U-ARMTD paper developed a robust controller and it is used in this paper as well. The main results are that given uncertainty in the inertial properties of the robot, the tracking error is uniformly and ultimately bounded. \Parker{Does this extend to uncertainty in the properties of the object placed on the tray?}
%        
%        \3 Useful inclusions from the T-RO paper:
%        
%            \4 \begin{defn}\label{def:worst_case_disturbance}
%            Let $\mathbb{I}\mathbb{R}^{n_q}$ be the set of all real-valued interval vectors.  
%            The \emph{measure of worst case disturbance} is the function $\rho: \mathbb{I}\mathbb{R}^{n_q} \xrightarrow{} \mathbb{R}^{n_q}$ which is defined as
%            \begin{equation}
%                \rho([\wdistinterval]) = \max(|\underline{\wdistinterval}|, |\overline{\wdistinterval}|)\label{eq:worst_case_disturbance},
%            \end{equation}
%            where the max$(\cdot)$ operator is applied element-wise over the interval vector.
%            \end{defn}
%            
%            \4 
%            \begin{prop}\label{thm:eigenvalue_bound}
%            Let $\intparams$ be an interval of inertial parameters.
%            % and let $[\bM] = [\bM(\cdot,\underline{\trueparams}), \bM(\cdot,\overline{\trueparams})]$ be the interval of corresponding inertia matrices. 
%            Define $\lambdamin(\bM(\q,\trueparams))$ and $\lambdamax(\bM(\q,\trueparams))$ to be the minimum and maximum eigenvalues of $\bM(\q,\trueparams)$, respectively.
%            % Let $\sigma_{m}(\trueparams)$ and $\sigma_{M}(\trueparams)$ be uniform bounds on the eigenvalues of $\bM(\cdot, \trueparams)$ \cite{Ghorbel1998uniform}.
%            There exist ultimate bounds $\sigma_m$ and $\sigma_M$ on the eigenvalues of the mass matrix so that
%            \begin{align}
%                \sigm &\leq \lambdamin(\Mq)\\
%                \sigM &\geq \lambdamax(\Mq)
%            \end{align}
%            holds for all $\q \in Q$ and $\trueparams \in \intparams$ \cite{Ghorbel1998uniform}.
%            % Let $\sigma_{m}(\trueparams)$ and $\sigma_{M}(\trueparams)$ be uniform bounds on the eigenvalues of $\bM(\q, \trueparams)$ for all $\q \in Q$ \cite{Ghorbel1998uniform}.
%            % Then for all $\trueparams \in \intparams$ and $\q \in Q$ we have
%            % \begin{align}
%            %     \sigma_{m}(\underline{\trueparams}) &\leq \lambdamin(\Mq)\\
%            %     \sigma_{M}(\overline{\trueparams}) &\geq \lambdamax(\Mq).
%            % \end{align}
%            \end{prop}
%            
%            \4
%            \begin{thm}
%            \label{thm:robust_controller}
%                % \pat{Robust input gives ultimate bound $\norm{\robr} \leq \ultbound \, \forall t > t_1$. Need to rearrange so these terms are introduced before the proof}
%                Let $\roblevel > 0$ be a user-specified maximum value of the candidate Lyapunov function
%                \begin{equation}
%                    \label{eq:lyap_r}
%                    \roblyap = \frac{1}{2}\robr^\top \Mq \robr.
%                \end{equation}
%                and, define 
%                \begin{equation}
%                    \label{eq:CBF_defn}
%                    \robh = -\roblyap + \roblevel.
%                \end{equation}
%                Next, let 
%                \begin{equation}
%                    \label{eq:CBF_lower_bound}
%                    \robhmin \coloneqq \inf_{\trueparams^* \in \intparams}\left(-\frac{1}{2}\robr^\top M(q, \trueparams^*) \robr \right) + \roblevel,
%                \end{equation}
%                and therefore $\robhmin \leq \robh$ for all $\q \in Q$ and $\robr \in \R^{n_q}$.
%                \shrey{It seems bits of the proof have leaked into this theorem statement}
%                For brevity, we define $\normwmax = ||\rho([\wdistinterval])||$.
%                Finally, let $\robKinf:\R \to \R$ be some extended class $\mathcal{K}_\infty$ function (i.e., $\robKinf: \R \to \R$ is strictly increasing with $\robKinf(0) = 0$ and is defined on the entire real line $\R = (-\infty, \infty)$.
%                
%                Then, the robust input
%            \begin{equation}
%                \label{eq:robust_input}
%                \robv = -\robcoeff \frac{\robr}{\norm{\robr}}
%            \end{equation}
%            with
%            \begin{equation}
%                \label{eq:robust_coeff}
%                \robcoeff = \max\left(0, \frac{-\robKinf(\robhmin)}{\norm{\robr}} + \normwmax\right)
%            \end{equation}
%            ensures the modified tracking error trajectories $\robrnot$ are uniformly ultimately bounded:
%            \begin{equation}
%                \norm{\robr} \leq \ultbound \qquad \forall t \geq 0
%            \end{equation}
%            when tracking reference trajectories that satisfy Def. \ref{def:traj_param}.
%            
%            \end{thm}
%            
%            \4
%            % as a corollary, the tracking error is uniformly bounded
%            \begin{cor}\label{cor:tracking_error}
%            If $\robrnot$ is ultimately bounded, then the complete controller \eqref{eq:controller} with robust input \eqref{eq:robust_input} reaches any desired tracking performance provided a large enough gain matrix $K_r$.
%            In particular, letting
%            \begin{align}
%                \pbound &\coloneqq \frac{1}{K_r}\ultbound \label{eq:ultimate_bound_position}\\
%                \vbound &\coloneqq 2\ultbound,\label{eq:ultimate_bound_velocity}
%            \end{align}
%            \pat{@jon might need your help proving these...}
%            we have that $|\errj| \leq \pbound$ and $|\errjdot| \leq \vbound$ for all time.
%            \end{cor}
%        
%    \2 Numerical Implementation
%    
%        \3 Describe the numerical implementation of RNEA and IRNEA which are used to compute the robust input to the controller, as well as the contact forces for the waiter motion constraints.

==> Sections/experimental.tex <==
\section*{Experimental}
\label{sec:experiments_old}

This section details the implementation and testing of the \MethodName{} framework. \MethodName{} is implemented in MATLAB and was run on \Zac{insert computer details}. A comparison framework was built using GPOPS-II, and we test both frameworks in several scenarios. The control input trajectories for both frameworks were used in a verification simulation for each experiment using the PyBullet simulation environment.

\subsection{Implementation Details}

    \subsubsection{Simulation: Robot Model and Environment}
        % use Fetch Robot as the base manipulator. 
        % sample poses and eigenvalue was bounded by
        % use a modified Fetch URDF which has a tray added as a link. 
        % for matlab, the urdf also has a cylinder added as a link
        % for pybullet simulation, the cup is a separate body and is loosely placed on the tray.
        % uncertainty setups?
        
        We use a Fetch robot which is composed of 7 revolute joints \cite{wise2016fetch}.
        A thin tray with a mass of $1$ kg is added to the robot model as described in Assumption \ref{assum:contact}.
        For implementation in MATLAB, both frameworks have a cylinder with a mass of $0.25$ kg added to the robot model as well, which enables PZRNEA to calculate the contact wrench.
        For the verification simulation in PyBullet, the same cylinder is added to the simulation environment separately from the Fetch robot grasping the tray.
        PyBullet uses the built in contact model to simulate the interaction between the cylinder and tray.
        Millions of configurations of the Fetch robot were sampled and we found that the minimum eigenvalue of the mass matrix was uniformly bounded from below by $\sigma_m = 0.0017$. \Zac{need to repeat this when the robot has the tray and cup added?}
        
        % setup for experiment 1: no obstacles
        % setup for experiment 2: 10 random obstacles
        % setup for experiment 3: uncertainty and 10 random obstacles
        % vary the mass of the object by $\pm3%$, and the inertia matrices adjust accordingly.
        
    \subsubsection{Trajectories}
    
        We let $t_{plan} = 0.5s$ and $t_{f} = 1s$ for a single planning iteration.
        % selection of c_j and g_j
        As in Eq. \eqref{eq:bernstein_k_coeff}, we let $\kjoffset = \initqj$ and $\kjscale = \frac{\pi}{24}$, so that after $\tfin = 1$s the final position of any joint's trajectory can differ from its initial position by up to $\pm\frac{\pi}{24}$ radians. \Zac{update as needed}
        
    \subsubsection{Controller}
        
        % gain matrix for K_r
        % robust controller parameters
        For the nominal passivity-based controller we set $K_r = 10 I_7$, where $I_7$ is a $7 \times 7$ identity matrix.
        %\Zac{need to ask where these parameters are set}
        
        For the robust controller, we set $\alpha(y) = y$.
        This satisfies the requirement that $\alpha: \R \to \R$ is an extended class $\mathcal{K}_\infty$ function (i.e., $\robKinf: \R \to \R$ is strictly increasing with $\robKinf(0) = 0$ and is defined on the entire real line $\R = (-\infty, \infty)$.
        We let the Lyapunov function threshold be $\roblevel = 3.1 \times 10^{-7}$.
        Together with the bound on the smallest eigenvalue $\sigma_m$, this yields the uniform bound
        \begin{equation}
            ||\robr|| \leq \ultbound = \sqrt{\frac{2 \times 3.1 \times 10 ^ {-7}}{0.0017}} \approx 0.0191.
        \end{equation}
        Plugging into the position \eqref{eq:ultimate_bound_position} and velocity \eqref{eq:ultimate_bound_velocity} bounds yields $\pboundj \approx 0.00191 \text{ rad}$ and $\vbound \approx 0.0382 \text{ rad/s}$.
        \Zac{this needs to be updated}
    
    \subsubsection{Polynomial Zonotopes}
    
        \MethodName{} builds upon the CORA Toolbox \cite{althoff_cora} for generating and performing arithmetic operations with polynomial zonotopes. 
        We maintain a maximum zonotope order of 40 through reducing the polynomial zonotopes.
        A reduction operation for a polynomial zonotope is given in Eq. \eqref{eq:pz_reduce}.
        
    \subsubsection{High-level Planners}
    
        Recall that the \MethodName{} framework can be implemented with a user-specified cost function, which is minimized during each planning iteration subject to the constraints discussed in Sec. \ref{sec:plan_alg_theory}. 
        For this work, we use a cost function which minimizes the distance between $q(t_{f};k)$ and an intermediate waypoint. 
        A straight-line high-level planner generates the intermediate waypoint along a straight line in configuration space between the current state and the global goal state. 
        Note that the high-level planner does not need safety guarantees, meaning that a generated waypoint could result in an infeasible state if it were reached.
        The \MethodName{} framework is independent of the high-level planner, so it still enforces continuous-time safety.
        
    \subsubsection{Comparison Framework}
    
        % Discuss how the comparison framework works using GPOPS-II as the optimization solver
        A comparison framework was built in MATLAB using GPOPS-II \Zac{cite GPOPS} as the optimization solver. 
        The GPOPS-II framework uses the same high-level planner and cost function as the \MethodName{} framework. 
        However, GPOPS-II is solving the optimization problem given in Eq \eqref{eq:optcost}-\eqref{eq:opttipcon}.
        Each GPOPS-II call is initialized with the current state as the initial condition and the intermediate waypoint provided by the high-level planner as the goal state. 
        The control inputs that are output by the GPOPS-II solver are used to simulate the system forward using built-in MATLAB ODE solvers. 
        The end state from the ODE forward simulation is used to update the current state and therefore initialize the next GPOPS-II call. 
        This is repeated until the overall goal state is reached or a constraint violation is detected in the forward simulation. 
        
        % use the output trajectories of both in PyBullet to simulate contact between the cylinder and manipulator system.
        
    \subsubsection{Trajectory Optimization Implementation}
        
        % use fmincon
        The \MethodName{} framework uses MATLAB's $\texttt{fmincon}$ to solve the trajectory optimization problem during each planning iteration. \Zac{cite fmincon?}
        % cost function
        The cost function is  $f(k) = \norm{q(\tfin; k) - q_{\regtext{des}}}$, where $q_{\regtext{des}}$ is the intermediate waypoint provided by the high-level planner.
        Analytic gradients/subgradients of the cost function and constraints are provided for the optimization solver to speed computation.

\subsection{Experiment 1}

    \subsubsection{Setup}
        % 100 random trials that have feasible start and goal positions
        % obstacles?
        %A modified Fetch robot model \Zac{cite something here?} with a tray and cup added to the URDF was used for the simulation \Zac{could change to simulation in pybullet which is different}. 
        %It was assumed that the fetch robot could maintain force closure on the tray. \Zac{talk about cup not actually loosely placed in URDF, but including it in this way enables calculation of contact wrench using PZRNEA?}
        The first experiment focuses on testing the ability for the frameworks to operate in an obstacle free environment.
        The two frameworks were tested in 100 random trials where each trial was initialized with a random feasible start and goal state. 
        \Zac{mention time overall time limit?}

    \subsubsection{Results}
    
        % table of results
        \begin{table}[]
        \label{tab:experimental_results}
            \centering
            \begin{tabular}{c|c|c c c c}
                 Exp & Method & Goals Reached & Crashes & Safe Stops & Time Outs \\
                 \hline
                 1 & \MethodName{} & 100 & 0 & 0 & 0 \\ 
                 & GPOPS & 50 & 50 & 0 & 0 \\
                 \hline
                 2 & \MethodName{} & ? & ? & ? & 0 \\ 
                 & GPOPS & 10 & 90 & 0 & 0 \\
                 \hline
                 3 & \MethodName{} & 83 & 0 & 13 & 0 \\ 
                 & GPOPS & 10 & 90 & 0 & 0 
            \end{tabular}
            \caption{Results for 100 random scenarios for two optimization methods, \MethodName{} and GPOPS.}
            \label{tab:my_label}
        \end{table}
    
        % discuss results
        The results of the 100 random trials are presented in \ref{experimental_results}, with a single trial result shown in \ref{} \Zac{reference a results figure here}. 
        \MethodName{} safely reaches the goal state in a large majority of the trials. 
        In cases where the goal is not reached, it safely comes to a stop in a feasible position and is unable to find a new safe trajectory to execute. 
        \Zac{use exact numbers when have them} \Zac{GPOPS-II results here, expecting some successes and some failures}. 
        Further, the \MethodName{} framework takes roughly 30 seconds per planning iteration in the MATLAB implementation while GPOPS-II takes roughly 20 hours per planning iteration. 
        \Zac{note that the MATLAB implementation could be transferred to CUDA for real-time performance?}

        \Zac{Explain why stops occur? The safe stops for the \MethodName{} framework is caused due to a contact constraint being near a boundary when a braking maneuver is executed. In the following planning iteration, having the overapproximations buffered by the independent generators shifts the overapproximation across the constraint boundary, so while the current state is feasible, the optimization solver is unable to find a safe solution to move forward.} \Zac{could show a figure of this as well} 

        \begin{figure}
            \centering
            \includegraphics[width=0.9\columnwidth]{Figures/ExpResultsv3.jpg}
            \caption{Caption}
            \label{fig:our_method_exp1}
        \end{figure}
            
        \begin{figure}
            \centering
            \includegraphics[width=0.9\columnwidth]{Figures/ExpResultsv4.jpg}
            \caption{Caption}
            \label{fig:comparison_exp1}
        \end{figure}

\subsection{Experiment 2}

    \subsubsection{Setup}
    The second experiment tests the ability of the \MethodName{} framework to operate in environments where obstacles are present.
    Both frameworks were tested in 100 random trials where each trial had 10 box shaped obstacles in the workspace.
    The obstacles were random sized and randomly placed in the workspace.
    The side lengths of the obstacles were allowed to vary between $1$ to $50$ cm.
    Each trial had a random but feasible initial and goal state.
    
    \subsubsection{Results}
    \Zac{will fill in once results are ready}
    
\subsection{Experiment 3}

    \subsubsection{Setup}
    The third experiment tests the ability of the \MethodName{} framework to operate in the presence of uncertainty in the parameters of the system.
    Both frameworks were tested in 100 random trials where each trial had 10 random obstacles like experiment 2.
    We then introduce uncertainty in the mass of the cylinder being manipulated by allowing the mass to vary by $\pm3\%$.
    The inertia matrices vary accordingly, and the rest of the parameters remain the same.
    The new inertial parameters are denoted by $\intparams_{cyl}$
    
    % do coefficient of friction or the radius of contact area?
    
    \subsubsection{Results}
    \Zac{will fill in once results are ready}

% \subsection{Future Directions}
% Sloshing
% Closed loop PZRNEA for environment interactions and force closure on objects
% Reorientation of objects being manipulated


% ---------------------------------------
% From the outline

    % \2 One Object Simulation
        
    %     \3 Ran 100 trials with random initial/goal configurations. Expected results are:
            
    %         \4 \MethodName{}
    %             \5 no failures
    %             \5 some safe stops
    %             \5 computation time: on the order of minutes for a single trajectory and 30 seconds for a single planning iteration.
            
    %         \4 GPOPS
    %             \5 might have failures
    %             \5 not sure how to do safe stops
    %             \5 computation time: on the order of hours to days for a single trajectory and hours for a single planning iteration.
                
    % \2 Table of Simulation Results
    
    

==> Sections/introduction.tex <==
\section{Introduction}
\label{sec:intro_old}

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{Figures/RTD_Force_Figure1_v1-01.png}
    \caption{Caption}
    \label{fig: Overview of the proposed method. We consider safe planning of a manipulator with uncertain dynamics that firmly grasps a tray with uncertain object(s) placed on it.}
\end{figure}

\subsection{Background and Motivation}

    % re-explain waiter motion problem as industrial focused, highly structured environment. cooperative manufacturing, human collaboration, etc.
    
    % Motivation
    Robotic manipulators have the potential to revolutionize the manufacturing industry, the service industry and even everyday households. 
    Yet, they commonly operate in highly structured and isolated environments in factories and warehouses. % where they perform manipulation tasks that are well defined. % and repetitive.
    In order to transition robotic manipulators into unstructured environments and tasks, they will need to be able to operate in close proximity to humans and interact with objects whose properties are uncertain. 
    This transition can be realized through developing planning and control methods which can guarantee safe continuous-time operation of a robotic manipulator while it reacts to its unstructured environment. 
    
    %Many robotic manipulators are equipped with grippers, which often try to capture the dexterity and adaptability with which human hands can manipulate objects. 
    % A large portion of manipulation tasks are achieved through using a robotic hand or gripper which maintains form- or force-closure on the object being manipulated.
    % drawbacks of prehensile manipulation? severely restrict the range of objects depending on the gripper
    This paper focuses on an important sub-problem of non-prehensile robotic manipulation, the waiter motion problem, which has comparable tasks in industry applications.
    In this problem, a robotic system achieves manipulation of loosely placed objects through applying a contact wrench to the objects.
    Safely and successfully manipulating objects through a desired trajectory without relative motion to its supporting surface requires proper application of a contact wrench to each object. 
    If an incorrect contact wrench is applied, then the contact mode switches and affects the dynamics of the system.
    This can easily result in failure modes, such as the objects falling from their supporting surface or the robotic system colliding with an obstacle.
    % This paper focuses on non-prehensile manipulation, which means that an object is free to roll, slide or break contact with the manipulator. % instead
    % nonprehensile is challenging because... could cite the Ruggiero survey paper here. changing dynamics based on contact state (our contact state does change though)?
    % Manipulation of the object is achieved through the applied contact wrench from the manipulator.
    % Determining a trajectory from a start to goal state can be challenging due to changing dynamics based on switches in contact modes.
    % something about planning and motion control
    Current planning and control methods for the waiter-motion problem cannot guarantee continuous-time safety during execution of a desired trajectory. % has yet to be demonstrated. % bold claim
    % While non-prehensile manipulation enables a manipulator to use any surface to forcefully interact with an object, safely controlling the interaction forces has yet to be demonstrated. % bold claim probably
    % \Zac{talk about force constraints in nonprehensile manipulation and safely but forcefully interacting with the environment}
    % describe the problem
    An important example of non-prehensile manipulation, which requires safe control of the applied contact wrench, is the waiter motion problem.
    In this problem, a manipulator seeks to manipulate a loosely placed object such that the object does not move relative to the supporting surface of the manipulator that it is in contact with.
    Since the object is loosely placed, meaning free to roll, slip or break contact, the applied contact wrench needs to be constrained to prevent relative motion of the object.
    Failure to do so can result in the dynamics of the system changing as a contact mode switches, potentially leading to objects falling off the supporting surface or the manipulator running into an obstacle in the environment.
    % In order to deploy a system in a real-world scenario, a motion planning and control framework which is robust to uncertainty and can guarantee safety is crucial.
    This task can be applied to transport of goods in factories and warehouses, serving of food in restaurants, and beyond.
    %This example is illustrative of many tasks found in industry.
    % \pat{I think here you can say that most manipulation tasks require rigidly grasping an object in a hand or gripper, and then introduce the concept of non-prehensile manipulation. Then, introduce the waiter problem as an example of non-prehensile manipulation, and what its applications could be.} \Zac{added}
    
    % difficult to achieve dynamically stable manipulation of loose object?
    
    %An important example of a real-world task which requires safety and robustness to uncertainty is the waiter-motion problem, which consists of a robot manipulating a loosely placed object to a goal state such that the object does not move relative to the surface it is resting on and the entire system does not collide with obstacles.
    % The gap
    The focus of current methods addressing the waiter motion problem has been generating time-optimal trajectories for manipulation of loosely placed objects.
    This focus stems from current methods tackling the problem from the viewpoint of industrial or warehouse environments, despite its namesake invoking an image of a robot waiter in a busy restaurant.
    % In these structured environments, the manipulator is generally performing a repeated task with perfect knowledge of the parameters of the object being manipulated.
    As such, current methods for solving this problem often rely on assumptions such as perfect knowledge of the environment, object and manipulator and that tracking error is negligible.
    In an industrial setting, these assumptions can be valid, but place heavy restrictions on the range of objects that can be manipulated and on the robotic system being used.
    % The effects of these assumptions are discussed in depth in the related works section.
    % \pat{It might be worth saying here that these assumptions are discussed in depth in the related work section.} \Zac{added}
    %In contrast, this work seeks to approach the problem when the environment is unstructured, there is uncertainty both in the parameters of the manipulator and the object being manipulated, and tracking error is non-negligible.
    Current methods are not suitable for more unstructured environments or when uncertainty is present, such as in a busy restaurant, or a collaborative manufacturing environment.
    Therefore, different planning and control methods which can guarantee that a manipulator operates safely in environments that are unpredictable are needed.
    
    % key properties and why they are important
    There are two key properties that such a method needs to satisfy in order to address the waiter motion problem. 
    The first property is the ability to guarantee safety for all time (e.g. the manipulator will never collide with obstacles and the loosely placed object will never move relative to the supporting surface). % also that trajectories are dynamically feasible?
    This is crucial for deployment in unstructured environments, such as where humans are present, in order to prevent harm and also to ensure that the task of manipulating an object is successful. 
    % note that current methods assume model of robot and object, and knowledge of environment are good enough that discretization isn't a problem?
    The second property is the ability to robustly handle uncertainty in properties of the manipulator and the object being manipulated. 
    When deployed into real-world scenarios, robotic manipulators will be expected to manipulate arbitrary objects in their environment. 
    Such interactions will not come with perfect \textit{a priori} knowledge of the properties of the object, and sensors cannot provide exact measurements of the properties, resulting in uncertainty that the robotic manipulator must be able to handle in order to operate in a safe manner. 
    % Third property is real-time performance? % only if we get it working in real-time?
    % mention need receding horizon framework and therefore not worried about time-optimality
    
    
    % I guess I am trying to solve a different problem from the general waiter-motion problem that is introduced in other papers. I am saying time-optimal does not matter and instead, a robotic manipulator should be able to plan a guaranteed safe and uncertainty robust motion in a receding horizon fashion. The current general waiter-motion problem is focused on more structured industrial environments and not real-world environments that change with time. 
    
    % Current papers make assumptions, such as exact manipulator model (and high quality sensors), known object properties where variance is negligible and a given pre-specified path which doesn't need collision checking (not all), which are valid in an industrial environment, but will not generalize to changing and unstructured environments and tasks. In addition, the lack of guaranteed safety will prevent adoption due to either slow operation (slow computation and execution time) or risk of accidents. Each of these methods discretize, and while finer discretization increases likelihood of safe trajectory, it is not guaranteed and comes with computational cost. 
    % even in industrial settings, accidents can still occur.
    
    % in fact, humans as waiters tend keep the tray with loosely placed objects parallel to the ground, which does not result in a time-optimal motion, but instead helps to ensure safety.
    
    % time-optimal methods often result in trajectories that operate at the limits of the system (e.g. maximum accelerations), which would be sensitive to uncertainty in the manipulator model or object properties. Discretization would therefore lead to failure with robustness against uncertainty.

\subsection{Related Work}

    % organization of papers. 
        % only solve time-optimal of pre-specified geometric path
            % sort in here by constraint or type of problem (convex vs nonconvex?)
            % uncertainty (iterative learning paper)
        % solve for geometric path, then time-optimal trajectory
        
    % \cite{Nagy2018} - time optimal problem, slipping and jerk constraint (no torque bc don't know robot parameters), discretize super fine and say tracking error negligible because industrial robot, use Gurobi. (comes after \cite{Csorvasi2017})
    % \cite{Csorvasi2020} - same group as Nagy, slipping constraint, high end industrial robot so ignore tracking error. main difference is this paper optimizes a much longer path using a sequential solver
    % \cite{Gattringer2022} - trajectory geometry optimization and time-optimal optimization. 
    
    % Simplify to a time-optimal path following task
    The waiter motion problem has previously been simplified and treated as a time-optimal path following task, which assumes a geometric path is given. The problem is formulated as an optimization problem whose solution is a near time-optimal trajectory along the pre-specified path \cite{Debrouwere2013,Csorvasi2017,Gattringer2022,Gattringer2022a}. 
    The time-optimal trajectory is subject to constraints such as a friction cone constraint in \cite{Csorvasi2017}, as well as a lift and tipping constraint in \cite{Debrouwere2013} and a rotational friction cone constraint in \cite{Gattringer2022,Gattringer2022a}.
    It is important to note that in order to completely constrain relative motion of the loose object with respect to its supporting surface, all six degrees of freedom need to be constrained.
    Also, the geometric path in these methods is user-specified, thus it is assumed that the given discretized path is safe.
    
    % talk about the methods they use? \cite{Gattringer2022a, Gattringer2020} use a multiple shooting method. \cite{Debrouwere2013,Csorvasi2017} use a convex SOCP. 
    Other methods incorporate the optimization of the geometric path as well as solving for the time-optimal trajectory along that path \cite{Flores,Ichnowski2021,Avigal2022,Gattringer2022}.
    Gattringer et al. \cite{Gattringer2022} uses a multiple shooting method, subject to all of the constraints mentioned above, to determine an optimal discretized geometric path, and the time-optimal trajectory along that path. % no collision avoidance constraint
    While \cite{Ichnowski2021} and 
    \cite{Avigal2022} apply their framework to two similar problems to the waiter-motion problem, resulting in different constraints being implemented, the underlying framework, which is built upon the GOMP framework 
    \cite{Ichnowski2020}, aims to achieve a similar overall task of safe motion planning. % not sure how best to fit in these two papers since they tackle a different problem
    
    % Rodriguez paper here. They consider constraints on whether joints (revolute and frictional) can support an exerted wrench. frictional is related. 
    
    However, all of these methods do not meet the two key properties for a solution to the waiter problem.
    Each method discretizes and evaluates the constraints of the optimization problem, which means that the constraints are enforced only at discrete time points. 
    While finer discretization leads to a higher likelihood that the trajectory is safe, it does not guarantee safety for all time and comes at the cost of higher computation time. %, meaning that real-time operation is sacrificed. 
    % \Zac{Change this sentence to say that if the pre-specified geometric path were generated by other common methods, the discretization drawback still applies?} The methods that rely on a given geometric path generated from TrajOpt \cite{} or CHOMP \cite{} also do not have guarantees about collision-free trajectories for all time since TrajOpt and CHOMP must discretize as well. 
    % Therefore, these methods cannot guarantee safety for all time. 
    Discretization also means that these methods are vulnerable to uncertainty.
    Since they are formulated as time-optimal problems, the resulting trajectories generally have the robot operate at the maximum feasible limits.
    Uncertainty in parameters of the manipulator and object (e.g. mass, inertia, static coefficient of friction, etc) will cause tracking error while executing a desired trajectory. 
    If not dealt with robustly, uncertainty in the properties of the manipulator or object being manipulated could result in the executed trajectory being unsafe.
    These approaches are suitable for the assumed highly structured environment, such as an industrial setting, where the robot model is known, operates very accurately and performs a well defined task. 
    %a path is repeated many times and can therefore be computed beforehand and then repeatedly executed, offsetting the computation time. 
    But they do not meet the two key properties for deployment in unstructured environments where uncertainty is present. 
    
    Uncertainty in both parameter estimation and execution error was considered in \cite{Luo2017}, where interval-based uncertainty was applied to the coefficient of friction, the center of mass and contact locations of manipulated objects and errors due to control and disturbances.
    % only show COF (for waiter-motion) and ZMP (for walking robot)
    However, the same drawbacks due to discretization apply to this method as well.
    % no safety guarantee, it is fast, but not real-time (10s to generate dynamically feasible trajectory). focused more on learning
    % iteratively learn bounds on the uncertainty through trial and error. requires failures to learn. not sure how generalizable
    % do not handle inertial parameters
    
    % focusing not on time-optimality but safety, this is on the mid level of control and not the high level. our method provides safety at the mid level, and time-optimality can be achieved by designing better high level planners to select better waypoints.

\subsection{Contributions}

    We make two main contributions in this paper.
    First, we extend the ARMTD and \TROtitle{} safe motion planning frameworks to consider the wrenches exerted throughout a kinematic chain of a manipulator, including contact wrenches applied to manipulated objects.
    Second, we apply this framework to the waiter motion problem, resulting in a novel approach which can operate safely in a receding horizon fashion while robustly accounting for uncertain manipulator dynamics and uncertain properties of the object being manipulated.
    The framework is tested in simulation and compared against another framework which uses a different optimization solver. 
    % not sure what to highlight as the main theoretical contribution since this is basically just adding three constraints to the ARMOUR framework. 
    % \Zac{highlight difference from other related works. taking ARMTD approach in motion planning and applying it to the waiter-motion problem. online planning reacting to uncertain and changing environment. more water can be handled for instance.}

\subsection{Overview of Proposed Method}

    We give a brief overview of the \MethodName{} framework and the structure of this document.
    %% Notation Section
    First, we present relevant notation and mathematical objects.
    Then we describe the robot kinematics and dynamics, the robot's environment, and how we model and calculate the contact interactions for the waiter motion problem in Sec. \ref{sec:modeling}.
    %% Contact Modeling
    Next, we explain 
    % Then we detail our use of a recursive Newton-Euler algorithm (RNEA) to calculate the robot dynamics as well as the contact wrench the robot exerts on a loosely placed object (Sec. \ref{}).
    % feel like contact modeling might be best after or during trajectory design?
    The next sections walk through our motion planning and control hierarchy, which has three levels: a high-level planner (HLP), a mid-level safe trajectory planner, and a low-level robust controller.
    % talk about receding horizon?
    %% Trajectory Design
    First, we describe the parameterized set of desired joint trajectories that the mid-level safe trajectory planner uses (Sec. \ref{sec:traj_des}).
    An online trajectory optimization program optimizes over this set, resulting in a desired trajectory that is tracked by the low-level robust controller.
    The cost function of this program is arbitrary, and in this paper is set to the distance from a waypoint output from a HLP.
    %% Controller Design
    In Sec. \ref{sec:control_des}, we detail the low-level robust controller, which is a passivity-based controller that has ultimate bounds on tracking error and can handle uncertainty in the manipulator dynamics and object properties.
    While the controller tracks a desired trajectory, the mid-level planner is solving for the next desired trajectory, forming the receding horizon structure of this framework.
    %% Planning Algorithm Theory
    In Sec. \ref{sec:plan_alg_theory}, we describe how polynomial zonotope overapproximations are generated for the manipulator's trajectory, inputs and contact forces and how those are used to write constraints for the discrete-time trajectory optimization problem solved during each planning iteration.
    We also explain how these overapproximations enable safety guarantees about continuous time operation.
    % Reachable Set Construction
    % JRS, FK, FO, Input RS, Wrench RS, using PZs
    % Constraint Generation
    % Trajectory Optimization
    %% Planning Algorithm Implementation
    % PZFK, PZFO, PZRNEA for inputs and wrenches
    Sec. \ref{sec:plan_alg_imp} details the numerical implementations, using the polynomial zonotope overapproximations, of the forward kinematic (PZFK), forward occupancy (PZFO) and RNEA (PZRNEA) algorithms and the constraints written using their outputs.
    %% Experiments
    In Sec. \ref{sec:experiments}, 
    we test the \MethodName{} in simulation and compare against a similar framework.
    % Conclusion
    Lastly, we conclude and describe our future work in Sec. \ref{sec:conclusion}.




%%% Goals

% describe problem

% describe what properties matter and why

% the way they try to solve the problem

% table of papers

==> Sections/modeling_contact.tex <==
\section{System Environment, Kinematics and Dynamics} % Modeling of Contact Interactions
\label{sec:modeling}

This section introduces the kinematics and dynamics of the robotic manipulator, defines the environment it operates in and explains how contact interactions are modeled. % \Zac{obstacles if they make it in}

% \Zac{different title? System Kinematics and Dynamics? Introduce the kinematics and dynamics in trajectory design? and move modeling of contact to after trajectory design or later?}
% describe obstacles as well?

\subsection{Robotic Manipulator Model}

    We consider a robotic manipulator which is composed of $\nq$ revolute joints, with the $j^{th}$ joint actuating the robot's $j^{th}$ link. 
    Given a compact time interval $T \subset \R$, the configuration trajectory for the robot is defined as $q: T \to Q \subset \R^{\nq}$. 
    % assumptions
    We make the following assumptions about the robot model:
    \begin{assum}
        % moved workspace assumption to environment
        Joints with multiple degrees of freedom may be represented in this framework using links with zero length.
        The robot's $j^{th}$ joint has position and velocity limits given by $\qj \in [\qlim^-, \qlim^+]$ and $\qdj \in [\dqlim^-, \dqlim^+]$ for all $t \in T$, respectively.
        The robot is fully actuated, where the robot's input $u: T \to \R^{\nq}$ has limits that are given by $u(t) \in [\ulim^-, \ulim^+]$ for all $t \in T$.
    \end{assum}
    
\subsection{Manipulator Kinematics}
    
    % world frame
    % base frame
    Let there be a fixed inertial reference frame which we will refer to as the \textit{world} frame, and a \textit{base} frame, denoted as the $0^{th}$ frame.
    The base frame indicates the origin of the kinematic chain of the manipulator.  
    % link frames and axis of rotation (x-axis)
    The $j^{th}$ joint of the manipulator has a reference frame given by $\{\hat{x}_j, \hat{y}_j, \hat{z}_j\}$ where $\hat{x}_j$ is aligned with the axis of rotation for the corresponding joint.
    % homogeneous transformations
    A homogeneous transformation can be written to describe the configuration $\qj$ of reference frame $j$ with respect to the reference frame $j-1$ for a given time $t$ \cite[Ch. 2]{spong2005textbook}:
    \begin{equation}
        T_{j}^{j-1}(\qj) = 
        \begin{bmatrix} R\jssmu (\qj) & p\jssmu \\
        \mathbf{0}  & 1 \\
        \end{bmatrix},
    \end{equation}
    where $R\jssmu (\qj)$ is a configuration-dependent rotation matrix and $p\jssmu$ is the fixed translation vector from frame $j-1$ to frame $j$.

    % forward kinematics
    The forward kinematics of the manipulator are given by the map $\FK_j(\q): Q \to \R^{4 \times 4}$, which takes the manipulator's configuration at time $t$ and maps it to the position and orientation of the $j^{th}$ joint in the base frame.
    This map can be expressed as follows:
    \begin{equation}
        \label{eq:fk_j}
        \FK_j(\qt) = 
        \prod_{l=1}^{j} T_{l}^{l-1}(q_l(t)) = 
        \begin{bmatrix} R_j(\qt) & p_j(\qt) \\
        \mathbf{0}  & 1 \\
        \end{bmatrix}
    \end{equation}
    %\Zac{\st{should the $\qj$ in the product be $q_l(t)$ instead? also, should the matrix have a $R_{j}$ and $p_{j}$} fixed}
    %\pat{i think so, good catch!}
    where 
    \begin{equation}
        R_j(\qt) \coloneqq R_j^{0}(\qt) = \prod_{l=1}^{j}R_{l}^{l-1}(\ql)
    \end{equation}
    and 
    \begin{equation}
        p_j(\qt) = \sum_{l=1}^{j} R_{l}(\qt) p_{l}^{l-1}.
    \end{equation}
    % note this p_j depends on q(t) since it is jth frame wrt the base frame and not the preceding frame
    
\subsection{Manipulator Occupancy}
    
    % In order to avoid obstacles, the volume which the manipulator occupies needs to be determined.
    Using the forward kinematics of the manipulator, the volume which the manipulator occupies in the workspace can be calculated.
    Let the volume of the $j^{th}$ link in the corresponding reference frame be denoted by the set $L_j \subset \R^3$.
    The forward occupancy of the $j^{th}$ link is:
    \begin{align}
        \label{eq:forward_occupancy_j}
         \FO_j(\qt) &= p_j(\qt) \oplus R_j(\qt) L_j,
    \end{align}
    Then, the volume occupied by the entire arm in the workspace is given by the function $\FO: Q \to \pow{W}$ where
    \begin{align}
        \label{eq:forward_occupancy}
        \FO(\qt) = \bigcup_{j = 1}^{\nq} \FO_j(\qt) \subset W. 
    \end{align}

\subsection{Manipulator Dynamics}

    We assume the robotic manipulator is composed of $\nq$ rigid links with inertial parameters given by the vector
    \begin{equation}
        \label{eq:true_intertial_parameters}
        \Delta = (m_1, \dots, m_{\nq}, c_{x,1}, \dots, c_{z,{\nq}}, I_{xx,1}, \dots I_{zz,{\nq}})^{T}
    \end{equation}
    where $m_j$, $c_j =(c_{x,j}, c_{y,j}, c_{z,j})\trans$, and $(I_{xx,j}, \dots, I_{zz,j})\trans$  represent the mass, center of mass, and inertia tensor of the $j^{th}$ link, respectively. 
    The dynamics are represented by the standard manipulator equations \cite{spong2005textbook}
    \begin{equation}
        \label{eq:manipulator_equation}
        \roboteqn    
    \end{equation}
    where $\Mq \in \R^{\nq \times \nq}$ is the positive definite inertia matrix, $\Cqd$ is the Coriolis matrix, $\Gqd$ is the gravity vector, and $u(t;k)$ is the input torque.
    In addition, the following assumptions regarding the robot's dynamics are made.  
    \begin{assum}
    \label{assum:arm_model}
    We assume the model structure of the robot is known, but its true inertial parameters are unknown. 
    We assume the uncertainty in each inertial parameter is known and given by the interval vector
    \begin{equation*}
        % \begin{split}
        [\Delta] = \left( [m_1], \dots, [m_{\nq}], [c_{x,1}], \dots, [c_{z,{\nq}}], \left[I_{xx,1}\right], \dots, [I_{zz,\nq}] \right) \trans
        % \end{split}
    \end{equation*}
    where $[m_j] \subset \mathbb{IR}$, $[c_j] \subset \mathbb{IR}^3$, and $[I_j]\subset \mathbb{IR}^{3 \times 3}$ represent the uncertainties in the mass, center of mass, and inertia tensor of the $j^{th}$ link, respectively.
    We assume there is a nominal vector of inertial parameters $\Delta_{0} \in [\Delta]$ which is an estimate of the true inertial parameters and that $\Delta \in [\Delta]$.
    \end{assum}
    Note that the nominal vector $\Delta_{0}$ does not need to be a good estimate of the true inertial parameters $\Delta$.
    
\subsection{Environment and Obstacles}
    
    This section describes the environment of the manipulator and how we treat obstacles in that environment.
    First, we make the following assumptions:
    \begin{assum}
        \label{assum:obstacles}
        The manipulator operates in a three dimensional workspace, which we denote $W \subset \R^3$.
        At any time, the number of obstacles $\nObs \in \N$ in the workspace is finite ($\nObs < \infty$).
        Let $\obsset$ be the set of all obstacles $\{ O_1, O_2, \ldots, O_{\nObs} \}$.
        % \pat{$\obsset$ is a set here, but we use it like it's the union of obstacles when writing the trajopt}
        Each obstacle is convex, bounded, and static with respect to time.
        % The robot has access to a conservative estimate of the size and location of each obstacle (this work is concerned with planning and control, not perception).
        %The obstacle's volume in workspace $W$ can be overapproximated by a zonotope.
    \end{assum}
    \noindent Note this work is concerned with planning and control around obstacles, not perception of obstacles.
    If a portion of the scene is occluded then one can treat that portion of the scene as an obstacle. % define scene somewhere?
    Given Assumption \ref{assum:obstacles}, a convex, bounded object can always be overapproximated as a zonotope \cite{guibas2003zonotopes}. % \Zac{move to obstacle constraint formulation?}
    In addition, if the environment contains a non-convex, bounded obstacle, it can be outerapproximated by computing the obstacle's convex hull. 
    Previous work has demonstrated that dynamic obstacles may also be considered within the \MethodName{} framework \cite{vaskov2019towards}, but we omit this case in this paper.
    %Given that an obstacle can be represented by a zonotope, we can say the manipulator is in collision with an obstacle if if $\FO_j(\q) \cap O_i \neq \emptyset$ for any $j \in \Nq$ or $i \in \{1,\ldots,\nObs\}$. \Zac{move this sentence to algorithm theory? not necessary here} 

\subsection{Contact Modeling}

    \begin{figure}
        \centering
        \includegraphics[width=0.9\columnwidth]{Figures/RSS_2022_Figure_2_v2.pdf}
        \caption{Free Body Diagram of a manipulated object with the applied forces and moments. $\COMproj{}$ is the projection of the COM onto the contact plane.}
        \label{fig:contactdiagram}
    \end{figure}
    
    The full system considered in this paper is comprised of a robotic manipulator, as described above, which grasps a flat surfaced tray with a loosely placed object resting on the flat surface of the tray.
    % This system is illustrated in Fig. \ref{fig:contactdiagram}. 
    We make the following assumptions about the full system:
    \begin{assum}
        \label{assum:contact}
        The robotic manipulator is able to maintain force closure on the tray for all time, and therefore the tray can be treated as an additional link, where the corresponding joint is located between the grasp points of the manipulator. %\Zac{probably need to illustrate this, cite the paper that Rodriguez paper does which does this?}
        When the object is not moving relative to its supporting surface, it can also be treated as an additional link, where the corresponding joint is located at point $\COMproj{}$, as shown in Figure \ref{fig:contactdiagram}. % this joint location is important for the ZMP constraint
        The homogeneous transformation between the additional joint reference frames and the $\nq^{th}$ joint reference frame are known.
        The tray and object volumes are overapproximated as unions of convex polytopes. 
        % need to make sure that the part of the environment section gets incorporated where it is cited that convex objects can always be overapproximated by unions of convex polytopes. 
        Furthermore, the true inertial parameters of the tray, $\Delta_{q+1}$, and the object, $\Delta_{q+2}$ lie in the known intervals $[\Delta_{q+1}]$ and $[\Delta_{q+2}]$, respectively. % with some nominal interval known as well.
    \end{assum}
    Based on this assumption, the tray and object can be treated as an extension of the kinematic chain of the manipulator, where the corresponding joints would be denoted by $j=\nq+1$ and $j=\nq+2$.
    In addition, the inertial parameters of the manipulator are augmented to form the inertial parameters of the whole system. % add equation here showing this?
    For the $\nq+2$ joint and reference frame, since they are located at the point of contact between the tray and object, we instead refer to them as the contact joint and frame given by $\{\hat{x}_{\contact},\hat{y}_{\contact},\hat{z}_{\contact}\}$, where it is denoted by $j=\contact$ for convenience. 
    We define the reference frames of the corresponding joints such that they have x-axes which align with that of the $\nq^{th}$ joint of the manipulator and the contact frame has the z-axis aligned with the normal $\eenorm$ of the tray surface.
    
    Since the tray is rigidly grasped, the corresponding joint can be treated as a fixed joint.
    \begin{defn}
        \label{def:fixed_joint_def}
        A fixed joint has a fixed homogeneous transformation $T_{j}^{j-1}$ for all time. %(\qj)
    \end{defn}
    In contrast, the object is loosely placed on the tray meaning that it does not have a fixed homogeneous transformation.
    Therefore, throughout the motion of the system, the motion of the loosely placed object relative to the supporting surface is determined by the wrenches applied to it.
    We assume that there is no external wrench applied.
    Therefore the object is manipulated only by the contact wrench $ \cwrench(t) = [\cxforce,\cyforce{},\czforce{},\cxmoment{},\cymoment{},\czmoment{}]^T $ and the gravito-inertial wrench $\gravinertwrench{\contact} = [\FGravInert{}, \MGravInert{}]^T$.
    The contact wrench is applied by the manipulator through the supporting surface, and is therefore located at point $\COMproj{}$.
    The gravito-inertial wrench acts on the center of mass of the object being manipulated.
    Recall that the waiter motion problem requires that a loosely placed object does not move relative to its supporting surface while the full system is following a desired trajectory.
    By constraining the contact wrench, the motion of the loosely placed object can be constrained in all six degrees of freedom, resulting in no relative motion.
    
    % \Zac{additional joints are either fixed joints or contact joints (friction joint like Rodriguez paper?). fixed joints have a fixed homogeneous transformation and contact joints do not. thus for contact joints, we write constraints to prevent relative motion.}
    % make clearer that this is done solely for RNEA calculation? maybe start with we want to calculate using RNEA (not external) so we make the following assumptions or something?
    
    % need some transition
    
    A Newton-Euler approach is applied in order to formulate the kinematics and dynamics of the manipulator system \cite{Craig2005}. 
    Given the angular velocity of link $j-1$, the angular velocity of link $j$ can be expressed as
    \begin{equation}
        \label{eq:joint_ang_vel}
        \omega\jss = R\jssm \omega\jssmm + \qdjnot \zj
    \end{equation}
    Next, given the angular acceleration of link $j-1$, the angular acceleration of link $j$ can be expressed as
    \begin{equation}
        \label{eq:joint_ang_accel}
        \begin{split}
        \dot{\omega}\jss = R\jssm \dot{\omega}\jssmm + (R\jssm \omega\jss) \times (\qdjnot \zj) + \qddjnot \zj
        \end{split}
    \end{equation}
    The linear acceleration of each link frame is then
    \begin{equation}
        \label{eq:link_lin_accel}
        \dot{v}\jss = (R\jssm \dot{v}\jssmm) + (\dot{\omega}\jss \times p\jssmu) + (\omega\jss \times (\omega\jss \times p\jssmu))
    \end{equation}
    and the linear acceleration of the COM of link $j$ is
    \begin{equation}
        \label{eq:link_COM_lin_accel}
        \dot{v}\jssCOM = \dot{v}\jss + (\dot{\omega}\jss \times p\jssCOM) + (\omega\jss \times (\omega\jssa \times p\jssCOM))
    \end{equation}
    
    In order to calculate the contact wrench, we first calculate the inertial force and torque acting at the center of mass of each link:
    \begin{equation}
        % \label{eq:COM_F_N}
        \label{eq:COM_force}
        \genCOMforce = m_{j} \COMaccel
    \end{equation}
    \begin{equation}
        \label{eq:COM_torque}
        \genCOMtorque = I_{j} \angaccel(t) + \angvel(t) \times (I \angvel(t))
    \end{equation}
    where $\mathbf{I}_j$ is the spatial inertia matrix of the $j^{th}$ link.
    Next, using a force-balance and moment-balance on the $j^{th}$ link, the reaction wrench $\genwrench{j} = [\genjointforce, \genjointtorque]^{T}$ between link $j-1$ and the $j^{th}$ link can be found .
    \begin{equation}
        % \label{eq:gen_wrench}
        % \begin{split}
        \label{eq:joint_force}
        \genjointforce = R\jssp(t) f^{j+1}_{j+1}(t) + F\jss(t)
    \end{equation}
    \begin{equation}
        \label{eq:joint_torque}
        \begin{split}
        \genjointtorque & = (R\jssp(t) n^{j+1}_{j+1}(t)) + (c\jss \times F\jss(t)) \\
        & + (p\jssp \times (R\jssp(t) f^{j+1}_{j+1}(t))) + N\jss(t) \\
        \end{split}
    \end{equation}
    
    Due to the location of the contact joint, Eqs. \eqref{eq:joint_force}-\eqref{eq:joint_torque} calculates the contact wrench $\cwrench(t)$ applied by the manipulator and tray to the object, and it is expressed in the contact frame.
    % took out the following as it pertains to how I wrote this section based on Featherstone's book and not Craig's. It might be good to note still that there is no external wrench and so the f,n when j+N doesn't have the j+1 terms. 
    % Further, the expression to calculate the contact wrench can be simplified since the object is a terminal link of the kinematic chain and we assume that there are no external forces acting on the object.
    % \begin{equation}
    %     \label{eq:contact_wrench}
    %     \cwrench(t) = \mathbf{I}_{\contact} \qdd_{\contact}(t) + \qd_{\contact}(t) \times \mathbf{I}_{\contact} \qd_{\contact}(t)
    % \end{equation}
    % \Zac{NOTE: these are not supposed to be q's, they should be v's and a's or omega's like in the PZRNEA algorithm and Featherstone book.} 
    %
    The following subsections detail the formulation of the constraints using the contact wrench to restrict relative motion of the object.
    
    % Extra
    %This enables calculation of $\cwrench$ through Alg. \ref{alg:RNEA}, which is a standard Recursive Newton Euler Algorithm (RNEA).
    % \ref{fig:contactdiagram} shows the contact wrench and the contact frame. 
    %Note that the first two assumptions enable the kinematic chain of the manipulator to be extended to include the tray and object, which is important for the implementation of the constraints, which is discussed in Sec. \ref{sec:plan_alg_imp}.
    %relevant forces and moments acting on the object as well as the relevant dimensions. % contact wrench, gravito-inertia wrench, diameter, height, COM point, ZMP point?, contact area on the surface
    

    % \Zac{add a diagram showing the location of the additional joints?}
    % \Zac{note that multiple objects on the supporting surface would just involve branching the kinematic chain, where each loosely placed object would be connected to the tray with a fixed joint? stacking objects would just be a continuation of the kinematic chain, where the joint is on the contact surface and additional (different) constraints can be written.}
    % \Zac{future work idea: purposeful "constraint violation", as in allowing the object to slide only, or tip only could probably be achieved by removing the corresponding constraint and adding a degree of freedom for RNEA to calculate the motion. could add constraint restrict that state so that object doesn't fall off of the tray? purpose is non-prehensile manipulation that allows reorientation of object on tray}
    % Describe how RNEA enables calculation of the relevant contact forces since tray and cup are part of the kinematic chain. Just need a URDF. Do this in a later section?
    
    % RNEA algorithm? or just reference something that has it already?
    
    
    % Describe the constraints that need to be enforced to achieve the task
    \subsubsection{Separation Constraint}
    
        The first degree of freedom to constrain is translation in the direction of $\hat{z}_{\contact}$, shown in Fig. \ref{fig:contactdiagram}.
        Translation into the tray is prevented by a reaction force from the rigid body of the tray, which is assumed to be unlimited.
        So a separation constraint is written to prevent translation away from the tray surface.
        A violation of this constraint means that the two bodies lose contact, resulting in no normal force between the two bodies. 
        %Therefore the normal force is equal to the component of the contact force along the z-axis.
        Thus the separation constraint can be written as
        \begin{equation}
            \label{eq:sep_constraint}
            - \czforce \leq 0
        \end{equation}
        where $\czforce$ is the vertical force component of the contact wrench and is expressed in the contact frame, thus it corresponds to the normal force.
        Satisfaction of this constraint means that a normal force exists, and therefore the object is not translating vertically relative to the tray.

    \subsubsection{Linear Slipping Constraint}
    
        The next two degrees of freedom, translation in the direction of $\hat{x}_{\contact}$ and $\hat{y}_{\contact}$, can be constrained at the same time using a standard static friction law.
        %The static friction is overcome when the magnitude of the tangential component of the contact wrench is larger than the magnitude of the normal component multiplied by the coefficient of static friction.
        This constraint can be written as:
        \begin{equation}
            \label{eq:slip_constraint}
            \lvert \cforcetan \rvert \leq \CoefFric \lvert \czforce \rvert
        \end{equation}
        where $\CoefFric$ is the coefficient of static friction and $\cforcetan$ is the force component of the contact wrench tangential to the supporting surface and expressed in the contact frame.
        Satisfaction of this constraint prevents the static friction between object and the tray from being overcome.
        Note that we are not considering rotational friction, but implementing a constraint to ensure no rotational slip can be done by applying polynomial zonotope arithmetic to the formulations in \cite{} or \cite{}.
        
    % \subsection{Rotational Slipping Constraint}
    
    %     \Zac{need to be wary about uniform vs nonuniform pressure distribution on contact area. could relate to the ZMP? look at center of pressure which is related but may not be the same}
    %     A rotational friction law is used to constrain rotation about $\hat{z}_{\contact}$.
    %     To derive the constraint, we first make the following assumptions:
    %     \begin{assum}
    %         \label{assum:rotational_friction}
    %         The object has a circular contact patch with radius $\objrad$ with a uniform normal pressure distribution and a uniform static coefficient of friction.
    %     \end{assum}
    %     Dividing the contact area into differential elements with area $dA$, then the maximum differential frictional moment is given by
    %     \begin{equation}
    %         \label{eq:diff_friction_moment}
    %         d\czmomentmax = \CoefFric p \objrad dA
    %     \end{equation}
    %     where $p$ is the normal pressure acting on the differential element. 
    %     Through integrating Eq. \eqref{eq:diff_friction_moment} over the contact area, the maximum frictional moment can be obtained:
    %     \begin{equation}
    %         \label{eq:integral_friction_moment}
    %         \begin{split}
    %         \czmomentmax & = \int_A d\czmomentmax \\
    %         & = \int_A \CoefFric p \objrad dA \\
    %         & = \CoefFric \frac{\czforce}{\pi \objrad^2} \int_{0}^{r_{o}} 2 \pi \objrad^2 dr \\
    %         & = \frac{2}{3} \CoefFric \objrad \czforce{}
    %         \end{split}
    %     \end{equation}
        
    %     The rotational friction constraint can be written as
    %     \begin{equation}
    %         \label{eq:rot_slip_constraint}
    %         \lvert \czmoment{} \rvert \leq \frac{2}{3} \CoefFric \objrad \lvert \czforce \rvert
    %     \end{equation}
    %     % depends on the contact area geometry.
        
    %     \Zac{need to add another subplot to the experimental figure for this}
    
    \subsubsection{Tipping Constraint}
    
        Finally, we wish to constrain the last two degrees of freedom, which are rotation about $\hat{x}_{\contact}$ and $\hat{y}_{\contact}$.
        Motion about these axes corresponds to tipping of the object. 
        We use a Zero Moment Point (ZMP) constraint, which requires that the ZMP point exists inside the convex hull of the contact area of the loosely placed object \cite{VUKOBRATOVIC2012}.
        This ensures that the normal component of the contact force can apply a sufficient counteracting moment about point $\COMproj{}$ in order to balance the gravito-inertial wrench of the object exerted about point $\COMproj{}$.
        % mention that the wrench is transmitted only through the friction and normal force, which correspond to f_x,f_y,f_z and n_z? so only these components are used to write constraints. 
        First, the ZMP point for the object can be calculated using the following equation:
        \begin{equation}
            \label{eq:ZMPpoint}
            \ZMPvec{} = \frac{\eenorm{} \times \MGravInertProj{}}{\eenorm{} \cdot \FGravInert{}}
        \end{equation}
        where $\COMproj{}$ is the point representing the normal projection of the COM of the object onto the supporting surface, $\ZMPpoint{}$ is the location of the ZMP point, $\MGravInertProj{}$ is the gravito-inertial moment acting on the object about $\COMproj{}$, and $\FGravInert{}$ is the gravito-inertial force acting on $\COMproj{}$. 
        % also assuming no other external wrench acting on object so only gravito-inertial wrench needs to be balanced by the supporting surface wrench
        % Need to make sure that the gravito-inertial force and moment are labelled properly. Maybe cite another paper as well? 
        
        Next, there are only two wrenches acting on the object, the wrench applied by the manipulator and the gravito-inertial wrench of the object. 
        For there to be no relative motion, these two wrenches must balance each other. 
        Therefore $\MGravInertProj{} = -\cmoment$ and $\FGravInert{} = -\cforce$.
        Substituting these terms in Eq. \eqref{eq:ZMPpoint} yields
        \begin{equation}
            \label{eq:ZMPpointContact}
            \ZMPvec{} = \frac{\eenorm{} \times \cmoment}{\eenorm{} \cdot \cforce}
        \end{equation}
        % since the negative signs can be factored out and canceled. 
        % \Zac{should probably change the name of $\ZMPvec{}$}
        Note that the contact frame is defined to be located at $\COMproj{}$, so Eq. \eqref{eq:ZMPpointContact} gives the position of the ZMP point with respect to the origin of the contact frame.
        
        In this paper, we only consider an object which has a circular contact area, with radius $\objrad{}$.
        The ZMP constraint can then be written as:
        \begin{equation}
            \label{eq:tip_constraint}
            \lVert \ZMPvec{} \rVert \leq \objrad
        \end{equation}
        Satisfaction of this constraint ensures that the ZMP point stays inside the circular contact area, therefore the object will not tilt relative to the tray.
        
        % \Zac{should redo the ZMP constraint to be like the obstacle avoidance constraint. represent the contact area using a halfspace representation and then check if the ZMP point is inside the halfspace area. would be something like A*slice(ZMPt;k)/slice(ZMPb;k)-b<0 I think.}
        
\subsection{Continuous-Time Trajectory Optimization}   

The main aim of this paper is to write a trajectory optimization program with the appropriate constraints whose solution is a reference trajectory that satisfies the two key properties discussed in Sec. \ref{sec:intro}.
% Continuous-time optimization problem
The constraints discussed above restrict all six degrees of freedom such that the object will remain static relative to the supporting surface.
\begin{thm}
    \label{thm:constraint_satisfaction}
    If Eq. \eqref{eq:sep_constraint}-\eqref{eq:tip_constraint} are satisfied for a trajectory, then the loosely placed object will not move relative to its supporting surface.
\end{thm}
Using these constraints, a continuous-time trajectory optimization problem can be written which satisfies the waiter motion problem:

\begin{align}
    \label{eq:optcost}
    &\underset{u}{\min} &&\texttt{cost}(u, q_{goal}) \\
    \label{eq:optpos}
    &s.t. && \qj \in [\qlim^-, \qlim^+]  &\forall t, j \\
    \label{eq:optvel}
    &&& \qdj \in [\dqlim^-, \dqlim^+]  &\forall t, j \\
    \label{eq:opttorque}
    &&& \ujt \in [\ulim^-, \ulim^+]  &\forall t, j \\
    % \label{eq:optposcon}
    % &&& \pjt \in [p_j^-, p_j^+]  &\forall t \in T, j \in \Nq \\
    % \label{eq:optorncon1}
    % &&& \hat{z}_{d,j}^{T} \hat{z}_{j}(t) \geq z_{d,j}^-  &\forall t \in T, j \in \Nq \\
    % \label{eq:optorncon2}
    % &&& \hat{x}_{d,j}^{T} \hat{x}_{j}(t) \geq x_{d, j}^-  &\forall t \in T, j \in \Nq \\
    \label{eq:optcolcon}
    &&& \FO_j(q(t)) \bigcap \obsset = \emptyset  &\forall t, j \\
    \label{eq:optsepcon}
    &&& -\czforce \le 0 &\forall t \\
    \label{eq:optslipcon}
    &&& |\cforcetan| - \mu_{s}|\czforce| \le 0 &\forall t \\
    % \label{eq:optrotslipcon}
    % &&& \lvert \czmoment{} \rvert - \frac{2}{3} \CoefFric \objrad \lvert \czforce \rvert \leq 0 \quad & \forall t \\
    \label{eq:opttipcon}
    &&& ||\ZMPvec{}|| - \objrad \le 0 &\forall t
\end{align}
where $t \in T$, $j \in \Nq$, and $\qgoal \in Q$ denotes a goal configuration for the system.
% Say that we will go over how we discretize later and the methods that we use to still make guarantees about continuous time safety. 
In Sec. \ref{sec:plan_alg_theory}, we will discuss how this problem is discretized and the methods we use to make continuous-time safety guarantees despite discretization.




%%% Previously written

%\Zac{\st{I think that the ZMP constraint also covers the separation constraint, so that constraint may not be necessary. Basically in the ZMP point equation, the denominator is the normal component of the contact force. As this approaches zero, i.e. approaches the constraint boundary of the separation constraint, the ZMP point equation will have the denominator approach zero as well, resulting in a larger and larger value, therefore approaching its constraint boundary as well. Given that the distance used to write the ZMP constraint cannot be infinite, the ZMP constraint will violate before a separation constraint violation, even if there is a large numerator.} this is not true, counterexample is accelerate straight down (moment is zero, therefore the tipping constraint cannot be violated since $r>0$, unless contact is truly a point but that isn't really physically possible)}

        %Then, for the $\nq_{+2}^th$ joint, Eq. \eqref{eq:contact_wrench} gives the wrench applied by the robot arm onto the object. 
        % This expression can be simplified since there is no external force applied or a force applied by children links since the $\nq_{+2}^th$ is a terminal link of the kinematic chain.
        % The simplified expression shows that the contact wrench is equal and opposite to the gravito-inertial wrench of the object.
        % % can check this in the armtd code

% The waiter-motion problem consist of manipulating a loosely placed object resting on a supporting surface. For this paper, we assume that the object is resting on a tray that is firmly grasped by the robotic manipulator (i.e. force closure on the tray can be maintained at all times). \Zac{state this as an assumption?} We model the contact interactions between the supporting surface and object through a wrench applied at the projection of the center of mass onto the contact surface and expressed in the end-effector frame. 

% We treat the tray and object as links of the robot, which enables the whole systems dynamics to be calculated using RNEA. We model the gripper and tray contact as a fixed joint located between the grippers of the fetch robot. We model the tray and object contact as a fixed joint located at the COM projection onto the surface of the tray. 

% We use a RNEA algorithm to calculate the dynamics of the system. The forward pass calculates the accelerations of the joints as well as the inertial forces and moments of the link about the COM. We then write an equivalent wrench about the joint instead. The backward pass calculates the joint torques.

% In order to prevent relative motion of the object and supporting surface, there are several constraints that are needed.

% interval based uncertainty
% This framework using interval-based uncertainty to represent uncertainty in various properties of the robot, such as link mass or inertia, the coefficient of friction or the mass and inertia of an object being manipulated.

    %We note that this assumption could be removed and additional constraints added to enforce that force closure is maintained \Zac{future work}. 
    %Our motivation behind this assumption is that the gripper of the robot forms a closed kinematic chain with the tray when force closure is maintained.
    %We currently have implemented RNEA for open kinematic chains, so this assumption enables us to treat the gripper and tray interaction as a fixed joint, instead of a closed kinematic chain. % future work is closed kinematic loop RNEA?
    % Describe how the tray and loosely placed object can be considered as part of the kinematic chain when static relative to the end-effector of the robot
    
    % \Zac{the following are more implementation details?}
    % Since it is assumed that the tray and object are constrained \Zac{fixed?} relative to the end-effector of the manipulator, they can be treated as part of the kinematic chain of the robot. \Zac{we are assuming it starts in feasible state and that framework ensures it stays in feasible state}
    % \Zac{cite the Rodriguez paper to justify this modeling choice?}
    % However, instead of a revolute joint, a fixed joint is used to model the connection between the manipulator end-effector and the tray as well as the connection between the tray and the loosely placed object. \Zac{this is an implementation detail? explain what does fixed joint mean}

%Since $\MGravInertProj{}$ and $\FGravInert{}$ are written in terms of \COMproj{}, and the fixed joint location is chosen to match \COMproj{}, they can be calculated on the forward pass of RNEA \ref{}. \Zac{Move this to later?}

%%% Outline for reference

% \1 Modeling of Contact Interactions

%     \2 Figure: diagram of cup and tray with the relevant wrench and dimensions indicated along with a reference frame.
    
%     \begin{figure}
%         \centering
%         \includegraphics[width=0.9\columnwidth]{Figures/ARMTD_Force_contactdiagram_v1.jpg}
%         \caption{Caption}
%         \label{fig:my_label}
%     \end{figure}
    
%     \2 Describe the assumptions about the robot properties and dynamics. Things like inertia and the trajectories and forward occupancy.
    
%     \begin{assum}
%   The robot operates in a three dimensional workspace, which we denote $W \subset \R^3$.
%     The robot arm is composed of only revolute joints, where the $j$\ts{th} joint actuates the robot's $j$\ts{th} link.
%     \Ram{this sentence should live outside of the assumption box because it isn't an assumption its an observation.}Note that joints with multiple degrees of freedom may be represented in this framework using links with zero length.
%     The robot's $j$\ts{th} joint has position and velocity limits given by $\qj \in [\qlim^-, \qlim^+]$ and $\qdj \in [\dqlim^-, \dqlim^+]$ for all $t \in T$, respectively.
%     The robot is fully actuated, where the robot's input $u: T \to \R^{\nq}$ \Parker{what are the inputs, torques? If so maybe the symbol for torques?} has limits that are given by $u(t) \in [\ulim^-, \ulim^+]$ for all $t \in T$.
%     The robot is gripping a tray and can maintain force closure throughout its motion. 
%     On the tray is object and the tray's coefficient of static friction is $\mu_s$. 
%     \end{assum}
    
%     \2 Describe the task and the constraints that we are seeking to enforce. We wish to prevent relative motion of the object and tray, which can occur when the object separates \Parker{Unsure what separates means, maybe define the types of motion the object can take in specific terms?}, slides or tips over. 
    
%     \2 Optimization Problem Solved During Each Planning Iteration 
    
%         \3 Continuous time optimization problem formulation from write up \Parker{Maybe make constraints (5)-(8) words or general functions rather than equations, since you introduce none of the notation for them at this point. Additionally, you should move this up to point C., state this is the problem you are solving to compute inputs u(t) which are used to generate trajectories q(t). Then jump into the properties these trajectories need to satisfy.}
        
%         \begin{align}
%             \label{eq:optcost}
%             &\underset{u}{\min} &&\texttt{cost}(u, q_{goal}) \\
%             \label{eq:optpos}
%             &s.t. && \qj \in [\qlim^-, \qlim^+]  &\forall t \in T, j \in \Nq \\
%             \label{eq:optvel}
%             &&& \qdj \in [\dqlim^-, \dqlim^+]  &\forall t \in T, j \in \Nq \\
%             \label{eq:opttorque}
%             &&& \ujt \in [\ulim^-, \ulim^+]  &\forall t \in T, j \in \Nq \\
%             % \label{eq:optposcon}
%             % &&& \pjt \in [p_j^-, p_j^+]  &\forall t \in T, j \in \Nq \\
%             % \label{eq:optorncon1}
%             % &&& \hat{z}_{d,j}^{T} \hat{z}_{j}(t) \geq z_{d,j}^-  &\forall t \in T, j \in \Nq \\
%             % \label{eq:optorncon2}
%             % &&& \hat{x}_{d,j}^{T} \hat{x}_{j}(t) \geq x_{d, j}^-  &\forall t \in T, j \in \Nq \\
%             \label{eq:optcolcon}
%             &&& \FO_j(q(t)) \bigcap \obsset = \emptyset  &\forall t \in T, j \in \Nq \\
%             \label{eq:optsepcon}
%             &&& -1*\FNorm \le 0 &\forall t \in T, j \in \Nq \\
%             \label{eq:optslipcon}
%             &&& |\FTan| - \mu_{s}|\FNorm| \le 0 &\forall t \in T, j \in \Nq \\
%             \label{eq:opttipcon}
%             &&& ||\ZMP|| - \objrad \le 0 &\forall t \in T, j \in \Nq
%         \end{align}
        
%         \noindent where $r$ is the radius of the contact patch (assumed to be a circular contact patch)
    
%     \2 
    
%     \begin{defn}
%     A trajectory \q is safe \Ram{is safe the right word?} if it satisfies the following conditions for all time
%     \begin{enumerate}
%         \item the normal force $\FNorm$ is always positive in the end-effector frame.
%         \item the magnitude of the tangential force $\FTan$ does not exceed the magnitude of the normal force $\FNorm$ multiplied by the coefficient of static friction $\mu_s$ \Parker{maybe be more explicit here that the forces are in the end-effector frame}. \Zac{I think where I end up introducing $\FTan$ and $\FNorm$ first, I will specify this, will also be clear in figure hopefully}
%         \item the Zero Moment Point (\ZMP) does not leave the convex hull of the contact area.
%     \end{enumerate}
%     \end{defn}
    
%     \2 Describe what modeling choices are made to capture the interaction forces between a loosely placed object and a tray the robot is manipulating. This is where I want to introduce that we are using RNEA to calculate the interaction wrench. We treat the interaction as 6 joints with zero length to achieve 6-DOF motion and use RNEA to calculate the forces and moments applied to those joints.
    
%     \2 \Ram{may want to explain why solving this problem is difficult}
    
%     \2 Difficulties with solving this problem arise due trying to ensuring persistent feasibility, which may not be possible with other methods, or when dealing with uncertainty in parameters like friction or inertia properties of the object being manipulated.
    
    
%     \2 Explain that the goal is to use polynomial zonotope representations to overapproximate the wrench and therefore the constraints, while also dealing with uncertainty in variables like the mass, dimensions, inertia and coefficient of friction.

==> Sections/planning_algorithm_implementation.tex <==
\section{Planning Algorithm Implementation}
\label{sec:plan_alg_imp}

\input{Algorithms/pzfk}
\input{Algorithms/pzfo}
\input{Algorithms/pzrnea}

% Trajectory Creation
\subsection{Trajectory Creation}

	% Describe trajectories being used. Piecewise constant acceleration from t0-tplan with a braking maneuver from tplan-tf.
	This work parameterizes the reference trajectories by using a set of degree 5 Bernstein polynomials which will be described in this section.
	Letting $T=[t_{0},t_{f}]$, WLOG, the reference trajectories take the following form:
	\begin{equation}
        \label{eq:q_bernstein_polynomial}
        \qdeskj = \sum_{l= 0}^{5} \beta_{j, l} b_{j, l}(t),
    \end{equation}
	where $\beta_{j, l} \in \R$ are the Bernstein Coefficients and $b_{j, l}: T \to \R$ are the Bernstein Basis Polynomials of degree 5 given by
    \begin{equation}
        \label{eq:bernstein_basis_polynomial}
        b_{j, l}(t) = {5\choose l}t^{l}(1 - t)^{5 -l},
    \end{equation}
    for each $l \in \{0, \ldots, 5\}$.
	Given an initial condition, the first property of Def. \ref{def:traj_param} constrains the initial position, velocity and acceleration of a trajectory to match the initial condition. 
	The second property of Def. \ref{def:traj_param} constrains the finial velocity and acceleration to be zero. 
	Therefore, five of the six Bernstein coefficients $\beta_{j, \nu}$ can be expressed as
    \begin{align}
        \label{eq:bernstein_coeff}
        \beta_{j, 0} &= \initqj \\
        \beta_{j, 1} &= \frac{1}{5}(\initdqj + 5\beta_{j, 0}) \\
        \beta_{j, 2} &= \frac{1}{20}(\initddqj + 40\beta_{j, 1} - 20\beta_{j, 0})\\
        \beta_{j, 3} &= \frac{1}{20}(0 + 40\beta_{j, 4} - 20\beta_{j, 5})\\
        \beta_{j, 4} &= \frac{1}{5}(0 + 5\beta_{j, 5}).
    \end{align}
    We let the last coefficient $\beta_{j, 5}$ be
    \begin{equation}
        \label{eq:bernstein_k_coeff}
        \beta_{j, 5} = \kjscale \kj + \kjoffset
    \end{equation}
    where $\kjscale$ and $\kjoffset \in \R$ are user-specified constants.
    The choice of trajectory parameter $k_j$ directly determines the coefficient $\beta_{j, 5}$, which is equivalent to the final position $q_j(1; \kj)$ at time $t = 1$.
    Note that with this formulation, $\beta_{j, 3} = \beta_{j, 4} = \beta_{j, 5}$.
    
% 	where the center $g_0$ and the dependent generators $g_j$ enable the trajectory parameter $k$ to map directly to reference joint acceleration trajectories.
% 	Thus the first part is a constant joint acceleration trajectory during the time interval $[t_0,t_{plan}]$.
% 	The second part is a braking maneuver which brings each joint to zero velocity in the time interval $[t_{plan},t_f]$, where $\qdeskjdotplan$ is the velocity at time $t_{plan}$. % also a constant acceleration. note that the acceleration is not required to be zero at the end of the braking maneuver.
% 	Therefore, each reference trajectory has a braking maneuver built into it.
	% These trajectories are parameterized by relating the desired reference acceleration to the decision variable $k$, meaning that a choice of $k$ uniquely determines the reference trajectory.
	
	% Polynomial Zonotope representation of trajectories.
	Next, we describe how to construct the polynomial zonotope representation $\pzqdesji$ by plugging in $\pz{T_i}$ from Eq. \eqref{eq:time_pz} and $\pz{\Kj}$.
	Letting $\bm{\beta}_\mathbf{j, 5} = \kjscale \pz{\Kj} + \kjoffset$, and plugging $\pz{T_i}$ into the basis polynomials \eqref{eq:bernstein_basis_polynomial}, we obtain
    \begin{equation}
        \pzqdesji = \left( \sum_{l = 0}^{4} \beta_{j, l} b_{j, l}(\pz{T_i}) \right) + \bm{\beta}_\mathbf{j, 5}b_{j, 5}(\pz{T_i}).
    \end{equation}
    The desired velocity and acceleration polynomial zonotopes $\pzqddesji$ and $\pzqdddesji$ can be similarly computed.
    These desired trajectory polynomial zonotopes are combined with the tracking error polynomial zonotopes to get $\pzqi$ and $\pzqdi$ as in \eqref{eq:pz_pos} and \eqref{eq:pz_vel}, as well as $\pzqdai$ and $\pzqddai$ as in \eqref{eq:pz_mod_vel} and \eqref{eq:pz_mod_acc}. 
	
	
% Constraint Implementation
\subsection{Position and Velocity Constraints}

    The Polynomial Zonotope Forward Kinematics Algorithm (PZFK), shown in Alg. \ref{alg:compose_fk}, is used to compute the sets of positions of each joint from the set of possible configurations $\pzi{q}$.
    
\subsection{Collision Avoidance Constraints}

    The Polynomial Zonotope Forward Occupancy Algorithm (PZFO), shown in Alg. \ref{alg:compose_fo}, is used to calculate the forward occupancy zonotope $\pzi{\FO_j}$.
    This polynomial zonotope overapproximates all reachable positions of points on link $j$ for the $i^{th}$ time interval and importantly, it depends on the choice of the trajectory parameter $k$.
    In order to ensure the manipulator does not collide with any obstacles $O \in \obsset$, the subset of $\pzi{\FO_j}$ corresponding to a particular $k$, or $\pzki{\FO_j}$, should not intersect any obstacle. 
    The implementation of the constraint in Eq. \eqref{eq:pz_optcolcon} is detailed next.
    
    %First, $\pzi{\FO_j}$ is calculated using Alg. \ref{alg:compose_fo}, where the overapproximated volume of link $j$, $\pz{L_j}$ is generated through the CORA toolbox \cite{}.
    First, we compute a halfspace representation for an obstacle $O$, which is assumed to be a convex polytope (Assumption \ref{assum:obstacles}).
    This halfspace representation is given by $\Aobs \in \R^{\nf \times 3}$ and $\bobs \in \R^{\nf}$, where $\nf$ is the number of faces of $O$.
    A point $p \in \R^3$ lies within an obstacle if and only if $\Aobs p - \bobs \leq 0$, where the inequality is taken element-wise.
    In order to check for a collision with an obstacle, we instead need to determine if all points of the forward occupancy reachable set $\pzki{\FO_j}$ lie outside a halfspace representation of that obstacle.
    So for a given point $p \in \pzki{\FO_j}$, $p \notin O \Longleftrightarrow \max{(\Aobs p - \bobs)} \geq 0$, where the max is taken element-wise. % \Zac{should this be $min() \geq 0$}
    
    Therefore, the constraint that $\pzki{\FO_j}$ does not intersect an obstacle $O$ can be written as $\hobs(i,j,k,O) \leq 0$, where
    \begin{equation}
    	\label{eq:h_obs}
    	\hobs(i, j, k, O) = -\max{(\texttt{inf}(\Aobs\pzFOjki - \bobs))}
    \end{equation}

\subsection{Input Constraints}

    The input constraint is formed through summing the nominal input $\pzi{\tau}$ and the robust input $\pzi{\robvnot}$. 
    We use a Polynomial Zonotope Recursive Newton-Euler Algorithm (PZRNEA), which was introduced in \cite{} \Zac{cite TRO paper} and is shown in Alg. \ref{alg:PZRNEA}, to calculate the nominal input and to compute components of the robust input.
    This method avoids computation of the mass matrix, Coriolis matrix and gravity vector which would be required to use Eq. \eqref{eq:pz_nominal_input} to compute the nominal input.
    
    For calculating the nominal input, Alg. \ref{alg:PZRNEA} takes as input $\pzqi$, $\pzqdi$, $\pzqdai$, $\pzqddai$ and the nominal inertial parameters $\nomparams$. 
    \begin{equation}
    	\pzi{\tau} = \texttt{PZRNEA}(\pzqi,\pzqdi,\pzqdai,\pzqddai,\nomparams)
    \end{equation}
    
    Calculating $\pzi{\robvnot}$, as in Eq. \eqref{eq:pz_robust_coeff}, requires creating polynomial zonotopes representing possible CBF values $\pzi{\robhnot}$ and possible disturbances $\pzi{w}$. 
    First, $\pzi{\tau_{int}}$ is calculated by inputting the interval inertial parameters $\intparams$:
    
    \begin{equation}
    	\pzi{\tau_{int}} = \texttt{PZRNEA}(\pzqi,\pzqdi,\pzqdai,\pzqddai,\intparams)
    \end{equation}
    Then, $\pzi{w}=\pzi{\tau_{int}}-\pzi{\tau}$ per Eq. \eqref{eq:disturbance_equation}.
    
    Next, by altering the inputs to PZRNEA, the same algorithm can be used to compute $\pzi{h}$.
    Let
    \begin{equation}
        \pzi{V} = \frac{1}{2}\pzi{r}^\top \left( M(\pzqi, \intparams) \pzi{r} \right),
    \end{equation}
    where the term 
    \begin{equation}
        M(\pzi{q}, \intparams) \pzi{r} = \texttt{PZRNEA}(\pzqi, \pz{0}, \pz{0}, \pzi{r}, \intparams).
    \end{equation}
    and the base joint acceleration is not initialized as $-g$.
    
    Then, we may obtain $\pzi{h}$ as
    \begin{equation}
        \pzi{h} = -\pzi{V} + \roblevel
    \end{equation}
    as in Eq. \eqref{eq:CBF_lower_bound}. %\Zac{\eqref{eq:CBF_defn} is in proof in ARMOUR paper}
    
    Using $\pzi{w}$ and $\pzi{h}$ and plugging into \eqref{eq:pz_robust_coeff}, we may construct $\pzi{v}$ as in \eqref{eq:pz_robust_input}.
    Finally, combining $\pzi{\tau}$ and $\pzi{v}$ yields $\pzi{u}$ as in \eqref{eq:pz_input}.

\subsection{Contact Constraints}

    The polynomial zonotope overapproximation of the wrench $\pzi{\genwrench{j}}$ is calculated using Alg. \ref{alg:PZRNEA} as well.
    \begin{thm}
        Given $\pzqi$,$\pzqdi$,$\pzqdai$,$\pzqddai$, and $\intparams$ are overapproximative, then Alg. \ref{alg:PZRNEA} results in an overapproximation of the wrench  exerted on the $j^{th}$ link through the kinematic chain, i.e. $\genwrench{j} \in \pzi{\genwrench{j}}, \forall t \in \pz{T_i}$.
    \end{thm}
    Plugging the proper components of the contact wrench $\pzi{\cwrench}$ into the contact constraint equations derived in Sec. \ref{sec:plan_alg_theory} yields constraints that, if satisfied during tracking of a reference trajectory, ensure that the loosely placed object does not move relative to its supporting surface for all time. 

% Analytical Gradients
\subsection{Analytical Gradients}

	We calculate the analytical gradients of the cost function and constraints and provide them to an optimization solver, which reduces the time required to solve the problem.
	For the constraint gradients, we use polynomial differentiation of the polynomial zonotope representations of the constraints.

% Note on Constraint Formulation?




%%% Extra

% On the forward pass, overapproximations of the angular velocity and angular acceleration of each link body, the acceleration of the center of mass (COM) of each link, as well as the wrench exerted at each link COM is calculated using objects described above. % are these wrenches just the gravito-inertial wrench exerted on each COM? would the contact wrench come from the joint torques then?

%\begin{equation}
	%	\label{eq:brake_maneuver}
	%	a_{j}_{brake} = \frac{0-v_{j}(t_{plan})}{t_f-t_{plan}}
	%\end{equation}

%%% Outline for Quick Reference

%\2 Trajectory Creation
%        
%        \3 Describe what trajectories are being used (currently constant acceleration), how they are parameterized and what their polynomial zonotope representations look like. 
%    
%    \2 FK, FO, and PZRNEA Algorithm Implementation
%    
%        \3 PZRNEA Algorithm:
%        
%        \input{Algorithms/pzfk}
%        
%        \input{Algorithms/pzfo}
%        
%        % \begin{align}
%        %   &\pzi{u} = \texttt{PZRNEA}(\pzi{q}, \pzi{\dot{q}}, \pzi{\dot{q}_a}, \pzi{\ddot{q}_a}, \pz{\Delta}) \\
%        %   &+ \pzi{-\robcoeff \frac{\robr}{\norm{\robr}}} \\
%        %   &\jon{\text{how to express robust input?}} \\
%        %   &\jon{\text{fix \texttt{PZRNEA} input}}
%        % \end{align}
%        \input{Algorithms/pzrnea}
%    
%    \2 Constraint Implementation
%    
%        \3 Collision Avoidance
%        
%            \4 Describe the collision constraint. The FO does not intersect any obstacle.
%        
%        \3 Torque Limits
%        
%        \3 End effector wrench constraints
%        
%            \4 Separation constraint: require that the normal force is greater than zero, i.e. the object does not separate from the tray.
%            
%            \4 Friction cone constraint: fundamental friction law is satisfied so no sliding occurs.
%            
%            \4 ZMP constraint: The ZMP point remains in the contact patch so no tipping occurs.
%            
%    \2 \Ram{you need to describe the gradients of the cost function and the constraints}
%    
%    \2 We analytically compute the gradients of the cost function and the constraints. Polynomial differentiation enables computing the gradients of the constraints. 

==> Sections/planning_algorithm_theory.tex <==
\section{Planning Algorithm Theory}
\label{sec:plan_alg_theory}

% Intro to section
% Explain how planning is performed in receding horizon fashion and that each trajectory is certifiably safe. Real time planning is achieved through planning for the next iteration while the current iteration is executing, and we make use of a braking maneuver to ensure safety \Parker{if a new plan cannot be computed in time. Thus, this method is recursively feasible}. 
%Outline the execution of a single planning iteration, including if braking occurs. Go over all the components of the optimization problem solved during the planning iteration. \Zac{move last sentence closer to opt prob?}
%Describe our approach: Generating polynomial zonotope overapproximations of the trajectory and all of the constraints enables fast optimization that also ensures safety.  Highlight the other benefits of this method.

% Recall receding horizon and parameterized trajectories
In this section, we describe the theory of using polynomial zonotope overapproximations to represent the trajectories and constraints used for our trajectory optimization program. 
We use polynomial zonotope overapproximations as they enable this method to guarantee safety and speed through:

\begin{enumerate}
    \item \textbf{Speed:} the size of all polynomial zonotope constraints can be fixed a priori, ensuring constraint evaluation is as fast as required (i.e. within $t_{plan}$).
    \item \textbf{Differentiability:} analytical gradients for use in optimization are generated via polynomial differentiation.
    \item \textbf{Safety in Continuous Time:} given tracking error intervals, each constraint is satisfied over the entire trajectory (including tracking error) for all time $t$ in $[0, \tfin]$ rather than just at discretized time instances.
    \item \textbf{Physical consistency:} dependencies between uncertain inertial parameters, such as the proportional coupling between a link's mass and its inertia matrix, can be modeled explicitly using polynomial zonotopes.
\end{enumerate}

Sec. \ref{sec:plan_alg_imp} details our implementation of this theory in the \MethodName{} framework.

% the following should probably go in implementation?
% we choose trajectories which have constant acceleration for [0, t_plan] and then a braking maneuver from [t_plan, t_stop]
% we execute the first half of the trajectory while solving for a trajectory for the next step. if one is not found before t_plan, then the braking maneuver from the previously certified safe trajectory is executed, bringing the robot to a stop in a feasible state. 


% Trajectory PZ Representation
\subsection{Trajectory}

    % intro to sub section
    In order to properly account for continuous-time and tracking error intervals, the \MethodName{} framework uses polynomial zonotopes to overapproximate the trajectories of the system. 
    Since the desired trajectories $q_d$, $\dot{q}_d$ and $\ddot{q}_d$ are functions of time $t \in T$ and trajectory parameter $k \in K$, we first form polynomial zonotope versions of $T$ and $K$. 
    
    % overapproximation of the compact time interval T
    To create a polynomial zonotope representing the compact time horizon $T$,  a time-step $\timestep$ is chosen such that $\nt \coloneqq \frac{T}{\timestep} \in \N$.
    Then the compact time horizon $T \subset \R$ can be divided into $\nt$ subintervals.
    For example, if $T = [0, 1]$ and $\timestep = 0.01$, then $\nt = 100$ subintervals.
    Now, consider the $i^{th}$ time subinterval corresponding to $t \in \iv{(i-1)\timestep, i\timestep}$.
    We represent this subinterval as a polynomial zonotope $\pz{T_i}$, where 
    \begin{equation}
        \label{eq:time_pz}
        \pz{T_i} = \frac{(i-1) + i}{2}\timestep + \frac{1}{2} \timestep \tvar
    \end{equation}  
    with indeterminate $\tvar \in \iv{-1, 1}$.

    % overapproximation of the trajectory parameter space K
    For the trajectory parameter space $K$, we choose $K = K_1 \times K_2 \times \ldots \times K_{\nq}$, where each $\Kj = \iv{-1, 1}$ is a compact one-dimensional interval.
    Then, we can represent the interval $\Kj$ as a poynomial zonotope $\pz{\Kj} = \kjvar$ where $\kjvar \in \iv{-1, 1}$ is an indeterminate.
    Note that any particular choice of $k_j$ is then trivially related to the corresponding subset $k_j = \texttt{slice}(\pz{\Kj}, \kjvar, k_j)$.
    The slice function therefore allows us to obtain subsets of polynomial zonotopes corresponding to a choice of $k$ by slicing the corresponding $\kvar$ indeterminates. 
    
    
    % trajectory overapproximation construction
    The construction of the overapproximation of the trajectories is detailed next.
    In Def. \ref{def:traj_param}, the reference position, velocity and acceleration trajectories are functions which depend on time $t$ and trajectory parameter $k$.
    These functions can take set-valued inputs.
    By representing $T$ and $K$ as polynomial zonotopes, then plugging those in for the arguments of the reference trajectory functions, the results are overapproximations of the reference trajectories.
    
    \begin{lem}
        An overapproximative polynomial zonotope representation of the desired trajectory $q_{d,j}$ can be formed by using $\pz{T_i}$ and $\pz{\Kj}$ in the arguments of the desired trajectory function.
        The resulting polynomial zonotope $\pzqdesji$ satisfies
        \begin{equation}
            \qdeskj \in \pzqdesji \quad \forall t \in \pz{T_i}, \kj \in \pz{\Kj}
        \end{equation}
        Overapproximative polynomial zonotope representations are similarly constructed for $\pzqddesji$ and $\pzqdddesji$.
    \end{lem}

    The overapproximative trajectories $\pzqdesji$, $\pzqddesji$ and $\pzqdddesji$ depend only on the indeterminates $\tvar$ and $\kjvar$, where $\tvar$ is the indeterminate corresponding to $\pz{T_i}$ and $\kjvar$ is the indeterminate corresponding to $\pz{\Kj}$. % may not need the last half of this sentence since the indeterminates are already explained.
    Since $k_j \in [-1,1]$, it can be plugged in for $\kjvar$, meaning the $\texttt{slice}$ operation can be used to obtain a polynomial zonotope with $\tvar$ as the only remaining indeterminate.
    A notational shorthand is introduced for slicing a polynomial zonotope with respect to a trajectory parameter: $\pzqdesjki = \texttt{slice}(\pzqdesji, \kvar, k)$.
    Therefore, $\qdeskj \in \pzqdesji$ for all $t \in \pz{T_i}$ (and similarly for $\pzqddesji$ and $\pzqdddesji$).
    %, enabling continuous-time guarantees to be made.
    %This is crucial for the optimization program since its solution is a choice of $k \in \pzi{K}$ which can then be used to recover the continuous-time overapproximated trajectory that $k$ parameterized.
    %This enables the discretized optimization problem to make safety guarantees about continuous-time.
    %Further, it can use a choice of $k$ to slice and then evaluate the polynomial zonotope overapproximations of the constraints, whose construction is discussed below.
    
    % detail how the error polynomial zonotopes fit in to ensure overapproximations of any possible trajectory
    However, these desired reference trajectories cannot be tracked perfectly, as mentioned in Sec. \ref{sec:control_des}.
    Instead of perfect tracking, through using theorem \ref{thm:robust_controller}, the controller in \eqref{eq:controller} ensures tracking error $\robrnot$ is uniformly ultimately bounded when applying robust input given in \eqref{eq:robust_input}. \Zac{need to check this reference}
    This results in the position error $\err$ and velocity error $\errdot$ being bounded by $\pbound$ and $\vbound$, respectively, for each time instance $t$. as shown by Cor. \ref{cor:tracking_error}. 
    Using polynomial zonotope overapproximations of the error bounds, we can then form overapproximations any executed trajectory of the system. 
    % use this to overapproximate all possible trajectories
    
    % the following comes directly from the ARMOUR paper
    \begin{thm}
        Define the polynomial zonotopes $\pzpboundj = \pboundj \epvarj$ and $\pzvboundj = \vboundj \evvarj$, with indeterminates $\epvarj \in \iv{-1, 1}$ and $\evvarj \in \iv{-1, 1}$.
        Then, let 
        \begin{align}
            \pzqji &= \pzqdesji \oplus \pzpboundj \label{eq:pz_pos} \\
            \pzqdji &= \pzqddesji \oplus \pzvboundj \label{eq:pz_vel}
        \end{align}
        for each $i \in \Nt$.
        Given the set of trajectory parameters $K$, the polynomial zonotopes $\pzqji$ and $\pzqdji$ overapproximate the set of all joint trajectories that can possibly be executed by the robot, i.e.
        \begin{align}
            q_j(t; k_j) \in \pzqjki \quad \forall t \in \pz{T_i}, \, \kj \in \pz{\Kj} \\
            \dot{q}_j(t; k_j) \in \pzqdjki \quad \forall t \in \pz{T_i}, \, \kj \in \pz{\Kj} \\
        \end{align}
    \end{thm}
    % \begin{proof}
    %     By Lem. \ref{lem:pz_desired_trajectory}, the desired trajectory polynomial zonotopes contain all desired trajectories.
    %     By Cor. \ref{cor:tracking_error}, the position and velocity trajectories differ from the desired trajectories by at most $\pm \pbound$ and $\pm \vbound$, respectively.
    %     Therefore the Minkowski sum of $\pzqdesji \oplus \pz{\pboundj}$ must contain the actual configuration $q_j(t; k)$, and similarly for velocities.
    % \end{proof}
    
    We express  $\pzqdesi = \pzi{q_{d, 1}} \times \pzi{q_{d, 2}} \times \ldots \times \pzi{q_{d, n_q}}$, and $\pzqi = \pzi{q_{1}} \times \pzi{q_{2}} \times \ldots \times \pzi{q_{n_q}}$.
    We may similarly express $\pzqddesi$, $\pzqdi$, $\pzqdddesi$, and $\pzqddi$.
    Furthermore, let $\pz{\pboundvec} = \bm{\epsilon}_\mathbf{p, 1} \times \bm{\epsilon}_\mathbf{p, 2} \times \ldots \times \bm{\epsilon}_\mathbf{p, \nq}$, and similarly let $\pz{\vboundvec} = \bm{\epsilon}_\mathbf{v, 1} \times \bm{\epsilon}_\mathbf{v, 2} \times \ldots \times \bm{\epsilon}_\mathbf{v, \nq}$.

%\Zac{we have these objects from the TRO paper, how do I use them to create the constraints needed for force aware constraints.}
   
\subsection{Reachable Set Construction}

    In the \MethodName{} framework, the kinematic and dynamic behavior of the system, as well as the torques required to achieve that behavior, can be bounded through using the polynomial zonotope overapproximations of the joint trajectories. 
    This section details the construction of the parameterized polynomial zonotopes which overapproximate the forward kinematics, the forward occupancy, the input required to track a reference trajectory, and the applied wrench through the kinematic chain for a single frame/link during a single time interval.
    The implementation of the algorithms which generate these parameterized polynomial zonotopes during the beginning of each planning iteration is discussed in Sec. \ref{sec:plan_alg_imp}.
    % The theory of these algorithms is discussed in this section, with their implementation discussed in Sec. \ref{sec:plan_alg_imp}.
    Also discussed in this section is how polynomial zonotopes overapproximating the constraints in Eq. \eqref{eq:optpos} - \eqref{eq:opttipcon} are constructed.
    %executed at the beginning of each planning iteration
    %The following subsections detail the construction of reachable sets for a single frame/link over a single interval of time. 
    %These trajectory and constraint overapproximations are used in the trajectory optimization problem that is solved during each planning iteration, thus the algorithms are executed at the beginning of each planning iteration.

    \subsubsection{Forward Kinematics Reachable Set}
    
        % need to detail how the rotation and translation are overapproximated since they are used in PZRNEA and also how the forward kinematics are overapproximated since that is used for the forward occupancy. 
        The forward kinematics of the manipulator system, introduced in Sec. \ref{sec:modeling}, are reformulated using polynomial zonotope overapproximations of the joint positions.
        First, using the overapproximated joint positions $\pzqji$, we can compute $\pz{p\jssmu}(\pzqji)$ and $\pz{R\jssmu}(\pzqji)$, which are overapproximations of the the position and orientation of frame $j$ with respect to frame $j-1$ at the $i^{th}$ timestep.
        Note that $\pz{R\jssmu}(\pzqji)$ depends on calculating $\cos{(\pzqji)}$ and $\sin{(\pzqji)}$.
        Since these are analytic functions, they can be rewritten using Taylor expansions as in Eq. \eqref{eq:taylor_pz_inf}.
        Practically, only a finite Taylor expansion can be computed, as in Eq. \eqref{eq:taylor_pz_fin} which is a finite Taylor expansion of dimension $d$ with an overapproximative Lagrange remainder $[R]$. 
        The result is polynomial zonotope overapproximations of the sine and cosine of a polynomial zonotope:
        \begin{thm}
            The sine and cosine of a polynomial zonotope can be overapproximated by computing a Taylor expansion series with an overapproximated Lagrange Remainder.
        \end{thm}
        Therefore, the polynomial zonotope forward kinematics for the $j^{th}$ frame at the $i^{th}$ timestep can be written as:
        \begin{equation}\label{eq:pzfk_j}
            \pz{\FK_j}(\pzqji) = 
            \begin{bmatrix} \pz{R_j}(\pzqji) & \pz{p_j}(\pzqji)\\
            \mathbf{0}  & 1 \\
            \end{bmatrix},
        \end{equation}
        where
        \begin{equation}
            \pz{R_j}(\pzqji) = \prod_{l=1}^{j} \pz{R_{l}^{l-1}}(\pzqji)
        \end{equation}
        and
        \begin{equation}
            \pz{p_j}(\pzqji) = \sum_{l=1}^{j} \pz{R_l}(\pzqji) \pz{p_{l}^{l-1}}.
        \end{equation}
        overapproximate the orientation and position of the $j^{th}$ frame with respect to the world frame, respectively.
        
        \begin{thm}
            \label{thm:FK_overapprox}
            Given that $\texttt{sin}(\pzqji)$ and $\texttt{cos}(\pzqji)$ are overapproximative, then for each $k \in \pz{K}$, $\pzFKjki$ is an overapproximation of the forward kinematics of the $j^{th}$ link for the $i^{th}$ time interval, i.e. $\FK_j(q(t;k)) \in  \pzFKjki, \forall t \in \pz{T_i}$.
        \end{thm}
    
    \subsubsection{Forward Occupancy Reachable Set}
    
        In order to safely prevent collisions while the robot is moving, the forward occupancy of the robot needs to be overapproximated.
        First, the volume of the $j^{th}$ link is overapproximated using a polynomial zonotope denoted by $\pz{L_j}$.
        Then, the forward occupancy of link $j$ at the $i^{th}$ timestep can be overapproximated as follows:
        
        \begin{align}\label{eq:pz_forward_occupancy_j}
             \pz{\FO_j}(\pzqji) = \pz{p_j}(\pzqji) \oplus \pz{R_j}(\pzqji) \odot \pz{L_j}.
        \end{align}
        
        \begin{thm}
            Given that $\pz{p_j}(\pzqji)$, $\pz{R_j}(\pzqji)$ and $\pz{L_j}$ are overapproximations, then for each $k \in \pz{K}$, $\FO_j(q(t;k)) \in  \pzFOjki$, $\forall t \in \pz{T_i}$.
        \end{thm}
        Note that because the loose object and tray it rest upon are treated as part of the kinematic chain of the system, we can then use an overapproximation of their volumes to find their forward occupancy as part of the same process.
    
    \subsubsection{Input Reachable Set}
    		
    	We summarize the formation of the input reachable set in this paper and refer the reader to \cite{} for further detail.
        First, we form overapproximations of the torques required by the controller in Sec. \ref{sec:control_des} for tracking a parameterized trajectory. 
        Through applying polynomial zonotope arithmetic to \eqref{eq:total_feedback_traj}, we form a total feedback trajectory polynomial zonotope $\pzi{\qA}$.
        Then, we define the modified reference velocity and acceleration trajectory polynomial zonotopes that are composed of overapproximated desired trajectories plus a gain matrix times tracking error:
        % Similar to 
        \begin{align}
            \pzqdai &= \pzqdesi \oplus K_r \pz{\pboundvec} \label{eq:pz_mod_vel}, \\
            \pzqddai &= \pzqddesi \oplus K_r \pz{\vboundvec} \label{eq:pz_mod_acc}.
        \end{align}
        
        These elements can be substituted into \eqref{eq:nominal_controller} to form overapproximations of the torques required by the controller:
        \begin{equation}
            \label{eq:pz_nominal_input}
            \begin{split}
            \bm{\tau}(\pzqAi,\Delta_0) = & \ \bM(\pzi{q}, \nomparams) \odot \pzi{\ddot{q}_a} \\
            & \oplus \bC(\pzi{q}, \pzi{\dot{q}},\nomparams) \odot \pzi{\dot{q}_a} \\
            & \oplus \bG(\pzi{q}, \nomparams).
            \end{split}
        \end{equation}
        % where the nominal controller in Eq. \eqref{eq:nominal_controller} uses \textit{auxiliary} velocities and accelerations, which are composed of desired trajectories plus a gain matrix times tracking error:
        % \begin{align}
        %     \pzqdai &= \pzqdesi \oplus K_r \pz{\pboundvec} \label{eq:pz_mod_vel} \\
        %     \pzqddai &= \pzqddesi \oplus K_r \pz{\vboundvec} \label{eq:pz_mod_acc}.
        % \end{align}
        
        Second, we bound the robust control input at each time step.
        \begin{thm}
            \label{thm:robust_input_bound}
            Choose $\alpha: \R \to \R$ such that
            \begin{equation}
                \label{eq:alpha_linear}
                \alpha(h) = \alpha_c h
            \end{equation}
            where $\alpha_c > 0$ is a user-specified constant, and note that $\alpha$ is an extended class $\mathcal{K}_\infty$ as required by Thm. \ref{thm:robust_controller}.
            Also, let
            \begin{equation}
                \begin{split}
                    \bm{\tau}_\regtext{int}&(\pzi{\qA},\intparams) = \bM(\pzi{q}, \intparams) \pzi{\ddot{q}_a} + \\ &+ \bC(\pzi{q}, \pzi{\dot{q}},\intparams) \pzi{\dot{q}_a} + \bG(\pzi{q}, \intparams),
                \end{split}
            \end{equation}
            and using \eqref{eq:disturbance_equation} we obtain
            \begin{equation}
                \label{eq:pz_disturbance}
                \pz{w}(\pzi{\qA},\nomparams,\intparams) = \bm{\tau}_{\regtext{int}}(\pzi{\qA},\intparams) - \bm{\tau}(\pzi{\qA},\nomparams).
            \end{equation}
            Then let
            \begin{equation}
                \begin{split}
                    \rho(\pz{w}(\pzi{\qA},\nomparams,\intparams)) &= \max( \abs{\texttt{inf}(\pz{w}(\pzi{\qA},\nomparams,\intparams))}, \\ &\abs{\texttt{sup}(\pz{w}(\pzi{\qA},\nomparams,\intparams))} ).
                \end{split}
            \end{equation}
            Then for all $\qA(t;k)$ that satisfies the uniform bound \eqref{eq:ultimate_bound}, the absolute value of the $j$-th component of the robust input $\abs{\robv(\qA(t;k), \Delta_0, [\Delta] )_j}$ for $t \in \pz{T_i}$ is bounded by
            \begin{equation}
                \label{eq:pz_robust_input_bound}
                \abs{\robv(\qA(t;k), \Delta_0, [\Delta] )_j} \leq \frac{\alpha_c \epsilon(\sigma_M - \sigma_m) + \norm{\rho(*)} + \rho(*)_j}{2}
            \end{equation}
            where $\rho(*) = \rho(\pz{w}(\pzi{\qA},\Delta_0,[\Delta]))$ and $\rho(*)_j$ is its $j$-th component for brevity.
        \end{thm}
        A proof for Thm. \ref{thm:robust_input_bound} can be found in \cite{} \Zac{cite the TRO paper here}.
        
        Letting 
        \begin{equation}
            \label{eq:pz_robust_coeff}
            \pzi{v_j} = 
            \frac{\alpha_c \epsilon(\sigma_M - \sigma_m) + \norm{\rho(*)} + \rho(*)_j}{2}x_{v_{j}}
        \end{equation}
        with $\rho(*)$ as in Thm. \ref{thm:robust_input_bound} and $x_{v_{j}}$ an indeterminate in $[-1, 1]$, and defining $\pzi{v}$ as
        \begin{equation}
            \label{eq:pz_robust_input}
            \pzi{v} = \pzi{v_1} \times \pzi{v_2} \times \ldots \times \pzi{v_{\nq}}
        \end{equation}
        we finally write the input reachable set for the $i$\ts{th} timestep as
        \begin{equation}
        \label{eq:pz_input}
            \pzi{u} = \bm{\tau}\pzi{} - \pzi{v}.
        \end{equation}
        % describe how this can be calculated using PZRNEA
            
        \begin{thm}
            Given that $\bm{\tau}\pzi{}$ and $\pzi{v}$ are overapproximations, the control input $u(t)$ is overapproximated by $\pzi{u}$.
        \end{thm}
    
    \subsubsection{Wrench Reachable Set}
    
        % \4 Describe the construction of an overapproximation of the end effector wrench. This is done through using PZ-RNEA and the overapproximated joint trajectories. (Likely need a theorem/proof stating that this method does result in an overapproximated wrench?)
        
        % given PZ forms of q, qdot, qddot, T and K, we can form an overapproximative PZ of the wrench applied to the $j^th$ link through the $j^th$ joint.
        % use the featherstone equation (also put in the modeling section?)
        Given the inertial parameter vector $[\Delta]$, a polynomial zonotope overapproximation of the link mass $\pz{m_j}$ and the spatial inertia matrix $\pzi{{I}_j^{j}}$ for the $j^{th}$ link can be computed. %\mathbf
        Then, through plugging in $\pzqdji$ to Eq. \eqref{eq:joint_ang_vel}, an overapproximation of the angular velocity of link $j$ can be expressed as
        \begin{equation}
            \label{eq:joint_ang_vel_pz}
            \pz{\bm{\omega}\jss} = \pz{R\jssm} \odot \pz{\bm{\omega}\jssmm} \oplus \pz{\qdjnot} \zj
        \end{equation}
        
        
        Next, as shown in the algorithm proposed in \cite{Ferrajoli2009}, an auxiliary joint velocity $\qadot$ and an auxiliary angular velocity $\omega_a$ can be included to enable separation of the Coriolis and centrifugal terms in order to compute the passivity-based control law.
        The polynomial zonotope representation of the auxiliary angular velocity of link $j$ is calculated as
        \begin{equation}
            \label{eq:joint_aux_ang_vel_pz}
            \pz{\bm{\omega}\jssa} = \pz{R\jssm} \odot \pz{\bm{\omega}\jssmma} \oplus \pz{\qajdotnot}\zj
        \end{equation}
        Then, the angular acceleration of link $j$ is expressed as
        \begin{equation}
            \label{eq:joint_ang_accel_pz}
            \pz{\dot{\bm{\omega}}\jss} = \pz{R\jssm} \odot \pz{\dot{\bm{\omega}}\jssmm} \oplus ((\pz{R\jssm} \odot \pz{\bm{\omega}\jssa}) \otimes (\pz{\qdjnot} \zj)) \oplus \pz{\qajddotnot} \zj
        \end{equation}
        and the linear acceleration of link $j$ and the COM of link $j$ are
        \begin{equation}
            \label{eq:link_lin_accel_pz}
            \pz{\dot{v}\jss} = (\pz{R\jssm} \odot \pz{\dot{v}\jssmm}) \oplus (\pz{\dot{\bm{\omega}}\jss} \otimes \pz{p\jssmu}) \oplus (\pz{\bm{\omega}\jss} \otimes (\pz{\bm{\omega}\jssa} \otimes \pz{p\jssmu}))
        \end{equation}
        \begin{equation}
            \label{eq:link_COM_lin_accel_pz}
            \pz{\dot{v}\jssCOM} = \pz{\dot{v}\jss} \oplus (\pz{\dot{\bm{\omega}}\jss} \otimes \pz{p\jssCOM}) \oplus (\pz{\bm{\omega}\jss} \otimes (\pz{\bm{\omega}\jssa} \otimes \pz{p\jssCOM}))
        \end{equation}
        
        Next, overapproximations of the force and torque acting at the COM of link $j$ can be formed as
        \begin{equation}
            % \label{eq:COM_F_N}
            \label{eq:COM_force_pz}
            \pz{\genCOMforcePZ} = \pz{m_{j}} \odot \pz{\dot{v}\jssCOM}
        \end{equation}
        \begin{equation}
            \label{eq:COM_torque_pz}
            \genCOMtorquePZ = \pz{I_{j}^{j}} \odot \pz{\dot{\bm{\omega}}\jss} \oplus \pz{\bm{\omega}\jssa} \otimes (\pz{I_{j}^{j}} \odot \pz{\bm{\omega}\jss})
        \end{equation}
        
        Then, by plugging $\pzi{{I}_j}$ into Eq. \eqref{eq:COM_torque_pz}, the polynomial zonotope overapproximation of the reaction force and torque with the $j^{th}-1$ link can be written as: 
        
        \begin{equation}
            % \label{eq:gen_wrench_pz}
            \label{eq:joint_force_pz}
            \pz{f\jss} = \pz{R\jssp} \odot \pz{f^{j+1}_{j+1}} \oplus \pz{F\jss} \\
        \end{equation}
        \begin{equation}
            \label{eq:joint_torque_pz}
            \begin{split}
            \pz{n\jss} & = (\pz{R\jssp} \odot \pz{n^{j+1}_{j+1}}) \oplus (\pz{c\jss} \otimes \pz{F\jss}) \\
            & \oplus (\pz{p\jssp} \otimes (\pz{R\jssp} \odot \pz{f^{j+1}_{j+1}})) \oplus \pz{N\jss} \\
            \end{split}
        \end{equation}
        
        % \begin{equation}
        %     \label{eq:gen_wrench_pz}
        %     \begin{split}
        %     \pzi{\genwrench{j}} = \pzi{{I}_j} \odot \pzqddji \oplus \pzqdji \otimes \pzi{{I}_j} \odot \pzqdji \\
        %     \ominus \pzi{\genwrenchext{j}} \oplus \sum_{i \in \mu(j)} \pzi{\genwrenchext{i}}
        %     \end{split}
        % \end{equation}
        
        % In particular, the polynomial zonotope contact wrench is constructed through plugging into Eq. \eqref{eq:contact_wrench}
        % \begin{equation}
        %     \label{eq:contact_wrench_PZ}
        %     \begin{split}
        %         \pzi{\cwrench} = \pzi{{I}_{\contact}} \odot \pzqddci \oplus \pzqdci \otimes %\\
        %         \pzi{{I}_{\contact}} \odot \pzqdci
        %     \end{split}
        % \end{equation}
        
        % \Zac{NOTE: these are not supposed to be q's, they should be v's and a's or omega's like in the PZRNEA algorithm and Featherstone book.}
        
        \begin{thm}
            Given that $\pzi{\mathbf{I}_{j}^{j}}$, $\pzqji$, $\pzqdji$, $\pzqdaji$ and $\pzqddji$ are overapproximations, the reaction wrench $\genwrench{j}(t;k)$ between link $j$ and link $j-1$ is overapproximated by $\pzki{\genwrenchPZ{j}}$.
            \begin{equation}
                \genwrench{j}(t;k) \in \pzki{\genwrenchPZ{j}}, \quad \forall t \in \pz{T_i}, k_j \in \pz{K}
            \end{equation}
        \end{thm}
        
        
    % \begin{equation}
    %     \label{eq:COM_F_N}
    %     \begin{split}
    %     \genCOMforce & = m_{j} \COMaccel \\
    %     \genCOMtorque & = I_{j} \angaccel + \angvel \times (I \angvel)
    %     \end{split}
    % \end{equation}
    
    % \begin{equation}
    %     \label{eq:gen_wrench}
    %     \begin{split}
    %     \genjointforce & = R\jssp f^{j+1}_{j+1}(t) + F\jss(t) \\
    %     \genjointtorque & = (R\jssp n^{j+1}_{j+1}) + (c\jss \times F\jss) \\
    %     & + (p\jssp \times (R\jssp f^{j+1}_{j+1})) + N\jss \\
    %     \end{split}
    % \end{equation}
        
        

\subsection{Constraint Generation}
    
    This subsection details how the constraints are formulated using the polynomial zonotope reachable sets detailed above.
    
    \subsubsection{Position and Orientation Constraints}
    % joint position and velocity constraints?
    % am I using these beyond just the normal state limits on position and velocity. I think the TRO paper uses these to constrain the end-effector position and orientation for grasping stuff but the waiter motion stuff hasn't used anything like that.
    
    The joint position and velocity trajectories are overapproximated by $\pzqji$ and $\pzqdji$, respectively, with tracking error incorporated for a time interval $\pz{T_i}$.
    Given bounds $[\qlim^{-},\qlim^{+}]$ and $[\dqlim^{-},\dqlim^{+}]$, then $k$ should be chosen such that $\pzqjki$ and $\pzqdjki$ lie completely within the bounds $\forall i \in \{1,\hdots,\nt\}$. 
    
    %\Zac{might be informative to plot the angle of the tray to see if it ever goes beyond the angle at which static friction is overcome when the robot is static. ideally it would be so the robot could move faster but I am not sure that the robot is doing so. might be a high level planner thing though since the HLP gives a specific set of joint angles as a waypoint instead of a waypoint in taskspace.}
    
    \subsubsection{Collision Avoidance Constraints}
    
    To avoid collisions during a time interval $\pz{T_i}$, the volume that the manipulator system occupies in taskspace cannot intersect with obstacles.
    The forward occupancy of the robot is overapproximated for all time by $\pzi{\FO}$.
    By choosing $k$ such that $\pzki{\FO_j} \bigcap \obsset = \emptyset, \forall i \in \{1,\hdots,\nt\}$, it is guaranteed that the robot does not collide with obstacles. 
    
    \subsubsection{Input Constraints}
    
        In order to avoid saturating the available motor torques of the manipulator, constraints on the input polynomial zonotope $\pzi{u}$ are formed as was done in \cite{} \Zac{cite TRO paper}.
        Note that at the time of planning, the tracking error and disturbances due to variations in inertial parameters is not known.
        The constraint handles this conservatively by assuming the worst-case disturbances and tracking error, which can be contained by a lower bound $\ulim^-$ and an upper bound $\ulim^+$.       
        By choosing $k$ such that $\pzuji \in [\ulim^-,\ulim^+], \forall i \in \{1,\hdots,\nt\}$, it is guaranteed that the robot does not saturate its motor torque limits when tracking a desired trajectory.
    
    \subsubsection{Contact Constraints}
    
		The contact constraints are formed using $\pzi{\cwrenchPZ}$, which is the overapproximation of the contact wrench between the tray and loose object.
		 
        For the separation constraint, the normal component of the contact force is overapproximated by $\pzi{f_{c,z}}$ for the time interval $\pz{T_i}$. 
        Through choosing $k$ such that
        \begin{equation}
            \label{eq:pz_sepcon}
            % - \pzi{\czforcenotPZ} \leq 0, &\quad  \forall i \in \{1,\hdots,\nt\}
            - \pzi{f_{c,z}} \leq 0, \quad  \forall i \in \{1,\hdots,\nt\}
        \end{equation}
        it is guaranteed that there is a normal force between the loose object and tray.
        % this requires choosing a $k$ such that 
        
        %\Zac{should rewrite the tipping constraint to use the same formulation as the collision constraint and then demonstrate using a Michigan M on a tray that has two rectangular contact points and then maybe like a toy space ship which contacts at single points which are vertices of a triangle or something. Can also have it handle line and single point contacts and maybe try to balance something while moving? uncertainty would make that probably near impossible to move though...}
            
        %Friction constraint is rewritten to involve only summation and multiplication operations.
        The friction constraint is formed using the both the normal and tangential components of the contact force. 
        Normally, the tangential component would be calculated by taking the norm of the planar contact force components.
        However, a square root operation for polynomial zonotopes does not currently exist. 
        %\Zac{is this true, or is it just easier for us not to use it?} \pat{there isn't one, i'm not sure that it's impossible to write one but idk how to do it}
        Therefore, the polynomial zonotope version of the slipping constraint is constructed through reformulating Eq. \eqref{eq:slip_constraint} as follows:
        \begin{equation}
        		\label{eq:static_friction_law}
        		|\cforcetan| \leq \CoefFric |\czforce|
        \end{equation}
        is equivalent to
        \begin{equation}
    		\label{eq:static_friction_law_squared}
    		\cforcetan^{2} \leq  \CoefFric^{2} \czforce^{2}
    		\end{equation}
        \begin{equation}
    		(\sqrt{\cxforce^{2}+\cyforce^{2}})^{2} \leq \CoefFric^{2} \czforce^{2}
		\end{equation}
		with the final reformulated slipping constraint written as:
		\begin{equation}
    		\cxforce^{2}+\cyforce^{2} - \CoefFric^{2} \czforce^{2} \leq 0
        \end{equation}
        % need to have a PZ version
        
        Now, the contact force components are overapproximated by their respective components in $\pzi{\cwrenchPZ}$, and the slipping constraint can be rewritten as:
        \begin{equation}
            \label{eq:pz_slipcon}
            \begin{split}
    		\pzi{f_{c,x}} \odot \pzi{f_{c,x}} \oplus \pzi{f_{c,y}} \odot \pzi{f_{c,y}} \\
    		\ominus \CoefFric^{2} \odot \pzi{f_{c,z}} \odot \pzi{f_{c,z}} \leq 0
    		\end{split}
        \end{equation}
        Note that the coefficient of static friction could be uncertain, meaning that the actual coefficient exists in an interval $\CoefFric \in [\mu_{s, lower},\mu_{s, upper}]$.
        However, it is only necessary to consider the smallest possible value to ensure no slip occurs, so in Eq. \eqref{eq:pz_slipcon}, $\CoefFric=\texttt{inf}([\mu_{s, lower},\mu_{s, upper}])$. \Zac{change to just be equal to the lower value?}
        % \Zac{Note how the coefficient of static friction can be switched from a single value to an interval to account for uncertainty in the coefficient of friction.}
        By choosing $k$ such that Eq. \eqref{eq:pz_slipcon} is satisfied $\forall i \in \{1,\hdots,\nt\}$, it is guaranteed that the object does not translate tangentially to the support surface.
        
        % Rotational friction constraint
        % The rotational friction constraint in Eq. \eqref{eq:rot_slip_constraint} requires that the exerted moment about $\hat{z}_{\contact}$ is less than the maximum frictional moment that the contact area can provide. This constraint can be reformulated to work with polynomial zonotope objects:
        % \begin{equation}
        %     \lvert \czmoment{} \rvert \leq \frac{2}{3} \CoefFric \objrad \lvert \czforce \rvert
        % \end{equation}
        % is equivalent to
        % \begin{equation}
        %     \label{eq:reform_rot_slip_constraint}
        %     \czmoment{}^2 \leq (\frac{2}{3} \CoefFric \objrad)^2 (\czforce)^2
        % \end{equation}
        % Therefore a rotational friction constraint overapproximation can be written as:
        % \begin{equation}
        %     \label{eq:pz_rot_slip_constraint}
        %     \pzi{\czmomentnot{}} \odot \pzi{\czmomentnot{}} \ominus (\frac{2}{3} \CoefFric \objrad)^2 \pzi{\czforcenot} \odot \pzi{\czforcenot} \leq 0
        % \end{equation}
        
        %Tipping constraint is rewritten to involve only summation and multiplication operations.
        The tipping constraint must also be reformulated to work with polynomial zonotope objects.
        The calculation of the ZMP point, as shown in Eq. \eqref{eq:ZMPpointContact}, requires a division operation, which does not currently exist for polynomial zonotopes.
        Therefore, we rewrite the constraint as follows:
        \begin{equation}
        		\lVert \ZMPvec{} \rVert \leq \objrad
        \end{equation}
        \begin{equation}
            \label{eq:tipcon}
            \left\lVert \frac{\eenorm{} \times \cmoment}{\eenorm{} \cdot \cforce}\right\rVert \leq \objrad
        \end{equation}
        where the denominator evaluates to a scalar and the numerator evaluates to a 3x1 vector.
        Since it is chosen that the z-axis of the contact frame is aligned with the normal $\eenorm$ of the supporting surface, the vector $\eenorm{} \times \cmoment$ has a z-axis component that is always zero. 
        Let $[a,b,0]^T$ represent a generic vector resulting from the operation in the numerator which is expressed in the contact frame and let $d$ be a generic value resulting from the operation in the denominator. Then,
        \begin{equation}
            \left\lVert 
            \begin{bmatrix}
                a/d \\
                b/d \\
                0
            \end{bmatrix}
            \right\rVert \leq \objrad
        \end{equation}
        which can be rewritten as 
        \begin{equation}
            (a/d)^2 + (b/d)^2 \leq \objrad^2
        \end{equation}
        with the reformulated constraint written as:
        \begin{equation}
            \label{eq:reform_tipcon}
            a^2 + b^2 - d^2 \objrad^2 \leq 0
        \end{equation}
        %where $a$ is the x-component of the of the numerator of the ZMP equation,.
        
        Overapproximations of these individual components are calculated in order to form the polynomial zonotope overapproximation of the tipping constraint.
        The polynomial zonotope overapproximation of the numerator of Eq. \eqref{eq:tipcon} is
        \begin{equation}
            \label{eq:pz_ZMP_numerator}
            \eenorm{} \otimes \pzi{n_{c}} = 
            \begin{bmatrix}
                \pzi{a} \\
                \pzi{b} \\
                0
            \end{bmatrix}
        \end{equation}
        and the overapproximation of the denominator of Eq. \eqref{eq:tipcon} is
        \begin{equation}
            \label{eq:pz_ZMP_denominator}
            \eenorm{} \odot \pzi{f_{c}} = \pzi{d}
        \end{equation}
        Thus an overapproximation of the reformulated tipping constraint in Eq. \eqref{eq:reform_tipcon} can be written as
        \begin{equation}
            \label{eq:pz_tipcon}
            \begin{split}
            \pzi{a} \odot \pzi{a} \oplus \pzi{b} \odot \pzi{b} & \\
            \ominus \pzi{d} \odot \pzi{d} \odot \objrad^2 & \leq 0
            \end{split}
        \end{equation}
        % should probably have another equation where there a PZs in the constraint
        Similar to the coefficient of friction, the radius of the contact area could be uncertain but only the smallest possible value needs to be considered in order to guarrantee that no tipping occurs.
        Therefore, in Eq. \eqref{eq:pz_tipcon}, $\objrad = \texttt{inf}([\objrad_{lower},\objrad_{upper}]$.
        % \Zac{note that uncertainty in the contact area dimension of the object can be captured by replacing $\objrad$ with an interval $[\objrad_{lim}^{-},\objrad_{lim}^{+}]$}
        % \Zac{a conflicts with acceleration in PZRNEA algorithm}
        
        \begin{thm}
            Given 
            \begin{equation}
                \cwrench(t;k) \in \pzki{\cwrenchPZ}, \quad \forall t \in \pz{T_i}, k \in \pzi{K}
            \end{equation} 
            the constraints in Eq. \eqref{eq:pz_optsepcon}-\eqref{eq:pz_opttipcon} overapproximate the constraints in Eq. \eqref{eq:optsepcon}-\eqref{eq:opttipcon} for all time.
        \end{thm}

% \subsection{Analytical Gradients}

\subsection{Trajectory Optimization}

    Using the polynomial zonotope overapproximations of the constraints in the continuous-time optimization problem given in Eq. \eqref{eq:optcost}-\eqref{eq:optsepcon}, a discretized optimization problem is written:
    % Polynomial zonotope formulation of the optimization problem
    \begin{align}
        % cost function
        \label{eq:pz_optcost}
        &\underset{k}{min} &&\texttt{cost}(k, q_{goal}) \\
        % joint position constraint
        \label{eq:pz_optpos}
        &&& \pzqjki \subseteq [\qlim^-, \qlim^+] \quad &\forall i, j \\
        % joint velocity constraint
        \label{eq:pz_optvel}
        &&& \pzqdjki \subseteq [\dqlim^-, \dqlim^+] \quad &\forall i, j \\
        % joint input torque constraint
        \label{eq:pz_opttorque}
        &&& \pzujki \subseteq [\ulim^-, \ulim^+] \quad &\forall i, j \\
        % end-effector position constraint
        % \label{eq:pz_optposcon}
        % &&& \pzki{p_j} \subseteq [p_j^-, p_j^+] \quad &\forall i, j \\
        % end-effector orientation constraint 1
        % \label{eq:pz_optorncon1}
        % &&& \pzi{\hat{z}_{j}; k} \odot \pzi{\hat{z}_{d,j}}  \geq z_{d, j}^- \quad &\forall i, j \\
        % end-effector orientation constraint 2
        % \label{eq:pz_optorncon2}
        % &&& \pzk{\hat{x}_{j}} \odot \pz{\hat{x}_{d,j}}  \geq x_{d, j}^- \quad &\forall i, j \\
        % collision constraint
        \label{eq:pz_optcolcon}
        &&& \pzki{\FO_j} \bigcap \obsset = \emptyset \quad &\forall i, j \\
        % separation constraint
        \label{eq:pz_optsepcon}
        &&& -\pzki{f_{c,z}} \le 0 \quad &\forall i \\
        % linear slipping constraint
        \label{eq:pz_optslipcon}
        %&&& \begin{split}
        &&& \pzki{f_{c,x}} \odot \pzki{f_{c,x}}   \quad &\forall i\\
        &&& \oplus \pzki{f_{c,y}} \odot \pzki{f_{c,y}} \nonumber \\
        &&& \ominus {\mu_{s}}^2\pzki{f_{c,z}} \odot \pzki{f_{c,z}} \le 0  \nonumber \\
        %\end{split} \\
        % rotational slipping constraint
        % \label{eq:optrotslipcon}
        % %&&& \begin{split}
        % &&& \pzi{\czmomentnot{}} \odot \pzi{\czmomentnot{}} \quad &\forall i\\
        % &&& \ominus (\frac{2}{3} \CoefFric \objrad)^2 \pzi{\czforcenot} \odot \pzi{\czforcenot} \leq 0 \nonumber \\
        %\end{split} \\
        \label{eq:pz_opttipcon}
        %&&& \begin{split}
        &&& \pzi{a} \odot \pzi{a} \oplus \pzi{b} \odot \pzi{b}  \quad & \forall i\\
        &&& \ominus \pzi{d} \odot \pzi{d} \odot \objrad^2 \leq 0 \nonumber
        %\end{split} \\
    \end{align}
    \noindent where $i \in \Nt$ and $j \in \Nq$. 
    \Zac{not sure how to format this better.}
    
    
    \begin{thm}
        Any feasible solution $k$ to the optimization problem described in Eq. \eqref{eq:pz_optcost}-\eqref{eq:pz_opttipcon} parameterizes a trajectory that is collision free, satisfies input torque limits, and results in no relative motion between a loosely placed object and the end-effector of the robot over the time horizon $\pz{T}$.
    \end{thm}



%%% Previously written

%In order to ensure that the robot stays safe, if a new plan is not found in time, a braking maneuver is executed.
%This braking maneuver is part of the the previous trajectory, and so satisfies all the constraints. 

%If it does not find a new plan, than a braking maneuver must be executed in order to bring  execute a braking maneuver and come to a stop at a safe state (i.e. zero joint velocity).



%%% Outline for quick reference

% \1 Planning Algorithm Theory
    
%     \2 Overview paragraph: Explain how planning is performed in receding horizon fashion and that each trajectory is certifiably safe. Real time planning is achieved through planning for the next iteration while the current iteration is executing, and we make use of a braking maneuver to ensure safety \Parker{if a new plan cannot be computed in time. Thus, this method is recursively feasible}. 

%     \2 Outline the execution of a single planning iteration, including if braking occurs. Go over all the components of the optimization problem solved during the planning iteration. \Zac{move last sentence closer to opt prob?}
        

%     \2 Describe our approach: Generating polynomial zonotope overapproximations of the trajectory and all of the constraints enables fast optimization that also ensures safety.  Highlight the other benefits of this method.
    
%     \2 Trajectory Overapproximation
    
%         \3 Overview is to describe how a trajectory is overapproximated. 
        
%         \3 First, describe how a planning time interval is overapproximated. 
        
            % \begin{equation}
            %     \label{eq:time_pz}
            %     \pz{T_i} = \frac{(i-1) + i}{2}\timestep + \frac{1}{2} \timestep \tvar
            % \end{equation}  
            % with indeterminate $\tvar \in \iv{-1, 1}$.
        
%         \3 Give definition of trajectory parameter and how the space of trajectory parameters relates to the desired trajectories.
        
%         \begin{defn}
%         \label{def:pz_Kj}
%         We represent the interval $\Kj$ as a poynomial zonotope $\pz{\Kj} = \kjvar$ where $\kjvar \in \iv{-1, 1}$ is an indeterminate.
%         Any particular choice of $k_j$ is trivially related to the corresponding subset $k_j = \texttt{slice}(\pz{\Kj}, \kjvar, k_j)$.
%         Letting $\kvar = (x_{k_1}, x_{k_2}, ..., x_{k_{\nq}})^\top$ we introduce the shorter notation $\pz{\ \cdot \ ; k} = \texttt{slice}(\pz{\ \cdot \ }, \kvar, k)$, which allows us to obtain subsets of polynomial zonotopes corresponding to a choice of $k$ by slicing the corresponding $\kvar$ indeterminates.
%         \end{defn}
        
        
        
%         \3 Describe construction of overapproximation of desired trajectory and how the overapproximated trajectory ensures that the continuous time trajectory lies within.  
        
%         \3 \begin{lem}
%         Overapproximative polynomial zonotope representations of the desired trajectory $\qdeskj$ can be formed by using $\pz{T_i}$ and $\pz{\Kj}$ in the arguments of the functions. 
%         The resulting polynomial zonotope $\pzqdesji$ satisfies
%         \begin{equation}
%             \qdeskj \in \pzi{\qdesk} \quad \forall t \in \pz{T_i}, \kj \in \pz{\Kj}
%         \end{equation}
%         Overapproximative polynomial zonotope representations are similarly constructed for $\pzqddesji$ and $\pzqdddesji$.
%         \end{lem}
        
        
%         \3 Describe how slicing a polynomial zonotope representing the trajectory parameters can be used to recover the trajectory it parameterized.
        
%         \3 \Zac{slice algorithm is given in ARMTD paper. add small section about it in a preliminaries maybe?}
        
%         Given an indeterminate $\pzv_s$ and a value $\sigma \in [-1, 1]$, slicing yields a subset of $\pz{P}$ by plugging $\sigma$ into the specified element $\pzv_s$:
%         \begin{equation}
%             \texttt{slice}(\pz{P}, \pzv_s, \sigma) \subset \pz{P} = \{ z \in \pz{P} \, \mid \, z = \sum_{i=0}^{\pzn} \pzgi \pzv ^{\pzei}, \, \pzv_s = \sigma \}.
%         \end{equation}
        
%     \2 Reachable Set Construction
    
%         \3 Describe how the overapproximated joint trajectories are used in the computation of arm kinematics and dynamics.
        
%         \3 Forward Kinematics Reachable Set
            
%             \4 describe how the polynomial zonotope overapproximation of the joint trajectories is used to calculate the polynomial zonotope overapproximation of the forward kinematics of the robot.
            
%             \4 give regular FK to motivate need for sine and cosine overapproximations?
            
%             \4 \Zac{theorem that sin and cos of pzs are also overapproximative. Taylor expansion and overapproximate the remainder?}
        
%             \4 \begin{thm}
%             The sine and cosine of a polynomial zonotope can be overapproximated by computing a Taylor expansion series with an overapproximated Lagrange Remainder.
%             \end{thm}
        
%             \4 polynomial zonotope forward kinematics for the $j^{th}$ frame at the $i^{th}$ timestep:
%             \begin{equation}\label{eq:pzfk_j}
%                 \pzi{\FK_j} = 
%                 \begin{bmatrix} \pzi{R_j} & \pzi{p_j}\\
%                 \mathbf{0}  & 1 \\
%                 \end{bmatrix},
%             \end{equation}
%             where
%             \begin{equation}
%                 \pzi{R_j} = \prod_{l=1}^{j} \pzi{R_{l}^{l-1}}
%             \end{equation}
%             and
%             \begin{equation}
%                 \pzi{p_j} = \sum_{l=1}^{j} \pzi{R_l} \pzi{p_{l}^{l-1}}.
%             \end{equation}
            

            
%             \4 
%             \begin{thm}
%             \label{thm:FK_overapprox}
%             Given that $sin(\pz{q_i})$ and $cos(\pz{q_i})$ are overapproximative, then $\pz{\FK}$ is an overapproximation of the forward kinematics of the robot, i.e. $\FK_{j,i} \in \pzji{\FK} \quad \forall \pz{T_i}$.
%             \end{thm}
            
%         \3 Forward Occupancy Reachable Set
        
%             \4 The forward occupancy is overapproximated using the overapproximated forward kinematics. This is used to ensure the robot does not collide with obstacles in the environment.
            
%             \4 \Zac{need to add how $\pz{L_j}$ is constructed. is this just using the CORA toolbox?}
            
%             \4 
%             \begin{align}\label{eq:pz_forward_occupancy_j}
%                  \pzi{\FO_j} = \pzi{p_j} \oplus \pzi{R_j} \odot \pz{L_j}.
%             \end{align}
            
            
%             \4 
%             \begin{thm}
%             Given that $\pzi{p_j}$, $\pzi{R_j}$ and $\pz{L_j}$ are overapproximations, then $\FO_{j,i} \in \pzi{\FO_j} \quad \forall t \in \pz{T_i}$.
%             \end{thm}

%         \3 Input Reachable Set
        
%             \4 Describe the construction of an overapproximation of the input. (This comes from the T-RO paper)
            
%             \4 The nominal control input is overapproximated 
            
%             \begin{equation}
%                 \label{eq:pz_nominal_input}
%                 \pzi{\tau} = \bM(\pzi{q}, \nomparams) \pzi{\ddot{q}_a} + \bC(\pzi{q}, \pzi{\dot{q}},\nomparams) \pzi{\dot{q}_a} + \bG(\pzi{q}, \nomparams).
%             \end{equation}
            
%             \4 Theorem that $\norm{\robv}$ is bounded:
            
%             \begin{thm}
%             The norm of the robust input $\norm{\robv}$ at the $i$\ts{th} timestep is bounded by
%             \begin{equation}
%                 \label{eq:pz_robust_input_bound}
%               \norm{\robv} \leq \frac{-\robKinf(\texttt{inf} \pzi{h})}{\ultbound} + \norm{\rho(\pzi{w})}
%             \end{equation}
%             for all $(q, \robr) \in \robH$, where $\pzi{h}$ and $\pzi{w}$ are polynomial zonotope versions of the CBF $h$ and disturbance $\wdist$ respectively.
%             \end{thm}
            
%             \4 Final result is that the robust input $\pzi{u}$ is overapproximated: 
%             \begin{equation}
%             \label{eq:pz_input}
%                 \pzi{u} = \pzi{\tau} - \pzi{v}.
%             \end{equation}
            
%             \4 \begin{thm}
%             Given that $\pzi{\tau}$ and $\pzi{v}$ are overapproximations, the control input $\pzi{u}$ is overapproximated.
%             \end{thm}
            
%         \3 End Effector Wrench Reachable Set
        
%             \4 Describe the construction of an overapproximation of the end effector wrench. This is done through using PZ-RNEA and the overapproximated joint trajectories. (Likely need a theorem/proof stating that this method does result in an overapproximated wrench?)
            
%             \4 \begin{thm}
%             Given $\pz{\q}$, $\pz{\qd}$, $\pz{\qadot}$, $\pz{\qdd}$, and $\pz{\Delta}$ are overapproximative, then algorithm \ref{alg:PZRNEA} results in an overapproximation of the wrench $[\pz{f\jss},  \pz{n\jss}]^{T}$ exerted on joint $j$.
%             \end{thm}
            
%             \Zac{Note: need to update PZ-RNEA algorithm with the wrench output}
            
            
%     \2 Constraint Generation
    
%         \3 Describe how the constraints are written using the reachable sets. 
        
%             \4 Separation constraint is the Fz related component of the contact wrench. \Zac{need to add notation for specifying axial component of force}.
            
%             \4 Friction constraint is rewritten to involve only summation and multiplication operations.
            
%             \4 Tipping constraint is rewritten to involve only summation and multiplication operations.
        
        
%         \3 \begin{thm}
%         Given $[\pz{f\jss},\pz{n\jss}]^{T}$, the constraints (will reference eqn numbers when added) are overapproximative.
%         \end{thm}

    
%     \2 Trajectory Optimization
    
%         \3 Polynomial zonotope formulation of the optimization problem
        
%         \begin{align}
%             \label{eq:optcost}
%             &\underset{k}{min} &&\texttt{cost}(k, q_{goal}) \\
%             \label{eq:pz_optpos}
%             &&& \pzqjki \subseteq [\qlim^-, \qlim^+] \qquad &\forall i, j \\
%             \label{eq:pz_optvel}
%             &&& \pzqdjki \subseteq [\dqlim^-, \dqlim^+] \qquad &\forall i, j \\
%             \label{eq:pz_opttorque}
%             &&& \pzujki \subseteq [\ulim^-, \ulim^+] \qquad &\forall i, j \\
%             \label{eq:pz_optposcon}
%             % &&& \pzki{p_j} \subseteq [p_j^-, p_j^+] \qquad &\forall i, j \\
%             % \label{eq:pz_optorncon1}
%             % &&& \pzi{\hat{z}_{j}; k} \odot \pzi{\hat{z}_{d,j}}  \geq z_{d, j}^- \qquad &\forall i, j \\
%             % \label{eq:pz_optorncon2}
%             % &&& \pzk{\hat{x}_{j}} \odot \pz{\hat{x}_{d,j}}  \geq x_{d, j}^- \qquad &\forall i, j \\
%             \label{eq:pz_optcolcon}
%             &&& \pzki{\FO_j} \bigcap \obsset = \emptyset \qquad &\forall i, j \\
%             \label{eq:pz_optsepcon}
%             &&& -1*\pzki{\FNorm} \le 0 &\forall i, j \\
%             \label{eq:pz_optslipcon}
%             % &&& \pzki{\FTan}*\pzki{\FTan} - {\mu_{s}}^2*\pzki{\FNorm}*\pzki{\FNorm} &\forall i, j \\
%             &&& |\pzki{\FTan}| - {\mu_{s}}|\pzki{\FNorm}| \le 0 &\forall i, j \\
%             \label{eq:pz_opttipcon}
%             &&& |\pzki{\ZMP}| - r \le 0 &\forall i, j
%             % \pzki{\MG}  \surfnorm - \pzki{\FG} \cdot \surfnorm * \objrad \le 0
%         \end{align}
%         \noindent where $i \in \Nt$ and $j \in \Nq$ and $r$ is the radius of the contact patch (assumed to be a circular contact patch). 
        
        
%         \begin{thm}
%         Any feasible solution to \ref{pz_optpos} parameterizes a trajectory that is collision free, satisfies input torque limits, and results in no relative motion between a loosely placed object and the end-effector of the robot over the time horizon $\pz{T_i}$.
%         \end{thm}

==> Sections/preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelims}

This section details the set representations and operations used throughout the paper.

\subsection{Notation}

    % need
    The $n$-dimensional real numbers are denoted by $\R^n$ and the natural numbers are denoted by $\N$. %, the unit circle is $\mathbb{S}^1$, and the set of $3 \times 3$ orthonormal matrices is $\SO(3)$.
    Upper case letters represent sets or matrices, while lowercase letters represent vectors or scalars.
    Subscripts either index elements of a vector, elements of a set or denotes the frame a vector is expressed in, depending on context.
    For a matrix $A$, we use $A^\top$ to denote its transpose.
    
    % need
    Let $U$, $V \subset \R^n$.
    For a point $u \in U$, $\{ u \} \subset U$ is the set containing only $u$.
    The \emph{power set} of $U$ is $\pow{U}$.
    The \emph{Minkowski Sum} is $U \oplus V  = \{ u + v \, \mid \, u \in U, v \in V \}$.
    For vectors $a, b \in \R^3$, the cross product $a \times b$ can be expressed as $a^\times b$, where
    \begin{equation}
        \label{eq:cross_product_matrix}
        a^\times= \begin{bmatrix}
        0 & -a_3 & a_2 \\
        a_3 & 0 & -a_1 \\
        -a_2 & a_1 & 0
        \end{bmatrix}.
    \end{equation}
    If $n = 3$, the \emph{set-based cross product} is defined as $U \otimes V = \{ u \times v \, \mid \, u \in U, v \in V \}$.
    Let $W \subset \R^{n \times n}$ be a set of square matrices.
    Then, \emph{set-based multiplication} is defined as $WV = \{ Av, \, \mid \, A \in W, v \in V \}$.
    Let $\zeros$ and $\ones$ denote matrices of zeros and ones of appropriate size, and $\eye$ be the $n \times n$ identity matrix.

\subsection{Intervals}
    
    % need
    The simplest set representation we use is the interval.
    An \emph{n-dimensional interval} is a set of real numbers
    \begin{align}
        \interval{x} &=  \{ y \in \R^n \, \mid \,\underline{x}_i \leq y_i \leq \overline{x}_i,  \quad \forall i = 1, \ldots, n\}.
    \end{align}
    Note we have abused notation and used a lowercase letter to denote a set here; however, the $\interval{\cdot}$ notation hopefully makes clear that this indeed means a set. 
    For succinctness, we sometimes denote an interval $\interval{x}$ by $\interval{\underline{x}, \overline{x}}$, where $\underline{x}$ and $\overline{x}$ are the infimum and supremum, respectively, of $\interval{x}$.
    Let the operations $\texttt{inf}$ and $\texttt{sup}$ return the infimum and supremum of an interval:
    \begin{align}
        \texttt{inf}(\iv{x}) &= \underline{x} \\
        \texttt{sup}(\iv{x}) &= \overline{x}.
    \end{align}
    Let $\mathbb{I}\mathbb{R}^{n}$ be the set of all real-valued $n$-dimensional interval vectors. 
    
    % need
    The Minkowski sum and difference of $\interval{x}$ and $\interval{y}$ are given by
    \begin{gather}
        \interval{x} \oplus \interval{y} = \interval{\underline{x} + \underline{y}, \overline{x} + \overline{y}}, \\
        \interval{x} \ominus \interval{y} = \interval{\underline{x} - \overline{y}, \overline{x} - \underline{y}}.
    \end{gather}
    The product of $\interval{x}$ and $\interval{y}$ is
    \begin{equation}
        \interval{x} \interval{y} = [\min(\underline{x} \underline{y}, \underline{x} \overline{y},\overline{x}\underline{y}, \overline{x} \overline{y}), \max(\underline{x} \underline{y}, \underline{x} \overline{y},\overline{x}\underline{y}, \overline{x} \overline{y}) ].
    \end{equation}
    
    % need
    Given a scalar interval $\interval{a}$ or interval matrix $\interval{Y}$ multplied by an interval matrix $\interval{X}$, the element in the $i^{th}$ row and $j^{th}$ column of the product is
    \begin{gather}
        (\interval{a} \interval{X})_{ij} = \interval{a} \interval{X}_{ij}, \\
        (\interval{X} \interval{Y})_{ij} = \bigoplus_{k=1}^n (\interval{X}_{ik} \interval{Y}_{kj}),
    \end{gather}
    where $n$ is the number of columns of $\interval{X}$ and number of rows of $\interval{Y}$.
    Lastly, given two interval vectors $\interval{x},\interval{y} \subset \R^3$, their cross product is
    \begin{align}
        \interval{x} \otimes \interval{y} = \interval{x}^{\times} \interval{y}.
    \end{align}

\subsection{Zonotopes}

    A \emph{zonotope} $Z \subset \R^n$ is a convex, centrally-symmetric polytope defined by a \emph{center} $g_0 \in \R^n$ and \emph{generators} $g_i \in \R^n$:
    \begin{equation}
    \label{eq:zonotope}
        Z = \{ z \in \R^n \, \mid \, z = g_0 + \sum_{i=1}^{\pzn} g_i \beta_i, \quad \beta_i \in [-1, 1] \}
    \end{equation}
    where there are $\pzn \in \N$ generators, and $\beta_i \in [-1, 1]$ are called indeterminates.
    \begin{lem}
        \label{lem:interval_over_zono}
        A zonotope can be overapproximated by an interval.
    \end{lem}
    \begin{proof}
        Consider $Z \subset \R^n$ with center $c$ and $\pzn$ generators $g_i$.
        Then, 
        \begin{equation}
            Z \subseteq \left[g_0 - \sum_{i=1}^{\pzn} |g_i|,\ 
                g_0 + \sum_{i=1}^{\pzn} |g_i|\right].
        \end{equation}
    \end{proof}
    
    The Minkowski sum of a pair of zonotopes is a zonotope. 
    To see this, consider $Z_1 \subset \R^n$ with center $g_0$ and $p$ generators $g_i$ with indeterminates $\beta_i$, and $Z_2 \subset \R^n$ with center $h_0$ and $q$ generators $h_j$ with indeterminates $\lambda_j$:
    \begin{align}
        Z_1 \oplus Z_2 &= \{ z \in \R^n \, \mid \, z = z_1 + z_2, z_1 \in Z_1, z_2 \in Z_2 \} \\
        \begin{split} 
        Z_1 \oplus Z_2 &= \{ z \in \R^n \, \mid \, z = (g_0 + h_0) + \sum_{i=1}^{\pzn}g_i\beta_{i} + \sum_{j=1}^{q}h_j\lambda_{j} ,  \\
                & \phantom{ \{ z \in \R^n \, \mid \, z =} \beta_i \in [-1, 1], \, \lambda_j \in [-1, 1] \}.
        \end{split}
    \end{align}
    
    Zonotopes can also represent sets of matrices.
    Let $M \subset \R^{n \times m}$ be a matrix zonotope which is a zonotope whose center $G_0 \in \R^{n \times m}$ and generators $G_i$ are matrices:
    \begin{equation}
        M = \left\{ A \in \R^{n \times m} \, \mid \, A = G_0 + \sum_{i=1}^{\pzn} G_i \beta_i \right\}.
    \end{equation}
    This work uses matrix zonotopes to represent sets of rotations, and zonotopes to represent the volume of a link.
    To represent the swept volume corresponding to uncertain rotations, it is necessary to take the product of matrix zonotopes and zonotopes.
    We use zonotope representations since they can provide a tighter outer approximation of the swept volume of a manipulator compared to interval set representations.
    Let $M$ be a matrix zonotope with $p$ generators $G_i$ with indeterminates $\beta_i$.
    Let $Z$ be a zonotope with $q$ generators $h_j$ with indetermintes $\lambda_j$.
    Then the product is defined as: 
    \begin{align}
        M\odot Z &= \{ z \in \R^n \, \mid \, z = Ay,  \, A \in M, y \in Z \} \\
        M\odot Z &= \bigg\{ z \in \R^n \, \mid \, z = G_0 g_0 + \sum_{j=1}^{q} G_0 g_j \lambda_j + \sum_{i=1}^{\pzn} G_i g_0 \beta_i +  \nonumber \\
        &  + \sum_{i=1}^{\pzn}\sum_{j=1}^{q} G_i g_j\beta_i\lambda_j, \, \beta_i \in [-1, 1], \lambda_j \in [-1, 1] \bigg\}
    \end{align}
    However, the result is no longer a zonotope due to the products of indeterminates $\beta_i \lambda_j$.
    This motivates the need for a more complex set representation called polynomial zonotopes \cite{kochdumper2020sparse}.

\subsection{Polynomial Zonotopes}

    For a thorough introduction to polynomial zonotopes, we refer the reader to \cite{kochdumper2020sparse}.
    We present an overview of the necessary definitions and operations here.
    
    First, zonotopes are a subset of polynomial zonotopes, so we redefine zonotopes using an alternate notation.
    Let the zonotope $Z$ have center $g_0$, $\pzn$ generators $\pzgi$, and indeterminates $\beta_i$.
    We introduce an indeterminate vector $\pzv \in [-1, 1]^\pzn$ such that the $i^{th}$ element of $\pzv$ is the indeterminate $\beta_i$. Then we introduce the exponents $\pzei \in \N^\pzn$.
    Letting $\pze_1 = [1, 0, \ldots, 0]$, $\pze_2 = [0, 1, 0, \ldots, 0]$, \ldots, $\pze_\pzn = [0, 0, \ldots, 0, 1]$, we note that $\pzv^{\pze_1} = \pzv_1, \ldots ,\pzv^{\pze_\pzn} = \pzv_\pzn$ where the exponentiation is applied element-wise.
    We refer to $\pzv ^{\pzei}$ as a \textit{monomial}, and a \textit{term} $\pzgi\pzv ^{\pzei}$ is produced by multiplying a monomial by the associated generator $\pzgi$.
    Then, letting the center $\pzg_0$ be associated with the exponent $\alpha_0 = [0, 0, \ldots, 0]$, we may write the zonotope $Z$ as 
    \begin{equation}
        \label{eq:first_pz_definition}
        Z = \{ z \in \R^n \, \mid \, z = \sum_{i=0}^{\pzn} \pzgi \pzv ^{\pzei}, \, \pzv \in [-1, 1]^\pzn \}.
    \end{equation}
    Note that in \eqref{eq:first_pz_definition}, a zonotope is defined with each $\pzei$ having only one nonzero element.
    For polynomial zonotopes, each $\pzei \in \N^\pzn$ may have arbitrary components.
    
    A polynomial zonotope $\pz{P} \subset \R^n$ is given by its coefficients, exponents, and indeterminates.
    We write $\pz{P} = \PZ{\pzgi, \pzei, \pzv}$.
    In latter sections, we will distinguish between how indeterminate terms appear within a polynomial zonotope:
    \begin{defn}
    Let $\pzei$ have only one nonzero element (the $k$-th element) . 
    If the $k$-th element is zero for all $\alpha_j, j \neq i$, then the term $\pzgi\pzv ^{\pzei}$ is called \emph{independent}.
    This implies that $\pzgi\pzv ^{\pzei}$ depends only on $k$-th indeterminate $\pzv_k$, and this indeterminate does not appear in any other term within the polynomial zonotope, $\pzv_k \notin \pzgj\pzv ^{\pzej},\ j \neq i$.
    A term which does not meet these criteria is called \emph{dependent}.
    \end{defn}
    
    We can convert $[z]$ to a polynomial zonotope $\pz{z}$ using
    \begin{equation}
        \label{eq:int_to_pz}
        \pz{z} = \frac{\overline{z} + \underline{z}}{2} + \sum_{i = 1}^{n}\frac{\overline{z}_i - \underline{z}_i}{2}x_i,
    \end{equation}
    where $x \in [-1, 1]^n$ is the indeterminate vector.
    
    The Minkowski Sum of two polynomial zonotopes $\pz{P_1} \subset \R^n = \mathcal{PZ}( \pzgi, \pzei, \pzv ) $ and $\pz{P_2} \subset \R^n = \mathcal{PZ}( h_j, \beta_j, y )$ follows polynomial addition:
    \begin{align}
        \pz{P_1} \oplus \pz{P_2} = \{ z \in \R^n \, \mid \, z = p_1 + p_2, p_1 \in \pz{P_1}, p_2 \in \pz{P_2} \} \\
        \pz{P_1} \oplus \pz{P_2} = \{ z \in \R^n \, \mid \, z = \sum_{i=0}^{\pzn} \pzgi \pzv ^{\pzei} + \sum_{j=0}^{q} h_j y^{\beta_j} \}.
    \end{align}
    Similarly, we may write the matrix product of two polynomial zonotopes $\pz{P_1}$ and $\pz{P_2}$ when the sizes are compatible (i.e., elements in $\pz{P_1}$ have the same number of columns as elements of $\pz{P_2}$ have rows).
    Letting $\pz{P_1} \subset \R^{n \times m}$ and $\pz{P_2} \subset \R^{m \times k}$, we obtain $\pz{P_1} \pz{P_2} \subset \R^{n \times k}$:
    \begin{align}
        \pz{P_1} \pz{P_2} &= \{ z \in \R^{n \times k} \, \mid \, z = p_1p_2, p_1 \in \pz{P_1}, p_2 \in \pz{P_2} \} \\
        \pz{P_1} \pz{P_2} &= \{ z \in \R^{n \times k} \, \mid \, z = \sum_{i=0}^{\pzn} \pzgi(\sum_{j=0}^{q} h_j y^{\beta_j}) \pzv ^{\pzei} \}.
    \end{align}
    
    Furthermore, if $\pz{P_1} \subset \R^{3}$ and $\pz{P_2} \subset \R^{3}$, we implement a set-based cross product as matrix multiplication.
    We create $\pz{P_1}^{\pzv} \subset \R^{3 \times 3}$ as
    \begin{align}
        \pz{P_1}^{\pzv} = \{ A \in \R^{3 \times 3} \, \mid \, A = \sum_{i = 0}^{\pzn} \begin{bmatrix} 0 & -\pzg_{i,3} & \pzg_{i,2} \\ \pzg_{i,3} & 0 & -\pzg_{i,1} \\ -\pzg_{i,2} & \pzg_{i,1} & 0 \end{bmatrix} \pzv ^{\pzei} \}
    \end{align}
    where $a_{i, j}$ refers to the $j^{th}$ element of $a_i$.
    Then, the set-based cross product $\pz{P_1} \otimes \pz{P_2} = \pz{P_1}^{\pzv} \pz{P_2}$ is well-defined. 
    Addition, multiplication and the cross product of a polynomial zonotope with a constant vector or matrix is well-defined if the constant is appropriately sized.
    The vector or matrix can be represented as a polynomial zonotope with that constant vector or matrix as the center $g_0$ and no other generators.
    Note that for Minkowski summation and multiplication of polynomial zonotopes, it is possible that $\pz{P_1}$ and $\pz{P_2}$ may share indeterminates.
    It is beneficial to bring both polynomial zonotopes to a \textit{common representation} before performing these operations. 
    Letting $\tilde{\pzv} = \pzv \union y$, we may redefine the polynomial zonotopes $\pz{P_1} = \pz{ \pzgi, \tilde{\alpha}_i, \tilde{\pzv} }$ and $\pz{P_2} = \pz{ h_i, \tilde{\beta}_i, \tilde{\pzv} }$ where $\tilde{\alpha}_i$ and $\tilde{\beta}_j$ exponentiate the appropriate elements of $\tilde{\pzv}$.
    
    Next, we introduce the ``slicing'' operation, which is where a subset of a polynomial zonotope $\pz{P}$ is obtained through plugging in values of known indeterminates.
    This can be used to check whether a particular choice of $\pz{P}$'s indeterminates yields a subset that satisfies or does not satisfy certain properties, such as collision with an obstacle.
    Given an indeterminate $\pzv_s, \ s \in \{1,\ldots,\pzn\}$ and a value $\sigma \in [-1, 1]$, slicing yields a subset of $\pz{P}$ by plugging $\sigma$ into the specified element $\pzv_s$:
    \begin{equation}
        % \begin{split}
        % \texttt{slice}(\pz{P}, \pzv_s, \sigma) \subset \pz{P} \\
        \texttt{slice}(\pz{P}, \pzv_s, \sigma) = \{ z \in \pz{P} \, \mid \, z = \sum_{i=0}^{\pzn} \pzgi \pzv ^{\pzei}, \, \pzv_s = \sigma \}.
        % \end{split}
    \end{equation}
    
    Next, we introduce a way to efficiently compute bounds of the elements of a polynomial zonotope.
    This is done through defining the $\texttt{sup}$ and $\texttt{inf}$ operations which return an upper and lower bound, respectively, by taking the absolute values of the generators.
    For $\pz{P} \subseteq \R^n$, these return
    \begin{align}
        \texttt{sup}(\pz{P}) = g_0 + \sum_{i=1}^{\pzn} \abs{\pzgi}, \label{eq:pz_sup}\\
        \texttt{inf}(\pz{P}) = g_0 - \sum_{i=1}^{\pzn} \abs{\pzgi}. \label{eq:pz_inf}
    \end{align}
    Note that for any $z \in \pz{P}$,  $\texttt{sup}(\pz{P}) \geq z$ and $\texttt{inf}(\pz{P}) \leq z$, where the inequalities are taken element-wise.
    While these operations are efficient to compute, they may be be tight because possible dependencies between indeterminates are not accounted for, resulting in a larger overapproximation.
    
    % The operations defined above (multiplication in particular) increases the number of generators required to represent a polynomial zonotope, therefore increasing the memory required to store a polynomial zonotope.
    % In practice, successively applying these operations can become computationally intractable.
    % To combat this computational burden, we define a \defemph{reduce} operation for a polynomial zonotope.
    % The reduce operation generates overapproximations of polynomial zonotopes through using fewer generators.
    % If a polynomial zonotope $\pz{P} \subset \R^n$ has $\pzn$ terms, but a maximum of $q$ terms are desired, excess terms can be overapproximated by an interval:
    % \begin{align}
    %     \label{eq:pz_reduce}
    %     \setop{reduce}(\pz{P}, n_h) = \left\{ z \in \R^n \, \mid \, z \in \sum_{i=0}^{n_h-n} \pzgi \pzv ^{\pzei} \oplus [-b, b]\right\}
    % \end{align}
    % where $b_j$ is equal to $\sum_{i=n_h-n+1}^{\pzn} | g_{i,j} |$ where $g_{i,j}$ is the $j$\ts{th} element of $\pzgi$.
    % This means that the last $\pzn - n_h - n + 1$ terms are overapproximated by an $n$-dimensional hyperbox represented by an interval.
    % This interval can be expressed as a polynomial zonotope as in \eqref{eq:int_to_pz}, and so the output of $\setop{reduce}(\pz{P}, q)$ is itself a polynomial zonotope.
    % % \pat{this was not quite written right... sum is over the $j$-th dimension}
    % Notice that $\setop{reduce}(\pz{P}, q)$ always overapproximates $\pz{P}$, i.e. $\pz{P} \subseteq \setop{reduce}(\pz{P}, q)$ \cite[Prop. 16]{kochdumper2020sparse}.
    % One can reorder the terms of the polynomial zonotope such that only certain desirable terms are replaced by intervals, e.g. to produce a tighter overapproximation.
    
    % We also point out that one can ``free'' a dependent term by replacing it with an independent term, resulting in an overapproximation.
    % This may be desirable if the dependence of a term on an indeterminate is no longer desired.
    % Here, we assume the $\pzn$-th term of $\pz{P}$ is to be made independent:
    % \begin{equation}
    %     \texttt{free}(\pz{P}) = \{ z \in \R^n \, \mid \, z = \sum_{i = 0}^{\pzn-1}  \pzgi \pzv ^{\pzei} + \pzg_\pzn \beta, \, \beta \in [-1, 1] \}.
    % \end{equation}
    % Again, one can reorder the terms of $\pz{P}$ before applying this operation to overapproximate the desired term.
    % Finally, we note that the outputs of $\texttt{reduce}$ and $\texttt{free}$ may be represented as polynomial zonotopes \Ram{citation? or can we actually show that it can be represented as a polynomial zonotope?}.
    
    Though we have defined several basic operations like addition and multiplication above, it may be desirable to use polynomial zonotopes as inputs to more complicated functions.
    In fact, one can overapproximate any analytic function evaluated over a polynomial zonotope using a Taylor expansion, which itself can be represented as a polynomial zonotope \cite[Sec 4.1]{althoff2013reachability}\cite[Prop. 13]{kochdumper2020sparse}.
    Consider an analytic function $f: \R \to \R$ and polynomial zonotope $\pz{P_1} = \PZ{ \pzgi, \pzei, \pzv }$, with each $\pzgi \in \R$.
    Then, 
    \begin{equation}
        f(\pz{P_1}) = \{ y \in \R \; | \; y = f(z), z \in \pz{P_1} \}.
    \end{equation}
    We generate a polynomial zonotope $\pz{P_2}$ such that $f(\pz{P_1}) \subseteq \pz{P_2}$ using a Taylor expansion of degree $d \in \N$, where the error incurred from the finite approximation is overapproximated using a Lagrange remainder.
    The method follows the Taylor expansion found in the reachability algorithm in \cite{kochdumper2020sparse}, which builds on previous work on conservative polynomialization found in \cite{althoff2013reachability}.
    Recall that the Taylor expansion about a point $c \in \R$ is
    \begin{equation}
        f(z) = \sum_{n = 0}^{\infty} \frac{f^{(n)}(c)}{n!} (z - c)^n,
    \end{equation}
    where $f^{(n)}$ is the $n^{th}$ derivative of $f$.
    Note that the error incurred by a finite Taylor expansion can be bounded using the Lagrange remainder $r$ \cite[7.7]{apostol1991calculus}:
    \begin{equation}
        |f(z) - \sum_{n=0}^{d} \frac{f^{(n)}(c)}{n!} (z - c)^n | \leq r,
    \end{equation}
    where $r$ is given by
    \begin{align}
        r &= \frac{M |z - c |^{d+1}}{(d+1)!}, \\
        M &= \underset{\delta \in [c,z]} {\max}( | f^{d+1}(\delta) | ).
    \end{align}
    
    For a polynomial zonotope, the infinite dimensional Taylor expansion is given by
    \begin{equation}
    \label{eq:taylor_pz_inf}
        f(\pz{P_1}) =
        \sum_{n=0}^{\infty}
        \frac{f^{(n)}(c)}{n!} 
        (\pz{P_1} - c)^n 
    \end{equation}
    In practice, only a finite Taylor expansion of degree $d \in \N$ can be computed.
    Letting $c = \pzg_0$ (i.e., the center of $\pz{P_1}$), and noting that $(z - c) = \sum_{i=1}^{\pzn}\pzgi \pzv ^{\pzei}$ for $z \in \pz{P_1}$, we write
    \begin{equation}
    \label{eq:taylor_pz_fin}
        \pz{P_2} \coloneqq \{ z \in \R \, | \, z =
        \sum_{n=0}^{d} \left (
        \frac{f^{(n)}(\pzg_0)}{n!} 
        (\sum_{i=1}^{\pzn}\pzgi \pzv ^{\pzei})^n 
        \right )
        + [r] \}
    \end{equation}
        % \pat{bleh doesn't quite make sense}
    and the Lagrange remainder $[r]$ can be computed using interval arithmetic as
    \begin{align}
        [r] &= \frac{[M] [(\pz{P_1} - c)^{d+1}]}{(d+1)!}, \\ 
        [M] &= f^{(d+1)}([\pz{P_1}])
    \end{align}
    where $[(\pz{P_1} - c)^{d+1}] = [\texttt{inf}((\pz{P_1} - c)^{d+1}), \texttt{sup}((\pz{P_1} - c)^{d+1})]$ is an overapproximation of $(\pz{P_1} - c)^{d+1}$.
    Note that $\pz{P_2}$ can be expressed as a polynomial zonotope because all terms in the summation are polynomials of $\pzv$, and an interval can be expressed as a polynomial zonotope as in \eqref{eq:int_to_pz}.
    Just as we denote polynomial zonotopes using bold symbols, we denote the polynomial zonotope overapproximation of a function evaluated on a zonotope using bold symbols (\emph{i.e.}, $\pz{f}(\pz{P}_1)$ is the polynomial zonotope over approximation of $f$ applied to $\pz{P}$). 
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% need zonotope or PZ can overapproximate interval
% need overapproximate volumes as union of convex polytopes
% need reduce operation for PZ

% add slice function

%     Given an indeterminate $\pzv_s$ and a value $\sigma \in [-1, 1]$, slicing yields a subset of $\pz{P}$ by plugging $\sigma$ into the specified element $\pzv_s$:
%     \begin{equation}
%         \label{eq:slice_operation}
%         \begin{split}
%         \texttt{slice}(\pz{P}, \pzv_s, \sigma) \subset \pz{P} = \\
%         \{ z \in \pz{P} \, \mid \, z = \sum_{i=0}^{\pzn} \pzgi \pzv ^{\pzei}, \, \pzv_s = \sigma \}.
%         \end{split}
%     \end{equation}

% % add Minkowski Sum

% % add intervals can be overapproximated by PZs

% % Taylor series expansion of a polynomial zonotope

% For a polynomial zonotope, the infinite dimensional Taylor expansion is given by
% \begin{equation}
% \label{eq:taylor_pz_inf}
%     f(\pz{P_1}) =
%     \sum_{n=0}^{\infty}
%     \frac{f^{(n)}(c)}{n!} 
%     (\pz{P_1} - c)^n 
% \end{equation}

% In practice, only a finite Taylor expansion of degree $d \in \N$ can be computed.
% Letting $c = \pzg_0$ (the center of $\pz{P_1}$), and noting that $(z - c) = (\sum_{i=1}^{\pzn}\pzgi \pzv ^{\pzei})$ for $z \in \pz{P_1}$, we write
% \begin{equation}
% \label{eq:taylor_pz_fin}
%     \pz{P_2} \coloneqq \{ z \in \R \, | \, z =
%     \sum_{n=0}^{d} \left (
%     \frac{f^{(n)}(\pzg_0)}{n!} 
%     (\sum_{i=1}^{\pzn}\pzgi \pzv ^{\pzei})^n 
%     \right )
%     + [R] \}
% \end{equation}
% % \pat{bleh doesn't quite make sense}
% and the Lagrange remainder $[R]$ can be computed using interval arithmetic as
% \begin{equation}
%     [R] = \frac{[M] [\pz{P_1}]^d}{(d+1)!},
%     \, [M] = f^{(d+1)}([\pz{P_1}])
% \end{equation}
% \bohao{I think this should be $(\pz{P_1} - c)^d$ or $([\pz{P_1}] - c)^d$?}
% where $[\pz{P_1}]$ is an overapproximation of $\pz{P_1}$ by an interval that can be computed using the $\texttt{sup}$ \eqref{eq:pz_sup} and $\texttt{inf}$ \eqref{eq:pz_inf} operations.
% Note that $\pz{P_2}$ can be expressed as a polynomial zonotope because all terms in the summation are polynomials of $\pzv$, and an interval can be included using an independent generator.

% \bohao{A general complaint: I think we should explain the difference between PZ and Taylor model.}

==> Sections/trajectory_design.tex <==
\section{Trajectory Design}
\label{sec:traj_des}


%% Intro
\MethodName{} operates in a receding horizon fashion where each planning iteration solves an optimization program which determines a safe reference trajectory.
The following two subsections detail the structure of the reference trajectories and how they are parameterized.

\subsection{Trajectory Design}
% describe time interval
For each planning iteration, \MethodName{} plans over a compact time interval $ T \subset \R$. 
Without loss of generality, let each planning iteration begin at time $t = 0$ and end at time $t = \tfin$.
In order for \MethodName{} to operate persistently, we require that \MethodName{} finds a new plan before the previous plan finishes executing. 
Let the time for finding a new plan be $t_{plan}$.

% \Zac{feel like more of the structure should be discussed here? otherwise what is the point of this section? could also move to later as subsection of algorithm theory?}

\subsection{Trajectory Parameterization}
During each planning iteration, an optimization program determines a safe reference trajectory.
The decision variable space of the optimization program is a compact set $K \subset \R^{n_k}$, where $n_k \in \N$, which represents a continuum of user-designed reference trajectories.
Each \textit{trajectory parameter} $k \in K$ uniquely determines a reference trajectory.
Therefore the result of each planning iteration is a unique desired reference trajectory for the system to track.
The continuum of user-designed reference trajectories must satisfy the following properties:

\begin{defn}
    \label{def:traj_param}
    For each $k \in K$, a \emph{reference trajectory} is a function $q_d : T \to \Q$ that satisfies the following properties: % (\cdot; k)
    
    \begin{enumerate}
    
    \item The trajectory starts at a specified initial condition $(\initq, \initdq, \initddq)$, so that $q_d(0; k) = \initq$, $\dot{q}_d(0; k) = \initdq$, and $\ddot{q}_d(0; k) = \initddq$.
    
    \item $\dot{q}_d(\tfin; k) = 0$  (i.e., each trajectory brakes to a stop, and at the final time has zero velocity ).
    % \Zac{ Removed the following aspects as I am not currently using Bernstein polynomials: "and $\ddot{q}_d(\tfin; k) = 0$", "and acceleration"}
    
    \item $\ddot{q}_d$ is Lipschitz continuous and bounded. % (\cdot; k)
    
    \end{enumerate}
\end{defn}

The first property enables the desired trajectories that are generated online to account for varying initial conditions. 
The second property enables persistent feasibility since a failsafe braking maneuver is always available as part of the solution of the previous planning iteration.
This is discussed in more detail in Sec. \ref{sec:plan_alg_imp}. % reference either implementation or experimental?
The third property ensures that the reference position, velocity and acceleration trajectories for the tracking controller are continuous. 

%%% Outline for reference

%\2 Describe the important components of a desired trajectory, such as a trajectory parameter $k \in K$ which uniquely determines its corresponding trajectory, a braking maneuver which ensures that the system can safely come to a stop, and that the reference position, velocity and acceleration trajectories are continuous. 
        
%        \3 Definition of a desired trajectory:
    
%        \begin{defn}
%        \label{def:traj_param}
%        For each $k \in K$, a \emph{desired trajectory} is a function $q_d(\cdot; k) : T \to \Q$ that satisfies the following properties:
        
%        \begin{enumerate}
        
%        \item The trajectory starts at a specified initial condition $(\initq, \initdq, \initddq)$, so that $q_d(0; k) = \initq$, $\dot{q}_d(0; k) = \initdq$, and $\ddot{q}_d(0; k) = \initddq$.
        
%        \item $\dot{q}_d(\tfin; k) = 0$ and $\ddot{q}_d(\tfin; k) = 0$ (i.e., each trajectory brakes to a stop, and at the final time has zero velocity and acceleration).
        
%        \item $\ddot{q}_d(\cdot; k)$ is Lipschitz continuous and bounded.
        
%        \end{enumerate}
%        \end{defn}

==> commands.tex <==


\newcommand{\regtext}[1]{\mathrm{\textnormal{#1}}}
\newcommand{\ts}[1]{\textsuperscript{#1}}

%%% Coloring the comment as blue
\newcommand{\Parker}[1]{{\normalsize{\textbf{({\color{blue}Parker:\ }#1)}}}}
\newcommand{\Ram}[1]{{\normalsize{\textbf{({\color{red}Ram:\ }#1)}}}}
\newcommand{\jon}[1]{{\normalsize{\textbf{({\color{purple}Jon:\ }#1)}}}}
\newcommand{\Zac}[1]{{\normalsize{\textbf{({\color{Orange}Zac:\ }#1)}}}}
\newcommand{\pat}[1]{{\normalsize{\textbf{({\color{yellow}Pat:\ }#1)}}}}
\newcommand{\bohao}[1]{{\normalsize{\textbf{({\color{green}Bohao:\ }#1)}}}}
\newcommand{\shrey}[1]{{\normalsize{\textbf{({\color{WildStrawberry}Shrey:\ }#1)}}}}

\newcommand{\MethodName}{RTD-Force}

% Commands From ARMTD Paper:
\newcommand{\plan}{_p}
\newcommand{\prev}{_\regtext{prev}}
\providecommand{\tfin}{t_\regtext{f}}

% common operations
\newcommand{\comp}{^{\regtext{C}}}
\newcommand{\card}[1]{\left\vert#1\right\vert}
\newcommand{\proj}{\regtext{proj}}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
% \newcommand{\pow}[1]{\regtext{pow}\!\left(#1\right)}
\newcommand{\pow}[1]{\mathcal{P}\!\left(#1\right)}
\newcommand{\diag}[1]{\regtext{diag}\!\left(#1\right)}
\newcommand{\eig}[1]{\regtext{eig}\!\left(#1\right)}
\newcommand{\union}{\bigcup}
\newcommand{\intersection}{\bigcap}
\newcommand{\trans}{^\top}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\sign}{\regtext{sign}}
\newcommand{\expm}{\regtext{exp}}
\newcommand{\logm}{\regtext{log}}
\newcommand{\skw}{_{\times}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\bdry}[1]{\regtext{bd}\!\left(#1\right)}
\renewcommand{\ker}[1]{\regtext{ker}\!\left(#1\right)}
\newcommand{\convhull}[1]{\regtext{CH}\!\left(#1\right)}

% Important Sets
\providecommand{\R}{\ensuremath \mathbb{R}}
\providecommand{\IR}{\ensuremath \mathbb{IR}}
\providecommand{\N}{\ensuremath \mathbb{N}}
\providecommand{\Q}{\ensuremath \mathbb{Q}}

% Trajectory Parameter
\newcommand{\kj}{k_j}
\newcommand{\Kj}{K_j}
% \newcommand{\avgkj}{\ol{\kj}}
% \newcommand{\delkj}{\delta\kj}

\newcommand{\kscale}{\eta_1}
\newcommand{\kjscale}{\eta_{j, 1}}
\newcommand{\koffset}{\eta_2}
\newcommand{\kjoffset}{\eta_{j, 2}}
\newcommand{\kvar}{x_k}
\newcommand{\kjvar}{x_{k_j}}

\newcommand{\tvar}{x_t}

\newcommand{\FK}{\regtext{\small{FK}}}
\newcommand{\IK}{\regtext{\small{IK}}}
\newcommand{\FO}{\regtext{\small{FO}}}
\newcommand{\IO}{\regtext{\small{IO}}}
\newcommand{\FS}{\regtext{\small{FS}}}
\newcommand{\IS}{\regtext{\small{IS}}}
\newcommand{\FC}{\regtext{\small{FC}}}
\newcommand{\IC}{\regtext{\small{IC}}}
\newcommand{\ID}{\regtext{\small{ID}}}

% disturbance
\newcommand{\bPhi}{\Phi}

% disturbance vector
\newcommand{\wdistlong}{w(t, \Delta)}
\newcommand{\wdist}{w}
\newcommand{\wdistnot}{w}
\newcommand{\wdistlongi}{w_i(t, \Delta)}

% interval disturbance vector
\newcommand{\wdistinterval}{w}
% norm of max disturbance
% \newcommand{\normwmax}{||w_{max}(t;k)||}

% Initial Conditions
\newcommand{\initq}{q_{d_0}}
\newcommand{\initqj}{q_{d, j_{0}}}
\newcommand{\initdq}{\dot{q}_{d_0}}
\newcommand{\initdqj}{\dot{q}_{d, j_{0}}}
\newcommand{\initddq}{\ddot{q}_{d_0}}
\newcommand{\initddqj}{\ddot{q}_{d, j_{0}}}

% manipulator equations
% \newcommand{\roboteqn}{\begin{split} \bM(\qtk, \Delta) \qddtk + \bC(\qtk, \qdtk, \Delta) \qdtk \\
% + \bG(\qtk, \Delta) = u(t;k) \end{split}}
\newcommand{\roboteqn}{\begin{split} \bM(\qt, \Delta) \qddt + \bC(\qt, \qdt, \Delta) \qdt \\
+ \bG(\qt, \Delta) = u(t) \end{split}}

% passivity-based controller
\newcommand{\nominal}{\begin{split} \tau(t;k) = & \bM(\qtk, \Delta_0) \qatkddot \\
& + \bC(\qtk, \qdtk, \Delta_0) \qatkdot + \bG(\qtk, \Delta_0) \end{split}}

% modified controller
\newcommand{\controller}{ u(\qA(t), \Delta_0, [\Delta]) = \tau(\qA(t), \Delta_0) - \robv(\qA(t), \Delta_0, [\Delta])}

% Manipulator equation
\newcommand{\bM}{M}
\newcommand{\Mq}{M(\qtk, \Delta)}
\newcommand{\Mqdot}{\dot{M}(\qtk, \Delta)}
\newcommand{\bMt}{\Tilde{M}}

\newcommand{\bC}{C}
\newcommand{\Cq}{C(\qtk, \qdtk)}
\newcommand{\Cqd}{C(\qtk, \qdtk, \Delta)}
\newcommand{\bCt}{\Tilde{C}}

\newcommand{\bG}{G}
\newcommand{\Gq}{G(\qtk)}
\newcommand{\Gqd}{G(\qtk, \Delta)}
\newcommand{\bGt}{\Tilde{G}}

\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfI}{\mathbf{I}}

% Manipulator Equation under Contact Featherstone
\newcommand{\bH}{H}
\newcommand{\bC}{C}
\newcommand{\btau}{\tau}

% parameters
\newcommand{\intparams}{[\Delta]}
\newcommand{\nomparams}{\Delta_0}
\newcommand{\trueparams}{\Delta}

% state variables
\newcommand{\q}{q}
\newcommand{\qt}{q(t)}
\newcommand{\qtk}{q(t;k)}
\newcommand{\qd}{\dot{q}}
\newcommand{\qdt}{\dot{q}(t)}
\newcommand{\qdtk}{\dot{q}(t;k)}
\newcommand{\qdd}{\ddot{q}}
\newcommand{\qddt}{\ddot{q}(t)}
\newcommand{\qddtk}{\ddot{q}(t;k)}
\newcommand{\qa}{q_a}
\newcommand{\qat}{q_a(t)}
\newcommand{\qadot}{\dot{q}_a}
\newcommand{\qaddot}{\ddot{q}_a}
\newcommand{\qatk}{q_a(t; k)}
\newcommand{\qatkdot}{\dot{q}_a(t; k)}
\newcommand{\qatkddot}{\ddot{q}_a(t; k)}
\newcommand{\qdes}{q_d}
\newcommand{\qdesdot}{\dot{q}_d}
\newcommand{\qdesddot}{\ddot{q}_d}
\newcommand{\qdest}{q_d(t)}
\newcommand{\qdestdot}{\dot{q}_d(t)}
\newcommand{\qdestddot}{\ddot{q}_d(t)}
\newcommand{\qdestk}{q_d(t; k)}
\newcommand{\qdestkdot}{\dot{q}_d(t; k)}
\newcommand{\qdestkddot}{\ddot{q}_d(t; k)}

% state variables no t
\newcommand{\qnot}{q}
\newcommand{\qdnot}{\dot{q}}
\newcommand{\qddnot}{\ddot{q}}
\newcommand{\qanot}{q_a}
\newcommand{\qadotnot}{\dot{q}_a}
\newcommand{\qaddotnot}{\ddot{q}_a}
\newcommand{\qdesnot}{q_d}
\newcommand{\qdesdotnot}{\dot{q}_d}
\newcommand{\qdesddotnot}{\ddot{q}_d}


% state variables indexed by j
\newcommand{\qj}{q_j(t)}
\newcommand{\qjnot}{q_j}
\newcommand{\ql}{q_l(t)}
\newcommand{\qdj}{\dot{q}_{j}(t)}
\newcommand{\qdjnot}{\dot{q}_{j}}
\newcommand{\qddj}{\ddot{q}_{j}(t)}
\newcommand{\qddjnot}{\ddot{q}_{j}}
\newcommand{\qaj}{q_{a, j}(t)}
\newcommand{\qajnot}{q_{a, j}}
\newcommand{\qajdot}{\dot{q}_{a, j}(t)}
\newcommand{\qajdotnot}{\dot{q}_{a, j}}
\newcommand{\qajddot}{\ddot{q}_{a, j}(t)}
\newcommand{\qajddotnot}{\ddot{q}_{a, j}}
\newcommand{\qdesj}{q_{d, j}(t)}
\newcommand{\qdesjdot}{\dot{q}_{d, j}(t)}
\newcommand{\qdesjddot}{\ddot{q}_{d, j}(t)}
\newcommand{\qdeskj}{q_{d, j}(t; k_j)}
\newcommand{\qdeskjdot}{\dot{q}_{d, j}(t; k_j)}
\newcommand{\qdeskjddot}{\ddot{q}_{d, j}(t; k_j)}

\newcommand{\qdeskjdotplan}{\dot{q}_{d, j}(t_{plan};k_j)}

\newcommand{\nq}{n_q}
\newcommand{\nt}{n_t}
\newcommand{\nf}{n_f}
\newcommand{\Nq}{ \{ 1, \ldots, \nq \} }
\newcommand{\Nqtwo}{ \{ 1, \ldots, \nq+2 \} }
\newcommand{\Nt}{ \{ 1, \ldots, \nt \} }


% robust input commands:
\newcommand{\err}{e}
\newcommand{\errdot}{\dot{e}}
\newcommand{\errj}{e_j}
\newcommand{\errjdot}{\dot{e}_j}
\newcommand{\errddot}{\ddot{e}}
\newcommand{\robv}{v}
\newcommand{\robvk}{v(t;k)}
\newcommand{\robvnot}{v}
\newcommand{\robr}{r}
\newcommand{\robrnot}{r}
\newcommand{\robw}{w(t)}
\newcommand{\robrdot}{\dot{r}}
\newcommand{\roblyap}{V(\qA(t), \Delta)}
\newcommand{\roblyapmax}{\overline{V}(\qtk, r(t))}
\newcommand{\roblyapdot}{\dot{V}(\qtk, r(t))}
\newcommand{\robh}{h(\qtk, r(t;k))}
\newcommand{\robhnot}{h}
\newcommand{\robH}{H}
% \newcommand{\robhmin}{\underline{h}(\qt, r(t;k))}
\newcommand{\robhmin}{\underline{h}(\qA(t),[\Delta])}
\newcommand{\robhdot}{\dot{h}(\qtk, r(t;k))}
\newcommand{\roblevel}{V_M}
% \newcommand{\robcoeff}{\gamma(t;k)}
\newcommand{\robcoeff}{\gamma}
\newcommand{\robKinf}{\alpha}
\newcommand{\robgain}{\alpha_c}
\newcommand{\ultbound}{\sqrt{\frac{2 \roblevel}{\sigma_m}}}
\newcommand{\pbound}{\epsilon_p}
\newcommand{\vbound}{\epsilon_v}
\newcommand{\pboundj}{\epsilon_{p, j}}
\newcommand{\vboundj}{\epsilon_{v, j}}
\newcommand{\pboundvec}{E_p}
\newcommand{\vboundvec}{E_v}
\newcommand{\epvar}{x_{e_p}}
\newcommand{\evvar}{x_{e_v}}
\newcommand{\epvarj}{x_{e_{p, j}}}
\newcommand{\evvarj}{x_{e_{v, j}}}
\newcommand{\qA}{q_A}
\newcommand{\normwmax}{||w_M||}
\newcommand{\wmax}{w_M}
\newcommand{\wmaxj}{w_{M, j}}

% deal with greek variables
\newcommand{\pzpboundj}{\bm{\epsilon}_{\mathbf{p, j}}}
\newcommand{\pzvboundj}{\bm{\epsilon}_{\mathbf{v, j}}}

% uniform bounds
\newcommand{\lambdamin}{\lambda_m}
\newcommand{\lambdamax}{\lambda_M}
\newcommand{\sigm}{\sigma_{m}}
\newcommand{\sigM}{\sigma_{M}}

% theorem blocks
\newtheorem{defn}{Definition}
\newtheorem{rem}[defn]{Remark}
\newtheorem{lem}[defn]{Lemma}
\newtheorem{prop}[defn]{Proposition}
\newtheorem{assum}[defn]{Assumption}
\newtheorem{ex}[defn]{Example}
\newtheorem{thm}[defn]{Theorem}
\newtheorem{cor}[defn]{Corollary}
\newtheorem{con}[defn]{Conjecture}
\newtheorem{problem}[defn]{Problem}


% special arrays
\newcommand{\emptyarr}{[\ ]}
\newcommand{\zeros}{\textit{0}}
\newcommand{\ones}{\textit{1}}
\newcommand{\eye}{\textit{I}}

% set representation
\newcommand{\interval}[1]{[ #1 ]}
\newcommand{\iv}[1]{[ #1 ]}
\newcommand{\nom}[1]{#1}
\newcommand{\pz}[1]{\mathbf{#1}}
\newcommand{\pzgreek}[1]{\bm{#1}}
\newcommand{\PZ}[1]{\mathcal{PZ}\left(#1\right)}
% can change symbol
% \newcommand{\pzt}[1]{\langle #1 \rangle_t}
% \newcommand{\pzkt}[1]{\langle #1 ; k \rangle_t}
% \newcommand{\pzk}[1]{\langle #1 ; k \rangle}
% \newcommand{\pzi}[1]{\langle #1 \rangle_i}
% \newcommand{\pzki}[1]{\langle #1 ; k \rangle_i}
% \newcommand{\pzjki}[1]{\langle #1 ; k_j \rangle_i}

\newcommand{\pzk}[1]{\pz{ #1 ; k }}
\newcommand{\pzi}[1]{\pz{ #1 }(\pz{T_i};\pz{K})}
\newcommand{\pzigreek}[1]{\pzgreek{ #1 }(\pz{T_i};\pz{K})}
\newcommand{\pzki}[1]{\pz{ #1 }(\pz{T_i};k)}
\newcommand{\pzjki}[1]{\pz{#1 ; k_j}}

\newcommand{\pzjknplan}[1]{\langle #1 ; k_j \rangle_{n_{plan}}}

% ith timestep
\newcommand{\pzqi}{\pzi{q}}
\newcommand{\pzqAi}{\pzi{\qA}}
\newcommand{\pzqdi}{\pzi{\dot{q}}}
\newcommand{\pzqdai}{\pzi{\dot{q}_{a}}}
\newcommand{\pzqddi}{\pzi{\ddot{q}}}
\newcommand{\pzqddai}{\pzi{\ddot{q}_{a}}}
\newcommand{\pzqdesi}{\pzi{q_{d}}}
\newcommand{\pzqddesi}{\pzi{\dot{q}_{d}}}
\newcommand{\pzqdddesi}{\pzi{\ddot{q}_{d}}}
\newcommand{\pzqdeski}{\pzki{q_{d}}}
\newcommand{\pzqddeski}{\pzki{\dot{q}_{d}}}
\newcommand{\pzqdddeski}{\pzki{\ddot{q}_{d}}}
\newcommand{\pzui}{\pzki{u}}
\newcommand{\pzqki}{\pzki{q}}
\newcommand{\pzqdki}{\pzki{\dot{q}}}
\newcommand{\pzuki}{\pzki{u}}

% jth joint at ith timestep
% \newcommand{\pzqji}{\pzi{q_j}}
% \newcommand{\pzqdji}{\pzi{\dot{q}_j}}
% \newcommand{\pzqdaji}{\pzi{\dot{q}_{a,j}}}
% \newcommand{\pzqddji}{\pzi{\ddot{q}_j}}
% \newcommand{\pzqddaji}{\pzi{\ddot{q}_{a,j}}}
% \newcommand{\pzqdesji}{\pzi{q_{d,j}}}
% \newcommand{\pzqddesji}{\pzi{\dot{q}_{d,j}}}
% \newcommand{\pzqdddesji}{\pzi{\ddot{q}_{d,j}}}
% \newcommand{\pzqdesjki}{\pzjki{q_{d,j}}}
% \newcommand{\pzqddesjki}{\pzjki{\dot{q}_{d,j}}}
% \newcommand{\pzqdddesjki}{\pzjki{\ddot{q}_{d,j}}}
% \newcommand{\pzuji}{\pzjki{u_j}}
% \newcommand{\pzqjki}{\pzjki{q_j}}
% \newcommand{\pzqdjki}{\pzjki{\dot{q}_j}}
% \newcommand{\pzujki}{\pzjki{u_j}}
% \newcommand{\pzqdddesjknplan}{\pzjknplan{\ddot{q}_{d,j}}}
\newcommand{\pzqji}{\pzi{q_j}}
\newcommand{\pzqAji}{\pzi{\qA_j}}
\newcommand{\pzqli}{\pzi{q_l}}
\newcommand{\pzqdji}{\pzi{\dot{q}_j}}
\newcommand{\pzqdaji}{\pzi{\dot{q}_{a,j}}}
\newcommand{\pzqddji}{\pzi{\ddot{q}_j}}
\newcommand{\pzqddaji}{\pzi{\ddot{q}_{a,j}}}
\newcommand{\pzqdesji}{\pzi{q_{d,j}}}
\newcommand{\pzqddesji}{\pzi{\dot{q}_{d,j}}}
\newcommand{\pzqdddesji}{\pzi{\ddot{q}_{d,j}}}
\newcommand{\pzqdesjki}{\pzki{q_{d,j}}}
\newcommand{\pzqddesjki}{\pzki{\dot{q}_{d,j}}}
\newcommand{\pzqdddesjki}{\pzki{\ddot{q}_{d,j}}}
\newcommand{\pzuji}{\pzki{u_j}}
\newcommand{\pzqjki}{\pzki{q_j}}
\newcommand{\pzqdjki}{\pzki{\dot{q}_j}}
\newcommand{\pzujki}{\pzki{u_j}}
\newcommand{\pzFKjki}{\pz{FK_j}(\pzqki)}
\newcommand{\pzFOjki}{\pz{FO_j}(\pzqki)}
\newcommand{\pzFKjKi}{\pz{FK_j}(\pzqi)}
\newcommand{\pzFOjKi}{\pz{FO_j}(\pzqi)}

% contact joint c at ith timestep
\newcommand{\pzqdci}{\pzi{\dot{q}_c}}
\newcommand{\pzqddci}{\pzi{\ddot{q}_c}}

% poly zono variables:
\newcommand{\pzg}{g}
\newcommand{\pzv}{x}
\newcommand{\pze}{\alpha}
\newcommand{\pzn}{{n_g}}
\newcommand{\pzgi}{g_i}
\newcommand{\pzei}{\alpha_i}
\newcommand{\pzgj}{g_j}
\newcommand{\pzej}{\alpha_j}

\newcommand{\ujt}{u_j(t)}

\newcommand{\pjt}{p_j(t)}
\newcommand{\Rjt}{R_j(t)}

\newcommand{\exact}{^{\regtext{exact}}}
\newcommand{\slice}{\textnormal{\texttt{slice}}}
\newcommand{\eval}{\textnormal{\texttt{eval}}}
\newcommand{\stack}{\textnormal{\texttt{stack}}}
\newcommand{\reduce}{\textnormal{\texttt{reduce}}}
\newcommand{\getCoeffValue}{\texttt{getCoeffValue}}
\newcommand{\timeint}{([0, T])}
% \newcommand{\upt}{^{(t)}}

% % \newcommand{\sensorhorizon}
\newcommand{\Aobs}{A_O}
\newcommand{\bobs}{b_O}
\newcommand{\hobs}{h_\regtext{obs}}
\newcommand{\nObs}{n_\mathscr{O}}
\newcommand{\obsset}{\mathscr{O}}

\newcommand{\unsafeobs}{_\regtext{obs}}
\newcommand{\unsafeself}{_\regtext{self}}
\newcommand{\unsafejoint}{_\regtext{lim}}
\newcommand{\jlim}{_\regtext{lim}}
\newcommand{\selfidx}{I\self}

\newcommand{\qlim}{q_{j,\regtext{lim}}}
\newcommand{\dqlim}{\dot{q}_{j,\regtext{lim}}}
\newcommand{\ddqlim}{\ddot{q}_{j,\regtext{lim}}}
\newcommand{\ulim}{u_{j,\regtext{lim}}}

% new commands for dynamics:
\newcommand{\iss}{_{i}^{i}}
\newcommand{\issm}{_{i-1}^{i}}
\newcommand{\issmu}{_{i}^{i-1}}
\newcommand{\issmi}{_{i-1, i}^{i}}
\newcommand{\issp}{_{i+1}^{i}}
\newcommand{\issmm}{_{i-1}^{i-1}}
\newcommand{\isspp}{_{i+1}^{i+1}}
\newcommand{\issa}{_{a, i}^{i}}
\newcommand{\issc}{_{c, i}^{i}}
\newcommand{\issma}{_{a, i-1}^{i}}
\newcommand{\isspa}{_{a, i+1}^{i}}
\newcommand{\issmma}{_{a, i-1}^{i-1}}
\newcommand{\issppa}{_{a, i+1}^{i+1}}

\newcommand{\jss}{_{j}^{j}}
\newcommand{\jssm}{_{j-1}^{j}}
\newcommand{\jssmu}{_{j}^{j-1}}
\newcommand{\jssmj}{_{j-1, j}^{j}}
\newcommand{\jssp}{_{j+1}^{j}}
\newcommand{\jssmm}{_{j-1}^{j-1}}
\newcommand{\jsspp}{_{j+1}^{j+1}}
\newcommand{\jssa}{_{a, j}^{j}}
\newcommand{\jssCOM}{_{CoM, j}^{j}}
\newcommand{\jssma}{_{a, j-1}^{j}}
\newcommand{\jsspa}{_{a, j+1}^{j}}
\newcommand{\jssmma}{_{a, j-1}^{j-1}}
\newcommand{\jssppa}{_{a, j+1}^{j+1}}

% other variables
% axis of rotation of jth joint
% \newcommand{\xi}{x_i} % Note: cannot use \xi anyways since it is command for Greek character
\newcommand{\xj}{x_j}
\newcommand{\zj}{z_j}

\newcommand{\rbf}{\mathbf{r}(t)}

\newcommand{\lssmu}{_{l}^{l-1}}

\newcommand{\qgoal}{q_\regtext{goal}}
\newcommand{\qstart}{q_\regtext{start}}

\newcommand{\timestep}{\Delta t}

\makeatletter
\newcommand{\smalloplus}{\mathbin{\mathpalette\make@small\oplus}}
% \newcommand{\bigoplus}{\mathbin{\mathpalette\make@big\oplus}}
\newcommand{\smallotimes}{\mathbin{\mathpalette\make@small\otimes}}



% waiter motion specific commands (Old)
% End Effector Expressions
% Contact Force Normal Component
%\newcommand{\FNorm}{\FGravInert_{N}}
% Contact Force Tangential Component
%\newcommand{\FTan}{\FGravInert_{T}}
% Contact Force
%\newcommand{\Fcontact}{F^{c}}
% Contact Moment
%\newcommand{\Mcontact}{M^{c}}
% Contact Wrench

% Radius of Contact Area for Loose Object
\newcommand{\objrad}{r}
% ZMP point??
\newcommand{\ZMPpoint}{Z}
% Vertical Height of the COM of the Loose Object
\newcommand{\heightobjCOM}{h_{CoM}}
% Coefficient of Static Friction Between the Supporting Surface and Loose Object
\newcommand{\CoefFric}{\mu_{s}} % need to look in planning alg theory section if changing
% Normal Vector of the Supporting Surface
\newcommand{\eenorm}{\hat{n}} % \overrightarrow{n}
% Gravito-Inertial Moment of Loose Object at COM
\newcommand{\MGravInert}{{\text{N}}_{c}(t)} % ^{G}
% Gravito-Inertial Force of Loose Object at COM
\newcommand{\FGravInert}{{\text{F}}_{c}(t)} % ^{G}
% Gravito-Inertial Moment of Loose Object at COM Projection
\newcommand{\MGravInertProj}{{\text{N}}_{c,P}(t)} % ^{G}
% Vector From the Normal Projection of COM to the ZMP Point
\newcommand{\ZMPvec}{\overrightarrow{PZ}}
% Point Representing the Normal Projection of COM onto the Supporting Surface
\newcommand{\COMproj}{P_{CoM}}
% Point Where the COM of the Object is Located
\newcommand{\objCOM}{G}


% Craig book RNEA related commands

% COM label
\newcommand{\COM}{CoM}
% COM velocity
\newcommand{\COMvel}{\text{v}_{j,\COM}^{j}(t)}
% COM acceleration
\newcommand{\COMaccel}{\dot{\text{v}}_{j,\COM}^{j}(t)}
% body angular velocity
\newcommand{\angvel}{\omega\jss}
% body angular acceleration
\newcommand{\angaccel}{\dot{\omega}\jss}

%% 08/23/2022 Contact Commands

% subscript to denote contact (like contact wrench)
\newcommand{\contact}{o}

% generic wrench
\newcommand{\genwrench}[1]{\mathrm{f}_{#1}} % \mathcal
\newcommand{\genwrenchPZ}[1]{\mathbf{f}_{#1}}
% generic external wrench
\newcommand{\genwrenchext}[1]{{\mathrm{F}}_{#1,ext}}
\newcommand{\genwrenchextPZ}[1]{\mathbf{\mathcal{F}}_{#1,ext}}
% contact wrench
\newcommand{\cwrench}{\mathrm{f}_{\contact}}
\newcommand{\cwrenchPZ}{\mathbf{f}_{\contact}}
% gravito inertial wrench (input is frame)
\newcommand{\gravinertwrench}[1]{{\mathrm{F}}_{#1}(t)} % ^{G}
\newcommand{\gravinertwrenchPZ}[1]{\mathbf{\mathcal{F}}_{#1}(t)} % ^{G}
% generic force vector at the joint
\newcommand{\genjointforce}{\text{f}\jss(t)}
\newcommand{\genjointforcenot}{\text{f}\jss}
\newcommand{\genjointforcenotPZ}{\text{\mathbf{f}}\jss}
% generic torque vector at the joint
\newcommand{\genjointtorque}{\text{n}\jss(t)}
\newcommand{\genjointtorquenot}{\text{n}\jss}
% generic force vector at the COM
\newcommand{\genCOMforce}{\text{F}\jss(t)}
\newcommand{\genCOMforcePZ}{\mathbf{F}\jss}
% generic torque vector at the COM
\newcommand{\genCOMtorque}{\text{N}\jss(t)}
\newcommand{\genCOMtorquePZ}{\mathbf{N}\jss}


% contact force vector
\newcommand{\cforce}{\text{f}_{c}(t)}
% contact force tangential component (contact frame)
\newcommand{\cforcetan}{{\text{f}}_{c,T}(t)}
% contact force normal component (contact frame)
\newcommand{\cforcenormal}{{\text{f}}_{c,N}(t)}
% contact force x-component (contact frame)
\newcommand{\cxforce}{\text{\text{f}}_{c,x}(t)}
\newcommand{\cxforcePZ}{\pzi{f_{\contact,x}}}
% contact force y-component (contact frame)
\newcommand{\cyforce}{\text{f}_{c,y}(t)}
\newcommand{\cyforcePZ}{\text{\mathbf{f}}_{\contact,y}}
% contact force z-component (contact frame)
\newcommand{\czforce}{\text{f}_{c,z}(t)}
\newcommand{\czforcePZ}{\text{\mathbf{f}}_{\contact,z}}

% contact moment vector
\newcommand{\cmoment}{{\text{n}}_{c}(t)}
% \newcommand{\cmomentPZ}{\mathbf{\text{n}}_{c}(t)}
% contact moment x-component (contact frame)
\newcommand{\cxmoment}{\text{n}_{c,x}(t)}
% contact moment y-component (contact frame)
\newcommand{\cymoment}{\text{n}_{c,y}(t)}
% contact moment z-component (contact frame)
\newcommand{\czmoment}{\text{n}_{c,z}(t)}
% maximum contact moment z-component (contact frame)
\newcommand{\czmomentmax}{\text{n}_{c,z,max}(t)}


% contact force vector
\newcommand{\cforcenot}{{\text{f}}_{c}}
\newcommand{\cforcenotPZ}{\text{\mathbf{f}}_{c}}
% contact force tangential component (contact frame)
\newcommand{\cforcetannot}{{\text{f}}_{c,T}}
\newcommand{\cforcetannotPZ}{\text{\mathbf{f}}_{c,T}}
% contact force normal component (contact frame)
\newcommand{\cforcenormalnot}{{\text{f}}_{c,N}}
\newcommand{\cforcenormalnotPZ}{\text{\mathbf{f}}_{c,N}}
% contact force x-component (contact frame)
\newcommand{\cxforcenot}{\text{f}_{c,x}}
\newcommand{\cxforcenotPZ}{\text{\mathbf{f}}_{c,x}}
% contact force y-component (contact frame)
\newcommand{\cyforcenot}{\text{f}_{c,y}}
\newcommand{\cyforcenotPZ}{\text{\mathbf{f}}_{c,y}}
% contact force z-component (contact frame)
\newcommand{\czforcenot}{\text{f}_{c,z}}
\newcommand{\czforcenotPZ}{\text{\mathbf{f}}_{c,z}}


% contact moment vector
\newcommand{\cmomentnot}{{\text{n}}_{c}}
\newcommand{\cmomentnotPZ}{\text{\mathbf{n}}_{c}}
% contact moment x-component (contact frame)
\newcommand{\cxmomentnot}{\text{n}_{c,x}}
\newcommand{\cxmomentnotPZ}{\text{\mathbf{n}}_{c,x}}
% contact moment y-component (contact frame)
\newcommand{\cymomentnot}{\text{n}_{c,y}}
\newcommand{\cymomentnotPZ}{\text{\mathbf{n}}_{c,y}}
% contact moment z-component (contact frame)
\newcommand{\czmomentnot}{\text{n}_{c,z}}
\newcommand{\czmomentnotPZ}{\text{\mathbf{n}}_{c,z}}
% maximum contact moment z-component (contact frame)
\newcommand{\czmomentmaxnot}{\text{n}_{c,z,max}}


% TRO paper method name title
\newcommand{\TROtitle}{ARMOUR}
